Tight Dimension Independent Lower Bound on the Expected Convergence Rate for Diminishing Step Sizes in SGD

We study the convergence of Stochastic Gradient Descent (SGD) for strongly convex objective functions. We prove for all $t$ a lower bound on the expected convergence rate after the $t$-th SGD iteration; the lower bound is over all possible sequences of diminishing step sizes. It implies that recently proposed sequences of step sizes at ICML 2018 and ICML 2019 are {\em universally} close to optimal in that the expected convergence rate after {\em each} iteration is within a factor $32$ of our lower bound. This factor is independent of dimension $d$. We offer a framework for comparing with lower bounds in state-of-the-art literature and when applied to SGD for strongly convex objective functions our lower bound is a significant factor $775\cdot d$ larger compared to existing work.

==> sections/10recurrence.tex <==
\section{Solving the Recurrence}

To prove the main result, we study the following recurrence. 
\begin{equation} Z_0=Y_0 \mbox{ and } Z_{t+1} = (1 - \mu \eta_t)Z_t + \eta_t^2 N, \label{recZ} \end{equation}
then by induction on $t$ we can prove the upper bound  $Y_t\leq Z_t$ if all  $\eta_t \leq \frac{1}{2L}$ where $Y_t$ is described in (\ref{main_ineq_sgd_new02}). 

The recurrence (\ref{recZ}) on $Z_t$ depends on the parameters $L$, $\mu$, $Y_0$, and $N$, where we want to chose the sequence of step sizes $\eta_t$ such that the $Z_t$ are minimized (in order to give the best possible upper bound on $Y_t$) under the constraints $\eta_t \leq \frac{1}{2L}$ (for which $Y_t\leq Z_t$ holds). In practice we know good estimates of $L$ and $\mu$. In our analysis below, we will show that the dependency of `optimal' $\eta_t$ on $Y_0$ and $N$ is in the form of a dependency on $N/Y_0$. We characterize the optimal $\eta_t$ that minimize $Z_t$ and we give precise lower and upper bounds on $Z_t$. 

In Section \ref{sec:tight1} we use the upper bound on $Z_t$ to show that the upper bound of $Y_t$ for our example is $\Ocal(t)$. 

%$Z_t$ is a tight bound for $Y_t$ by providing a class of examples for our main problem with convergence rates that meet $Z_t$ within a small factor for $t$ large enough.


%In Section \ref{sec:app} we use the lower bound on $Z_t$ to show that we can approximate $\eta_t$ by a step size function $\eta'_t$ which does not depend on $N/Y_0$ and we show that the resulting convergence rates meet the minimized $Z_t$ within a small factor for $t$ large enough. 
%
%In Section \ref{sec:tight} we use the upper bound on $Z_t$ to show that $Z_t$ is a tight bound for $Y_t$ by providing a class of examples for our main problem with convergence rates that meet $Z_t$ within a small factor for $t$ large enough.


\subsection{Minimizing Upper Bound $Z_t$ on the Convergence Rate}

\begin{thm}
\label{theorem:optimal_etat}
Let Assumptions~\ref{ass_stronglyconvex} ,\ref{ass_smooth} and \ref{ass_convex} hold. Let us consider Algorithm ~\ref{sgd_algorithm} with $N = 2 \mathbb{E}[ \|\nabla f(w_{*}; \xi)\|^2 ]$ and $Z_t$ as described in (~\ref{recZ}), i.e., $$Z_0=Y_0 \mbox{ and } Z_{t+1} = (1 - \mu \eta_t)Z_t + \eta_t^2 N.$$.
Let $Y_0 = \mathbb{E}[\|w_0 - w_*\|^2]$ and define  
\begin{equation}
\label{eqW}
W = 
  \begin{cases}{} 
 \lceil \frac{\ln( \frac{2 \mu L Y_0}{N}  - 1)}{\ln( (1- \frac{\mu}{2L})^{-1}  )}\rceil, & \mbox{if } \frac{N}{Y_0} < \mu L, \\
 0, & \mbox{if } \frac{N}{Y_0} \geq \mu L.
 \end{cases} 
\end{equation}

We consider the following sequence of $\eta_t$: 
\begin{itemize}
\item If $Y_0 \leq \frac{N}{\mu L}$, then $\eta_t = \frac{\mu Z_t}{2N}$ for $t\geq 0$.
\item Otherwise,  
\begin{equation}
 \eta_t = \left\{ \begin{array}{ll}
\frac{1}{2L}, & \mbox{if } t< W, \\
\frac{\mu Z_t}{2N}, & \mbox{if } t\geq W .
 \label{eqEta}
\end{array} \right.
\end{equation}
with
$$ \frac{N}{2\mu L} \leq Z_W \leq \frac{N}{\mu L}.$$
\end{itemize}
This stepsize minimizes $Z_t$. 
\end{thm}

The proof of Theorem~\ref{theorem:optimal_etat} is provided in Appendix~\ref{sec:append_01}. 

We also note that the analysis in Appendix~\ref{subsec:append_01_optimal_etat} shows
\begin{equation}
Z_W = 
 \left\{ \begin{array}{ll} 
\frac{N}{2\mu L} \leq Z_W \leq \frac{N}{\mu L}, & \mbox{if } \frac{N}{Y_0} < \mu L, \\
 Y_0\leq  \frac{N}{\mu L}, & \mbox{if } \frac{N}{Y_0} \geq \mu L.
\end{array} \right. \label{eqZW}
\end{equation}
We will use this property in the next subsection where we provide lower and upper bounds on the minimizing $Z_t$.

\subsection{Approximating the Minimal Bound $Z_t$ on the Convergence Rate}
The lower and upper bounds of minimized $Z_t$ in the above section are described in Theorem~\ref{theorem:bound_Zt}. 

\begin{thm}
\label{theorem:bound_Zt}
We consider the sequence $Z_t$ as described in~(\ref{recZ}), i.e., $$Z_0=Y_0 \mbox{ and } Z_{t+1} = (1 - \mu \eta_t)Z_t + \eta_t^2 N$$ where $\eta_t$ is defined as in Theorem~\ref{theorem:optimal_etat}. We have:
\begin{itemize}
\item For $t<W$ where $W$ is defined as in (\ref{eqW}),  $$Z_t=\frac{N}{2 \mu L} + (1-\frac{\mu}{2L})^{t} (Y_0 - \frac{N}{2 \mu L} ).$$
\item For $t\geq W$, we have the following tight upper and lower bounds of $Z_t$
\begin{equation}
\label{approxZ} 
 \frac{4N}{\mu^2} \frac{1}{ (t-W) + \frac{4N}{\mu^2 Z_W}}  \geq  Z_{t} \geq 
 \frac{4N}{\mu^2} \frac{1}{ (t-W) + \frac{4N}{\mu^2 Z_W} + \ln(t-W+ \frac{4N}{\mu^2 Z_W}) - \ln( \frac{4N}{\mu^2 Z_W})}. 
\end{equation}

Let define $\omega = \max\{\frac{N}{\mu L Y_0},1\}$. We have general weaker upper bound and lower bound of $Z_t$ as follows.

\textbf{Weaker Upper Bound}
\begin{equation} 
\label{eqUP}
Z_t \leq  \frac{4N}{\mu} \frac{1}{ \mu t- 2L \ln( \frac{2 \omega \mu L Y_0}{N}  - 1) + 4L\omega }.
\end{equation}

\textbf{Weaker Lower Bound}
\begin{equation}
Z_t \geq \frac{4N}{\mu} \frac{1}{ \mu (t +\ln( \frac{t\mu}{4L\omega}+1))   +  8L\omega   }. \label{eqLOW}
\end{equation} 

\end{itemize}
\end{thm}

The detailed proof of Theorem~\ref{theorem:bound_Zt} is provided in Appendix~\ref{subsec:append_01_bound_Zt}




==> sections/1recurrence.tex <==
\section{Solving the Recurrence}

The recurrence (\ref{recZ}) on $Z_t$ depends on the parameters $L$, $\mu$, $Y_0$, and $N$, where we want to chose the sequence of step sizes $\eta_t$ such that the $Z_t$ are minimized (in order to give the best possible upper bound on $Y_t$) under the constraints $\eta_t \leq \frac{1}{2L}$ (for which $Y_t\leq Z_t$ holds). In practice we know good estimates of $L$ and $\mu$. In our analysis below, we will show that the dependency of `optimal' $\eta_t$ on $Y_0$ and $N$ is in the form of a dependency on $N/Y_0$. We characterize the optimal $\eta_t$ that minimize $Z_t$ and we give precise lower and upper bounds on $Z_t$. 

In Section \ref{sec:app} we use the lower bound on $Z_t$ to show that we can approximate $\eta_t$ by a step size function $\eta'_t$ which does not depend on $N/Y_0$ and we show that the resulting convergence rates meet the minimized $Z_t$ within a small factor for $t$ large enough. In Section \ref{sec:tight} we use the upper bound on $Z_t$ to show that $Z_t$ is a tight bound for $Y_t$ by providing a class of examples for our main problem with convergence rates that meet $Z_t$ within a small factor for $t$ large enough.


\subsection{Minimizing Upper Bound $Z_t$ on the Convergence Rate}

\begin{thm}
\label{theorem:optimal_etat}
Let Assumptions~\ref{ass_stronglyconvex} ,\ref{ass_smooth} and \ref{ass_convex} hold. Let us consider Algorithm ~\ref{sgd_algorithm} with $N = 2 \mathbb{E}[ \|\nabla f(w_{*}; \xi)\|^2 ]$ and $Z_t$ as described in (~\ref{recZ}), i.e., $$Z_0=Y_0 \mbox{ and } Z_{t+1} = (1 - \mu \eta_t)Z_t + \eta_t^2 N.$$.
Let $Y_0 = \mathbb{E}[\|w_0 - w_*\|^2]$ and define  
\begin{equation}
\label{eqW}
W = 
  \begin{cases}{} 
 \lceil \frac{\ln( \frac{2 \mu L Y_0}{N}  - 1)}{\ln( (1- \frac{\mu}{2L})^{-1}  )}\rceil, & \mbox{if } \frac{N}{Y_0} < \mu L, \\
 0, & \mbox{if } \frac{N}{Y_0} \geq \mu L.
 \end{cases} 
\end{equation}

We consider the following sequence of $\eta_t$: 
\begin{itemize}
\item If $Y_0 \leq \frac{N}{\mu L}$, then $\eta_t = \frac{\mu Z_t}{2N}$ for $t\geq 0$.
\item Otherwise,  
\begin{equation}
 \eta_t = \left\{ \begin{array}{ll}
\frac{1}{2L}, & \mbox{if } t< W, \\
\frac{\mu Z_t}{2N}, & \mbox{if } t\geq W .
 \label{eqEta}
\end{array} \right.
\end{equation}
with
$$ \frac{N}{2\mu L} \leq Z_W \leq \frac{N}{\mu L}.$$
\end{itemize}
This stepsize minimizes $Z_t$. 
\end{thm}

The proof of Theorem~\ref{theorem:optimal_etat} is provided in Appendix~\ref{sec:append_01}. 

We also note that the analysis in Appendix~\ref{subsec:append_01_optimal_etat} shows
\begin{equation}
Z_W = 
 \left\{ \begin{array}{ll} 
\frac{N}{2\mu L} \leq Z_W \leq \frac{N}{\mu L}, & \mbox{if } \frac{N}{Y_0} < \mu L, \\
 Y_0\leq  \frac{N}{\mu L}, & \mbox{if } \frac{N}{Y_0} \geq \mu L.
\end{array} \right. \label{eqZW}
\end{equation}
We will use this property in the next subsection where we provide lower and upper bounds on the minimizing $Z_t$.

\subsection{Approximating the Minimal Bound $Z_t$ on the Convergence Rate}
The lower and upper bounds of minimized $Z_t$ in the above section are described in Theorem~\ref{theorem:bound_Zt}. 

\begin{thm}
\label{theorem:bound_Zt}
We consider the sequence $Z_t$ as described in~(\ref{recZ}), i.e., $$Z_0=Y_0 \mbox{ and } Z_{t+1} = (1 - \mu \eta_t)Z_t + \eta_t^2 N$$ where $\eta_t$ is defined as in Theorem~\ref{theorem:optimal_etat}. We have:
\begin{itemize}
\item For $t<W$ where $W$ is defined as in (\ref{eqW}),  $$Z_t=\frac{N}{2 \mu L} + (1-\frac{\mu}{2L})^{t} (Y_0 - \frac{N}{2 \mu L} ).$$
\item For $t\geq W$, we have the following tight upper and lower bounds of $Z_t$
\begin{equation}
\label{approxZ} 
 \frac{4N}{\mu^2} \frac{1}{ (t-W) + \frac{4N}{\mu^2 Z_W}}  \geq  Z_{t} \geq 
 \frac{4N}{\mu^2} \frac{1}{ (t-W) + \frac{4N}{\mu^2 Z_W} + \ln(t-W+ \frac{4N}{\mu^2 Z_W}) - \ln( \frac{4N}{\mu^2 Z_W})}. 
\end{equation}

Let define $\omega = \max\{\frac{N}{\mu L Y_0},1\}$. We have general weaker upper bound and lower bound of $Z_t$ as follows.

\textbf{Weaker Upper Bound}
\begin{equation} 
\label{eqUP}
Z_t \leq  \frac{4N}{\mu} \frac{1}{ \mu t- 2L \ln( \frac{2 \omega \mu L Y_0}{N}  - 1) + 4L\omega }.
\end{equation}

\textbf{Weaker Lower Bound}
\begin{equation}
Z_t \geq \frac{4N}{\mu} \frac{1}{ \mu (t +\ln( \frac{t\mu}{4L\omega}+1))   +  8L\omega   }. \label{eqLOW}
\end{equation} 

\end{itemize}
\end{thm}

The detailed proof of Theorem~\ref{theorem:bound_Zt} is provided in Appendix~\ref{subsec:append_01_bound_Zt}




==> sections/2approximating.tex <==
\section{Approximating the Optimal Step Sizes}
\label{sec:app}

We propose to use upper bound (\ref{eqUP}) on $Z_t$ in (\ref{eqEta}) to create a new, but hopefully close to optimal, candidate step size function $\eta'_t$. According to (\ref{eqEta}) this gives candidate $\eta'_t=\frac{1}{2L}$  if $t<W\approx \frac{2L}{\mu} \ln( \frac{2 \omega \mu L Y_0}{N}  - 1)$, and for $t\geq W$,
$$\eta'_t = \frac{2}{ \mu t- 2L \ln( \frac{2 \omega \mu L Y_0}{N}  - 1) + 4L\omega }.$$
Still $\eta'_t$ depends on the unknown parameter $\frac{Y_0}{N}$ in a rather complex way. A much coarser approximation would be to simply substitute $0$ for $W$ (it seems $W$ may often be equal to $0$ and if not, it may be rather small in relation to the larger $t$ which we see used in practice). And in addition we want to replace constant  $-2L \ln(\frac{2 \omega \mu L Y_0}{N}  - 1) + 4L\omega$ by $4L$ making it independent of $\frac{Y_0}{N}$. This leads to the candidate step size function 
\begin{equation}
 \eta'_t = \frac{2}{\mu t + 4L} \mbox{ for } t\geq 0. \label{eqCand}
 \end{equation}
Note that this candidate step size function has no dependency on the unknown parameters $N$ and $Y_0$ at all.

It turns out that step size function $\eta'_t$ in (\ref{eqCand}) has been analysed in Theorem 2 of \cite{Nguyen2018} where the following convergence bound has been proved: Let $Y'_t$ denote the convergence rate for step sizes $\eta'_t$ in the SGD algorithm. 

Then,
\begin{equation} Y'_t \leq  Z'_t \overset{\text{Theorem 2}\cite{Nguyen2018}}{=} \frac{16N}{\mu} \frac{1}{\mu (t -T') +4L}, \label{eqAPPRSOL} \end{equation}
for ($Y'_0=Y_0$)
$$ t\geq T' =  \frac{4L}{\mu} \max\{ \frac{L\mu Y_0}{N}, 1\} -\frac{4L}{\mu}
= \frac{4L}{\mu} \omega \mu L \frac{Y_0}{N} - \frac{4L}{\mu} =\frac{4L^2 \omega Y_0}{N} - \frac{4L}{\mu}.$$

We notice that $\frac{\omega \mu L Y_0}{N} \geq 1$ and $\ln x \leq x-1$ for $x\geq 1$. Applying this to $W$ gives (see (\ref{appW1}))
$$W \approx \frac{2L}{\mu} \ln( \frac{2 \omega \mu L Y_0}{N}  - 1) \leq \frac{2L}{\mu} (\frac{2\omega \mu L Y_0}{N}-2) = 4L^2 \omega Y_0/N - 4L/\mu=T'.$$
So, if $t\geq T'=4L^2 \omega Y_0/N - 4L/\mu$ then also $t\geq W$ and we have the lower bound (\ref{eqLOW}) on $Z_t$. 

Convergence rates $Y_t$ correspond to the optimal step sizes $\eta_t$ and we have shown $Y_t\leq Z_t$. In the next section we show a class of examples that show that this upper bound is tight within a factor $\approx 8$ for $t$ large enough. This means that within a factor $\approx 8$ for $t$ large enough the lower bound (\ref{eqLOW}) on $Z_t$ can be met (or possibly be surpassed) by the $Y_t$ for this class of examples. Therefore,
comparing the 
lower bound (\ref{eqLOW}) on $Z_t$ 
 and the upper bound $Z'_t$ on $Y'_t$ in  (\ref{eqAPPRSOL})  tells us how close the convergence rate corresponding to $\eta'_t$ and the convergence rate corresponding to the optimal $\eta_t$ (as defined in the previous section) are.
 
\begin{thm}
\label{theorem:ration_zt_ztp}
Assume  $\frac{\mu}{2L} \ll 1$ and $q$ is a constant which is larger or equal to 2. For given weaker lower bound of $Z_t$ as described in (\ref{eqLOW}) and upper bound $Z'_t$ as shown in (\ref{eqAPPRSOL}), we have:
 \begin{equation}
  (\ref{eqAPPRSOL})/ (\ref{eqLOW})  \leq
 4 \frac{q + 2\max\{0, \frac{N}{\mu L Y_0} -1\}  }{q-1} .\label{factorA}
 \end{equation}
\end{thm} 

The proof of Theorem~\ref{theorem:ration_zt_ztp} is provided in Appendix~\ref{append:approximation_stepsize}. 
 
So, for $\frac{N}{\mu L Y_0}\leq 1$  we can get within a factor  $4\frac{q}{q-1}$ for 
\begin{align*}
t &=  q \frac{4L}{\mu} \max\{ \frac{L\mu Y_0}{N}, 1\} - \frac{8L}{\mu}
 =  q \frac{4L}{\mu}\frac{L\mu Y_0}{N}- \frac{8L}{\mu} \leq (q-2) \frac{4L^2 Y_0}{N}
\end{align*} 
 with $q\geq 2$. If  $\frac{N}{\mu L Y_0}> 1$, i.e., $\frac{Y_0}{N} \leq \frac{1}{\mu L}$, then for  $$t= q \frac{4L}{\mu} \max\{ \frac{L\mu Y_0}{N}, 1\} - \frac{8L}{\mu} =  (q-2)\frac{4L}{\mu}$$ with $q\geq 2$ we can get within a factor 
   $4\frac{q+ 2(\frac{N}{\mu L Y_0} -1)}{q-1}$. Combining both arguments shows that (\ref{factorA}) holds for
   $$ t\geq (q-2)\frac{4L}{\mu} \max \{ \frac{\mu L Y_0}{N}, 1\} \mbox{ with } q\geq 2.$$
   
    The above shows that the convergence rate of the approximate solution $\eta'_t$ which is independent from $N$ and $Y_0$ approaches bound $Z_t$ on the convergence rate $Y_t$ of the optimal solution $\eta_t$ within a factor close to $4$ for $t$ large enough.

==> sections/3experimental.tex <==
\section{Experimental Validation}
 
TO DO Experimental results show that for common data sets $N/(\mu L Y_0)\leq 1$. .... Compare optimal versus approximate stepsizes. Also depict the bounds:
\begin{itemize}
 \item Simulated $Y_t$ for optimal stepsizes $\eta_t$
 \item Simulated $Y'_t$ for $\eta'_t$
 \item Actual $Z_t$, and lower and upper bounds on $Z_t$
 \item The bound $Z'_t$ (on $Y'_t$)
\end{itemize}
 
 This shows ``tightness'' within smaller $<32$ factor for practical data sets.
 
We show in the next section that theoretical examples can be constructed showing that ``this factor'' cannot be larger than 32 -- refer to general conclusion abstract etc.

For our numerical experiments, we consider the finite sum minimization problem
\begin{align*}
\min_{w\in \mathbb{R}^d} \left\{ F(w) = \frac{1}{n} \sum_{i=1}^n f_i(w) \right\}. \tagthis \label{finite_sum}
\end{align*}

Specifically, for strongly convex objective function, we consider $\ell_2$-regularized logistic regression problems with
\begin{align*}
f_i(w) &= \log(1 + \exp(-y_i x_i^\top w)) + \frac{\lambda}{2} \| w \|^2, 
\end{align*}
where the penalty parameter $\lambda$ is set to $1/n$, a widely-used value in literature (see e.g. \cite{Nguyen2017_sarah}). We conducted experiments for Algorithm \ref{sgd_algorithm} on some various datasets: \texttt{covtype} ($n = 406,708$ training data), \texttt{ijcnn1} ($n = 91,701$ training data), \texttt{w8a} ($n = 49,749$ training data), and \texttt{phishing} ($n = 7,738$ training data) from the LIBSVM\footnote{http://www.csie.ntu.edu.tw/$\sim$cjlin/libsvmtools/datasets/} website. The optimal solution $w_*$ of the strongly convex problem \eqref{finite_sum} is found by using SARAH method \cite{Nguyen2017_sarah} with the stopping criterion $\|\nabla F(w_*)\|^2 \leq 10^{-20}$. 

==> sections/4tightness.tex <==
\section{Tightness of the Convergence Rate $Z_t$}
\label{sec:tight}
 
\begin{thm}
\label{theorem:example_tightness}
We consider a multivariate normal distribution of a $k$-dimensional random vector $\xi$, i.e., $\xi \sim \mathcal{N}(m,\Sigma)$, where $m=\mathrm{E}[\xi]$ and $\Sigma = \mathrm{E}[(\xi-m)(\xi-m)^{\mathrm{T}}]$ is the (symmetric positive semi-definite) covariance matrix. The density function of $\xi$ is
$$
g(\xi) = \frac{\exp( \frac{- (\xi-m)^\mathrm{T}\Sigma^{-1}(\xi-m)}{2} )}{\sqrt{(2\pi)^k|\Sigma|}}. 
$$

We select  component functions 
 $$f(w;\xi)=s(\xi)\frac{\|w-\xi\|^2}{2},$$
 where function $s(\xi)$ is constructed {\em a-priori} according to the following random process: 
 \begin{itemize} 
 \item With probability $1-\mu/L$, we draw $s(\xi)$ from the uniform distribution over interval $[0, \mu/(1-\mu/L)]$, and
 \item with probability $\mu/L$, we draw $s(\xi)$ from the uniform distribution over interval $[0, L]$.
 \end{itemize}
We run Algorithm~\ref{sgd_algorithm} with stepsize $\eta_t$ as described in~(\ref{eqCand})
(i.e., $\eta_t = \frac{2}{\mu t + 4L} \mbox{ for } t\geq 0$). Then
\begin{equation}
 \label{tightLOW}
 Y_t \geq \frac{N}{2\mu} \frac{1}{\mu (t + \ln(t+ L/12 ))} ,
\end{equation}
For $t\geq W \approx \frac{4.796\cdot L}{\mu}$,
\begin{equation}
\label{tightZUP}
Z_t \leq \frac{4N}{\mu} \frac{1}{ \mu t- 0.796\cdot L }. 
\end{equation}
Now we can compare (\ref{tightLOW}) and (\ref{tightZUP}): For $t\geq  \frac{4.796\cdot L}{\mu}$,
\begin{equation}
\frac{(\ref{tightZUP})}{(\ref{tightLOW})} 
= \frac{ \frac{4N}{\mu} \frac{1}{ \mu t- 0.796\cdot L }}{ \frac{N}{2\mu} \frac{1}{\mu (t + \ln(t+ L/12 ) )}}
= 8 \frac{t + \ln(t+ L/12 )}{ t - 0.796\cdot L/\mu }.
\label{factorT}
\end{equation}
\end{thm}

The proof of Theorem~\ref{theorem:example_tightness} is provided in Appendix~\ref{sec:example_tightness}.

This proves that for large enough $t$, our example meets the minimizing $Z_t$ within a factor $\approx 8$. In other words, the bound $Y_t\leq Z_t$ cannot be improved by a factor larger than $8$ unless additional assumptions are stated with which a smaller bound can be proven.

As a final note we remark that the above analysis also holds if we define each component function $f(w;\xi)$ with its own symmetric  positive semi-definite correlation matrix $\Sigma(\xi)$ drawn from a general distribution with $\mathrm{E}[\Sigma(\xi)]=\Sigma$. This shows that the class of examples leading to a tight bound is even somewhat more general and larger.

\subsection{Numerical Experiments}\label{subsec_numerical_tightness}

We verify our theory by considering simulations with different values of sample size $n$ (1000, 10000, and 100000) and vector size $d$ (10, 100, and 1000). First, we generate $n$ vectors of size $d$ with mean $m$ and positive definite covariance matrix $\Sigma$. To be simple, we generate $m \in \mathbb{R}^d$ and diagonal matrix $\Sigma \in \mathbb{R}^{d \times d}$ with uniform at random in $[0,1]$ for each element in $m$ and each element in the diagonal of $\Sigma$. We experimented with 10 runs and reported the average results. 

\begin{figure}[h]
 \centering
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_100000_s3_1000}
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_100000_s4_1000}
   \caption{$Y_t$ with its lower bound and $Z_t$ with its upper bound ($n = 100,000$ and $d = 1,000$)}
  \label{figure_100000_1000}
 \end{figure}

We denote the label ``Lower Y$\_$t'' and ``Upper Z$\_$t'' in the figure as the lower bound of $Y_t$ in \eqref{tightLOW} and the upper bound of $Z_t$ in \eqref{tightZUP}, respectively. Due to the space limit, we provide a single example with $n = 100,000$ and $d = 1,000$ to show $Y_t$ with its lower bound and $Z_t$ with its upper bound in Figure~\ref{figure_100000_1000}. More experiments with different values of $n$ and $d$ can be found in Appendix~\ref{sec:experiments_tightness}. 


==> sections/5conclusion.tex <==
\section{Concluding Remarks}

\noindent
{\bf Summary.} We should that the convergence rate $Y_t$ in SGD can be upper bounded by $Y_t\leq Z_t$ where (after minimization over all possible step size functions) $Z_t$ is characterized by  (\ref{eqEta}) with (\ref{eqW})  in combination with recurrence (\ref{recZ}). The resulting $Z_t$ is a complex function in the unknown parameters $N$ and $Y_0$. In we show  lower and upper bounds,  (\ref{eqLOW}) and  (\ref{eqUP}),  on $Z_t$ that are simple functions in $N$ and $Y_0$ and hold for $\mu/(2L)$ small and $t\geq W$ with $W$ satisfying (\ref{appW1}).

The lower and upper bounds allow us to conclude our two main results assuming $\mu/L$ small:
\begin{enumerate}
\item For step sizes $\eta'_t  = \frac{2}{\mu t + 4L}$,  for $ t\geq 0$, see (\ref{eqCand}) and Theorem 2 in \cite{Nguyen2018}, we show that the resulting convergence rates $Y_t$ are upper bounded by  (\ref{eqAPPRSOL}) and we use this to prove that $Y_t$ is at most a factor $\tau_1$ larger than the lower bound (\ref{eqLOW}) on $Z_t$, where (see (\ref{factorA}))
$$ \tau_1 \leq  4 \frac{q + 2\max\{0, N/(\mu L Y_0) -1\}  }{q-1}$$
and
$$  t\geq (q-2)\frac{4L}{\mu} \max \{ \mu L Y_0/N, 1\} \mbox{ with } q\geq 2.$$
This shows that $Y_t$ is at most  approximately a factor $4$ worse than $Z_t$ for $t=O(L/\mu)$ large enough.
\item We provide a class with problems $\tt{P}'$ of $\mu$-strongly convex objective functions $F(w)$ with convex $L$-smooth component functions $f(w;\xi)$ and distribution $g(\xi)$ for which the SGD algorithm achieves  convergence rates $Y_t$ with the property that the upper bound  (\ref{eqUP}) on $Z_t$ is at most a factor $\tau_2$ larger than $Y_t$, where (see (\ref{factorT})
$$ \tau_2 \leq 8 \frac{t + \ln(t+ L/12 )}{ t - 0.796\cdot L/\mu }.
\label{factorT}$$
and
$$ t\geq  \frac{4.796\cdot L}{\mu}.$$
This shows that, for this class of examples,  $Z_t$  is at most approximately a factor $8$ worse than $Y_t$ for $t=O(L/\mu)$ large enough.
\end{enumerate}




The above results show that if we define the convergence rate  $Y_t(\tt{P}, \eta)$ in SGD as a function of the problem statement $\tt{P}$ and the step size function $\eta$, and  if we define the minimizing upper bound $Z_t(\tt{P})$ as a function of the problem statement $\tt{P}$ (minimized over all possible step size functions),
then, for $t=O(\mu/L)$, we have 
$\inf_{\eta} Y_t(\tt{P},\eta) \leq Z_t(\tt{P})$,
$$ Y_t(\tt{P},\eta') \leq \tau_1 Z_t(\tt{P}),$$
and
$$ Z_t(\tt{P}') \leq \tau_2 \inf_{\eta} Y_t(\tt{P}',\eta).$$
This implies that $Z_t(\tt{P}')$ is close to $\inf_{\eta} Y_t(\tt{P}',\eta)$ within a factor $\tau_2\approx 8$, and $Y_t(\tt{P},\eta')$ meets $ Z_t(\tt{P}$ within a factor $\tau_1\approx 4$. As result 
$$ \sup_{\tt{P}}  Y_t(\tt{P},\eta') \leq \tau_1 \tau_2  \sup_{\tt{P}}  \inf_{\eta} Y_t(\tt{P},\eta),$$
where $\tau_1\tau_2 \approx 32$ for $t=O(L/\mu)$ large enough.
This shows that choosing stepsizes $\eta'_t$ is a factor 32 close to optimal.

\vspace{2mm}

\noindent
{\bf Convexity.} If we do not require the component functions $f(w;\xi)$ to be convex as in Theorem 3 in \cite{Nguyen2018}, then the general recurrence will only hold for much smaller step sizes\footnote{As for the recurrence in \cite{Moulines2011}, see introduction. The proof in  \cite{Moulines2011} does require the component functions to be convex.} $\eta_t\leq \mu/(2L^2)$. This means that our anlysis will lead to much larger $W$ and as a result  the above conclusion will only hold for $t=O( (L/\mu)^2)$.

\textcolor{red}{Ha: i stop here}


TO DO Verify -- should be easy.

\vspace{2mm}

\noindent
{\bf Minibatch SGD.} TO DO (if we want this): Write out recurrence with $k_t$. One can do a similar analysis as above -- quickly verify what it gives -- my bet: the exact same factors. And no improvement over SGD at all, except $W$ may be smaller, so only $t=O(L/(k \mu))$ will be sufficient for our conclusions  ($k_t \approx k$).

\vspace{2mm}

\noindent
{\bf Transition Linear to Sublinear Convergence.} Our anlysis of $Z_t$ shows that for $t< W$ we can achieve linear convergence and for $t\geq W$ we achieve sublinear convergence. Our approximate solution $\eta'_t$ only starts to lead to convergence rates that come within a factor $4$ of $Z_t$ for $t$ at least a multiple of $W$, about $t\approx 2W$. This shows that the approximate solution completely misses the linear convergence phase. Yet, it catches up with some delay of $\approx 2W=O(\mu/L)$ after which the approximate solution achieves a convergence rate at iteration $t$ which lags about $4/\mu$ iterations behind (in that it achieves the convergence rate of the optimal solution at iteration $t-4/\mu$). TO DO HMMM - NOT SURE ABOUT THIS LAST CONCLUSION: VERIFY and remove or adapt, what do the experiments tell?

TO DO explain the above better



==> sections/Analysis_SGD.tex <==
\section{Analysis of the convergence of SGD}
\label{sec:convergence_SGD}


\subsection{Proof of Convergence}
\label{subsec:proof_convergence}

We note that the classical stepsize proposed in \cite{RM1951}: 
\begin{align*}
\sum_{t=1}^{\infty} \eta_t = \infty \ \text{and} \ \sum_{t=1}^{\infty} \eta_t^2 < \infty
\end{align*}
is very famous in convex optimization literature. 
It could achieve the desired balance between diminishing the stepsizes sufficiently quickly to ensure convergence, but not so quickly so as to prevent the iterates from reaching the minimizer. 

In this section, we extend the class of stepsizes which make SGD converge using Lemma~\ref{lemma:hogwild_recursive_form}, i.e., we want to relax the condition $\sum_{t=0}^{\infty} \eta_t^2 < \infty$. 
 
Let $\mathcal{F}_{t} = \sigma(w_{1},\xi_{1},\dots,\xi_{t-1})$ is the $\sigma$-algebra generated by $w_{1},\xi_{1},\dots,\xi_{t-1}$, i.e., $\mathcal{F}_{t}$ contains all the information of $w_{1},\dots,w_{t}$. The sequence of random variables $\{\xi_t\}_{t \geq 1}$ is assumed to  be i.i.d.\footnote{Independent and identically distributed.}
If Assumptions~\ref{ass_stronglyconvex},~\ref{ass_convex} and ~\ref{ass_smooth} hold, then by Lemma \ref{lem_bounded_secondmoment_04}, we have

\begin{gather*}
\mathbb{E}[\|\nabla f(w;\xi)\|^2 | \mathcal{F}_{t} ] \leq  4 L [ F(w_{t}) - F(w_{*}) ] + N. \tagthis \label{ineq:bounded_lemma3_new02}
\end{gather*}

Hence, $\mathbb{E}[\| w_{t+1} - w_{*} \|^2 | \mathcal{F}_{t}]$
\begin{align*}
 & = \mathbb{E}[ \| w_{t} - \eta_t \nabla f(w_{t};\xi_t) - w_{*} \|^2 | \mathcal{F}_{t}] \\
& = \| w_{t} - w_{*} \|^2 - 2 \eta_t \langle \nabla F(w_{t})  , (w_{t} - w_{*}) \rangle + \eta_t^2 \mathbb{E}[\|\nabla f(w_{t}; \xi_t)\|^2 | \mathcal{F}_{t} ] \\
& \overset{\eqref{eq:stronglyconvex_00}\eqref{ineq:bounded_lemma3_new02}}{\leq} \| w_{t} - w_{*} \|^2 - \mu \eta_t \| w_{t} - w_{*} \|^2 - 2 \eta_t [ F(w_{t}) - F(w_{*}) ] + 4 L \eta_t^2 [ F(w_{t}) - F(w_{*}) ]  + \eta_t^2 N \\
& = \| w_{t} - w_{*} \|^2 - \mu \eta_t \| w_{t} - w_{*} \|^2 - 2 \eta_t ( 1 - 2 L \eta_t) [ F(w_{t}) - F(w_{*}) ]  + \eta_t^2 N \\
& \leq \| w_{t} - w_{*} \|^2 - \mu \eta_t \| w_{t} - w_{*} \|^2  + \eta_t^2 N.
\end{align*}

The last inequality follows since $0 < \eta_t \leq \frac{1}{2L}$. Therefore,
\begin{align*}
\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]  \leq (1-\mu \eta_t) \mathbb{E}[ \| w_{t} - w_{*} \|^2 ] + \eta_t^2 N. \tagthis \label{main_ineq_sgd_new02}
\end{align*}

Note that with Assumptions~\ref{ass_stronglyconvex} and ~\ref{ass_smooth} hold with $\eta_t \leq \frac{1}{2L\kappa}$(i.e., no Assumption~\ref{ass_convex}), using Lemma~\ref{lem_bounded_secondmoment_04_new}, we also have similar result as described in~\eqref{main_ineq_sgd_new02} and we only need to focus one case, i.e.,  \textbf{Assumptions~\ref{ass_stronglyconvex},~\ref{ass_convex} and ~\ref{ass_smooth} hold}. Moreover, the result described in~\eqref{main_ineq_sgd_new02} can be found in~\cite{NguyenNguyenvanDijkEtAl2018}.


\begin{thm}
\label{theore:SGD_convergence}
Let Assumptions \ref{ass_stronglyconvex}, \ref{ass_convex} and \ref{ass_smooth} hold. For Algorithm \ref{sgd_algorithm} with a stepsize sequence such that 
\begin{itemize}
\item $\eta \leq \frac{1}{2L}$
\item $\eta_t \rightarrow 0$
\item $\frac{d}{dt}\eta_t \leq 0$
\item $\sum_{t=1}^\infty \eta_t \rightarrow \infty$,
\end{itemize}
we have $\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ] \rightarrow 0$. 
\end{thm}

\begin{proof}

As shown in~\eqref{main_ineq_sgd_new02}

$$\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]  \leq (1-\mu \eta_t) \mathbb{E}[ \| w_{t} - w_{*} \|^2 ] + \eta_t^2 N,$$

when $\eta_t \leq \frac{1}{2L}$.

Let $Y_{t+1}=\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]$, $Y_{t}=\mathbb{E}[\| w_{t} - w_{*} \|^2 ]$, $\beta_t= 1 - \mu \eta_t$ and $\gamma_t=\eta^2_tN$. As proved in Lemma~\ref{lemma:hogwild_recursive_form}, if $Y_{t+1} \leq \beta_t Y_t + \gamma_t$, then 
\begin{align*}
Y_{t+1} &\leq \sum_{i=1}^t [\prod_{j=i+1}^t \beta_j] \gamma_i + (\prod_{i=1}^t\beta_i)Y_1\\
&=  \sum_{i=1}^t [\prod_{j=i+1}^t (1 - \mu \eta_j)] \gamma_i + [\prod_{i=1}^t(1 - \mu \eta_i)]\mathbb{E}[\| w_{1} - w_{*} \|^2 ]\\
\end{align*}


Let us define 
\begin{equation}
\label{eq:nj_etaj}
n(j)=\mu \eta_j. 
\end{equation}

Since $1-x \leq \exp(-x)$ for all $x\geq 0$, $$\prod_{j=i+1}^t (1 - \mu \eta_j)\leq \exp(-\sum_{j=i+1}^t(\mu \eta_j))= \exp(-\sum_{j=i+1}^t n(j)).$$ 
Furthermore, since $n(j)$ is decreasing in $j$, we have
$$\sum_{j=i+1}^t n(j) \geq \int_{x=i+1}^{t+1}n(x)dx.$$

With two inequalities above, we have:

\begin{align*}
Y_{t+1} &\leq \sum_{i=1}^t \exp(-\sum_{j=i+1}^t n(j)) n^2(i) N + \exp(-\sum_{j=1}^t n(j)) Y_1 \\
&\leq \sum_{i=1}^t \exp(-\int_{x=i+1}^{t+1}n(x)dx) n^2(i) N + \exp(-\int_{x=1}^{t+1}n(x)dx) Y_1 \\
&=\sum_{i=1}^t \exp(-[M(t+1)-M(i+1)]) n^2(i) N + \exp(-M(t+1)) Y_1,
\end{align*}

where $M(y)=\int_{x=1}^y n(x)dx$ and $\frac{d}{dy}M(y) = n(y)$. We focus on $$F=\sum_{i=1}^t \exp(-[M(t+1)-M(i+1)]) n^2(i).$$

%[TO DO: Given my next remarks -- let me give a slightly different derivation: ]

We notice that
$$F=\exp(-M(t+1)) \sum_{i=1}^t \exp(M(i+1)) n^2(i).$$
We know that $\exp(M(x+1))$ increases and $n^2(x)$ decreases, hence, in the most general case either their product first decreases and then starts to increase or their product keeps on increasing. We first discuss the decreasing and increasing case.
  Let $a(x)=\exp(M(x+1))n^2(x)$ denote this product and let integer $j\geq 1$ be such that $a(1)\geq a(2) \geq \ldots \geq a(j)$ and $a(j)\leq a(j+1)\leq a(j+2)\leq \ldots$ (notice that $j=1$ expresses the situation where $a(i)$ only increases). Function $a(x)$ for $x\geq 1$ is minimized for some value $h$ in $[j,j+1)$. For $2\leq i\leq j$, $a(i)\leq \int_{x=i-1}^{i} a(x) dx$, and for $j+1\leq i$, $a(i)\leq \int_{x=i}^{i+1} a(x) dx$.
 This yields the upper bound 
 \begin{align*}
 \sum_{i=1}^t a(i) &= a(1) + \sum_{i=2}^{j} a(i) + \sum_{i=j+1}^t a(i) \\
 &\leq a(1) + \int_{x=1}^{j} a(x) dx + \int_{x=j+1}^{t+1} a(x) dx, \\
 &\leq a(1) + \int_{x=1}^{t+1} a(x) dx.
 \end{align*}
 The same upper bound holds for the other case as well, i.e., if $a(i)$ is only decreasing.
 We conclude 
 $$F \leq \exp(-M(t+1)) [\exp(M(2))n^2(1) + \int_{x=1}^{j+1} \exp(M(x+1))n^2(x) dx ] .$$
 Combined with
  $$M(x+1)=\int_{y=1}^{x+1}n(y)dy\leq \int_{y=1}^{x}n(y)dy + n(x)=M(x) +n(x) $$
  we obtain
   \begin{align*}
   F &\leq \exp(-M(t+1)) [\exp(M(2))n^2(1) + \int_{x=1}^{t+1} \exp(M(x))n^2(x) exp(n(x)) dx ]\\
   &\leq  \exp(-M(t+1)) [\exp(M(2))n^2(1) + \exp(n(1)) \int_{x=1}^{t+1} \exp(M(x))n^2(x)  dx ].
   \end{align*}
   This gives
   \begin{align*}
Y_{t+1} &\leq  \exp(-M(t+1)) [\exp(M(2))n^2(1) + \exp(n(1)) \int_{x=1}^{t+1} \exp(M(x))n^2(x)  dx ]  N \\
& + \exp(-M(t+1)) Y_1 \\
&=  N \exp(n(1)) C(t+1)  + \exp(-M(t+1)) [\exp(M(2))n^2(1)N  + Y_1], \tagthis \label{eq:Yt_Ct_nt}
\end{align*}
%where the second inequality follows from $M(t+1)\geq M(t)$.
where
$$ C(t) = \exp(-M(t)) \int_{x=1}^{t} \exp(M(x))n^2(x)  dx .$$

 For $y\leq t$, we derive (notice that $n(x)$ is decreasing)
\begin{align*}
C(t) &= \exp(-M(t)) \int_{x=1}^{t} \exp(M(x))n^2(x)  dx \\
&= \exp(-M(t)) \int_{x=1}^{y} \exp(M(x))n^2(x)  dx + \exp(-M(t)) \int_{x=y}^{t} \exp(M(x))n^2(x)  dx \\
&\leq \exp(-M(t)) \int_{x=1}^{y} \exp(M(x))n^2(x)  dx + \exp(-M(t)) \int_{x=y}^{t} \exp(M(x))n(x)n(y)  dx \\
&= \exp(-M(t)) \int_{x=1}^{y} \exp(M(x))n^2(x)  dx + \exp(-M(t))n(y) \int_{x=y}^t \exp(M(x))n(x)dx \\
&= \exp(-M(t)) \int_{x=1}^{y} \exp(M(x))n^2(x)  dx + n(y)[1-exp(-M(t))\exp(M(y))] \\
&\leq \exp(-M(t)) \int_{x=1}^{y} \exp(M(x))n^2(x)  dx + n(y).
\end{align*}

Let $\epsilon>0$. Since $n(y) \rightarrow 0$ as $y\rightarrow \infty$, there exists a $y$ such that $n(y)\leq \epsilon/2$.
Since $M(t)\rightarrow \infty$ as $t\rightarrow \infty$, $exp(-M(t))\rightarrow 0$ as $t\rightarrow \infty$. Hence, there exists a $T$ such that for $t\geq T$,
$exp(-M(t)) \int_{x=1}^{y} \exp(M(x))n^2(x)  dx \leq \epsilon/2$. This implies $C(t)\leq \epsilon$ for $t\geq T$.
This proves $C(t)\rightarrow 0$ as $t\rightarrow \infty$, and we conclude $Y_t\rightarrow 0$ as  $t\rightarrow \infty$.



\end{proof}


\begin{thm}\label{theorem:convergence_rate}
Let Assumptions \ref{ass_stronglyconvex}, \ref{ass_convex} and \ref{ass_smooth} hold. For Algorithm \ref{sgd_algorithm} with a stepsize sequence such that 
\begin{itemize}
\item $\eta \leq \frac{1}{2L}$
\item $\eta_t \rightarrow 0$
\item $\frac{d}{dt}\eta_t \leq 0$
\item $\sum_{t=1}^\infty \eta_t \rightarrow \infty$,
\end{itemize}
$\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]$ is at most 

$$
N\exp(n(1)) 2n(M^{-1}(\ln [ \frac{n(t+1)}{n(1)} ]+ M(t+1)))  + \exp(-M(t+1)) [\exp(M(2))n^2(1)  N  + \mathbb{E}[\| w_{1} - w_{*} \|^2 ]],
$$

where $n(t)=\mu \eta_t$ and $M(t)=\int_{x=1}^t n(x)dx$. 
\end{thm}

\begin{proof}
Now, we are compute the convergence rate of $Y_t=\mathbb{E}[\| w_{t} - w_{*} \|^2 ]$ for a given $M(t)$. We have shown that $C(t) \leq \exp(-M(t)) \int_{x=1}^{y} \exp(M(x))n^2(x)  dx + n(y)$. We are interested in the following problem: finding the largest $y\leq t$ such as 
$$\exp(-M(t))[\int_{x=1}^y \exp(M(x))n^2(x)dx] \leq n(y).$$

The solution is equal to 
$$
y = \sup \{ y\leq t: \exp(-M(t))[\int_{x=1}^y \exp(M(x))n^2(x)dx] \leq n(y) \}.
$$

Since $M(x)$ always decreases, 

\begin{align*}
y &\geq \sup \{ y\leq t: \exp(-M(t))[\int_{x=1}^y \exp(M(x))n(x) n(1) dx] \leq n(y) \}\\
  &= \sup \{ y\leq t: \exp(-M(t))n(1)[\exp(M(y))-\exp(M(1))] \leq n(y) \}\\
  &= \sup \{ y\leq t: \exp(M(y)) \leq \exp(M(1)) + \frac{n(y)}{n(1)} \exp(M(t))\}\\
  &\geq \sup \{ y\leq t: \exp(M(y)) \leq \exp(M(1)) + \frac{n(t)}{n(1)} \exp(M(t))\}\\
 &\geq \sup \{ y\leq t: \exp(M(y)) \leq  \frac{n(t)}{n(1)} \exp(M(t))\}\\  
 &=\sup \{ y\leq t: M(y) \leq  \ln [ \frac{n(t)}{n(1)} ]+ M(t)\}\\
 &= M^{-1}(\ln [ \frac{n(t)}{n(1)} ]+ M(t)),
\end{align*}
where $M^{-1}(t)$ exists for $t\in (0,n(1)]$ (since $M(y)$ strictly increases and maps into $(0,n(1)]$ for $y\geq 1$).

Therefore, $$C(t) \leq 2n(M^{-1}(\ln [ \frac{n(t)}{n(1)} ]+ M(t)))$$
and 
$$
Y_{t+1} \leq N \exp(n(1)) 2n(M^{-1}(\ln [ \frac{n(t+1)}{n(1)} ]+ M(t+1)))  + \exp(-M(t+1)) [\exp(M(2))n^2(1) N + Y_1].
$$

[TO DO: show that this bound is not very good for $n(t)=1/t$, although the bound does show the behavior of $n(t)$ is followed by $Y_t$ with some ``delay''.]
\end{proof}

\begin{lem}
\label{lem:smaller_Stepsize}
With given stepsizes $\eta_t\leq 1/t \ln^k t$,  $\mathbb{E}[\| w_{t} - w_{*} \|^2 ]$ does not converge to $0$ for any given $k>1$. 
\end{lem}
\begin{proof}
As shown in~\eqref{eq:Yt_Ct_nt}, we have 
$$
\mathbb{E}[\| w_{t} - w_{*} \|^2 ] \leq A C(t) + B \exp(-M(t)),  
$$

where $A= N \exp(n(1))$ and $B=\exp(M(2))n^2(1)N  + \mathbb{E}[\| w_{1} - w_{*} \|^2 ]$. 
We need $\sum^{\infty}_{t=1} n(t)= \mu( \sum^{\infty}_{t=1} \eta_t)$ is infinite to make $\exp(-M(t))$ converges to $0$. But the convergence of $\sum^{\infty}_{t=1} \eta_t= \sum^{\infty}_{t=e} 1/t \ln^k t$ and  $\int_{t=e}^\infty (1/t \ln^k t) dt$ are relative. We compute $\int_{t=e}^{\infty} (1/t \ln^k t) dt$ using substitution technique, i.e., $u=\ln t$, we have $du/dt = 1/t$ and $t=e^u$. Thus, $$\int_{t=e}^{\infty} (1/t \ln^k t) dt = \int_{t=1}^{\infty} u^{-k} du = -u^{-k+1}/(k-1)\big|_{1}^{\infty}= \frac{1}{k-1}<\infty.$$ 
\end{proof}

The Lemma~\ref{lem:smaller_Stepsize} tells us important following fact: \textbf{we cannot have stepsize smaller than $\frac{1}{t\ln t}$}.


\begin{lem}
\label{lem:Ct}
For given 
\begin{equation}
\label{eq:Ct}
C(t) = \exp(-M(t)) \int_{x=1}^t \exp(M(x)) n^2(x)dx,
\end{equation}

where $\frac{d}{dx}M(x)=n(x)$ and the function $n(x)$ satisfies the following conditions:

\begin{enumerate}
\item $\frac{d}{dx}n(x) < 0$,
\item $\frac{d}{dx}n(x)$ is continuous.
\end{enumerate}

Then, there is a moment $T$ such as for all $t>T$, $C(t)>n(t)$.
\end{lem}

\begin{proof}
% BG

We take the derivative of $C(t)$, i.e., 
\begin{align*}
\frac{d}{dt}C(t) &= - \exp(-M(t)) n(t) \int_{x=1}^t \exp(M(x)) n^2(x)dx + \exp(-M(t)) \exp(M(t)) n^2(t)\\
&=n(t) [ n(t) - C(t) ] \\
\end{align*}
This shows that
$$ C(t) \mbox{ is decreasing if and only if } C(t)>n(t).$$

Initially $C(1)=0$ and $n(1)>0$, hence, $C(t)$ starts increasing from $t\geq 1$. Since $n(t)$ decreases for all $t\geq 1$, we know that there must exist a first cross over point $x$:
\begin{itemize}
\item There exists a value $x$ such that $C(t)$ increases for $1\leq t<x$, and
\item $C(x)=n(x)$ with derivative $d C(t)/dt |_{t=x} =0$.
\end{itemize}

Since $n(x)$ has a derivative $<0$, we know that $C(t)>n(t)$ immediately after $x$.
Suppose that $C(y)=n(y)$ for some $y>x$ with $C(t)>n(t)$ for $x<t<y$.
This implies that $d C(t)/dt |_{t=y} =0$ and since $d C(t)/dt$ is continuous 
$$ C(y-\epsilon) = C(y) + O(\epsilon^2).$$
Also,
$$ n(y-\epsilon) = n(y) - \epsilon d n(t)/dt |_{t=y} + O(\epsilon^2).$$
Since $d n(t)/dt |_{t=y}<0$, we know that there exists an $\epsilon$ small enough (close to 0) such that
$$ C(y-\epsilon) < n(y-\epsilon).$$
This contradicts $C(t)>n(t)$ for $x<t<y$. We conclude that there does not exist a $y>x$ such that $C(y)=n(y)$:
\begin{itemize}
\item For $t>x$, $C(t)>n(t)$ and $C(t)$ is strictly decreasing.
\end{itemize}

\textbf{Conclusion.} For any given $n(t)$, there exists a time $T$ such that $C(t)<n(t)$ for all $t \in [1,T)$, $C(T)=n(T)$ and then $C(t)>n(t)$ when $t\in (T,\infty]$. Note that $C(t)$ is always bigger then zero. As proved above, $C(t)$ always decreases after $T$ and thus, $C(t)$ converges to zero when $t$ goes to infinity.  
\end{proof}
 
We want to highlight the following note: As shown in~\eqref{eq:Yt_Ct_nt}, we have 
$$
\mathbb{E}[\| w_{t} - w_{*} \|^2 ] \leq A C(t) + B \exp(-M(t)).  
$$ 
Now Lemma~\ref{lem:Ct} tells us $C(t)\rightarrow 0$ when $t\rightarrow \infty$. Moreover $\exp(-M(t)) \rightarrow 0$ when $t\rightarrow \infty$ because $\sum_{t=1}^\infty n(t) \rightarrow \infty$. Based on two these results, we conclude that $\mathbb{E}[\| w_{t} - w_{*} \|^2 ] \rightarrow 0$ when $t\rightarrow \infty$. This is alternative proof for the convergence of SGD as shown in Theorem~\ref{theore:SGD_convergence}.    
 
 
 
\begin{thm}
\label{theorem:fastest_convergence}
Among all stepsizes $\eta_{q,t}=1/(K+t)^q$ where $q>0$, $K$ is a constant such that $\eta_{q,t}\leq \frac{1}{2L}$, with the stepsize $\eta_{1,t}=1/(2L+t)$, SGD algorithm enjoys the fastest convergence.  
\end{thm} 
 
\begin{proof}
Since in~\eqref{eq:Yt_Ct_nt}, we have 
$$
\mathbb{E}[\| w_{t} - w_{*} \|^2 ] \leq A C(t) + B \exp(-M(t)),  
$$

where $A= N \exp(n(1))$ and $B=\exp(M(2))n^2(1)N  + \mathbb{E}[\| w_{1} - w_{*} \|^2 ]$. Let us denote $C_q(t)=C(t),n_q(t)=\mu/(K+t)^q$ when $\eta_{q,t}=1/(K+t)^q$. It is obvious that $n_{q}(t)>n_1(t)$ for all $t$ and $q<1$. It implies for any $n_q(t)$ with $q<1$, we have $$\exp(-M(t))<\exp(-\int_{x=1}^t\mu 1/(K+x)dx)<\exp(-\int_{x=1}^t\mu 1/x dx) < 1/t.$$

Therefore, we always have $\exp(-M(t))<1/t=n_1(t)<n_q(t)<C_q(t)$. Now, we consider the following cases. We are finding $n(t)$ such as $n(t) = C(t)/2$. We rewrite it as 

$$ 
C(t) = \exp(-M(t)) \int_{x=1}^t \exp(M(x)) n^2(x) dx = 2 n(t)
$$

Taking derivatives of both sides, we have:

$$
-n^2 = n(n-2n) = n(n-C) = \frac{d}{dt}C = 2 \frac{d}{dt}n
$$ 

This is solved for $1/(at): -1/(a^2 t^2) = -2/(at^2)$ Hence, $a=1/2$ and $n(t)=2/t$. It means, $C_q(t)>C_1(t)$ and thus, the stepsize $\eta_{1,t}=1/(K+t)$ enjoys the fastest convergence. 

%Note that, in Lemma~\ref{lem:smaller_Stepsize}, there is no stepsize smaller than $1/t\ln t$. It shows that stepsize $1/(2L+t)$ is the most optimal one. 
\end{proof} 
 


\subsection{Convergence with Oracle}
\label{subsec:convergence_oracle}

Assume there exists an oracle which can give $\mathbb{E}[\| w_{t} - w_{*} \|^2 ] $ for choosing a stepsize $\eta_t$. As shown in \eqref{main_ineq_sgd_new02}, we have

$$
\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]  \leq (1-\mu \eta_t) \mathbb{E}[ \| w_{t} - w_{*} \|^2 ] + \eta_t^2 N. 
$$

If we define $n(t)=\mu\eta_t$, then we obtain

\begin{align*}
\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]  &\leq (1-n(t)) \mathbb{E}[ \| w_{t} - w_{*} \|^2 ] + n^2(t)\frac{N}{\mu^2}. \tagthis \label{eq:Ent2}
\end{align*}


Given $\mathbb{E}[\| w_{t} - w_{*} \|^2 ]$ from oracle, we want to minimize $(1-n(t)) \mathbb{E}[ \| w_{t} - w_{*} \|^2 ] + n^2(t)\frac{N}{\mu^2}$ by taking derivative wrt $n(t)$, i.e., $
-\mathbb{E}[ \| w_{t} - w_{*} \|^2 ] + 2n(t)\frac{N}{\mu^2} = 0$ or $n(t)=\frac{\mathbb{E}[ \| w_{t} - w_{*} \|^2 ] \mu^2}{2N}$. By substituting $n(t)=\frac{\mathbb{E}[ \| w_{t} - w_{*} \|^2 ] \mu^2}{2N}$ in \eqref{eq:Ent2}, it yields:

$$
\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]  \leq \mathbb{E}[\| w_{t} - w_{*} \|^2 ]  -  (\mathbb{E}[\| w_{t} - w_{*} \|^2 ])^2/c, 
$$
where $c= \frac{4N}{\mu^2}$. Let us $Y_t=\mathbb{E}[\| w_{t} - w_{*} \|^2 ] /c$, then we have

\begin{align*}
Y_{t+1} \leq Y_t(1-Y_t). 
\end{align*}	

Let $u_t=\frac{1}{Y_t}$ and then 
\begin{align*}
u_{t+1} &\geq \frac{1}{Y_t(1-Y_t)}= \frac{u_t}{1-1/u_t}= u_t + \frac{1}{u_t-1} +1.  
\end{align*}

Hence, $u_{t+1}\geq t+u_1+\sum_{i=1}^t\frac{1}{u_i-1}$, here we assume $u_1>1$. Actually, we can stop at $u_j$ such as $u_j>1$ for a certain $1\leq j \leq t$. From the formula above, we can see that $j$ should be less than 3. Now, we can say that $u_{t+1} \geq t+1$. In other words, $Y_{t+1}=\frac{1}{u_{t+1}}\leq \frac{1}{t+1}$, or 

$$
\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]  \leq \frac{4N}{\mu^2}\frac{1}{t+1}. 
$$

\textbf{Conclusion.} If we cannot improve our bounding strategy, then we can only prove that oracle access to $\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ] $ does not help in that the optimal solution without oracle access leads to the same convergence in expectation. This implies that if heuristic evaluations with oracle access to $\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]$ improve the $1/t$ convergence result, then a better proof strategy likely exists. If not, then the bounds in our paper are tight.



==> sections/BBB.tex <==
\section{AAA}
Let $n_0(x) = n(x)$ and define recursively 
$$
n_{k+1}(x) = \frac{-1}{n(x)} \frac{d n_k(x)}{dx} .
$$

Then,


$$
C(t) = \sum_{k=0}^K  n_k(t)  - e^{-M(t)}e^{M(1)} \sum_{k=0}^K  n_k(1) - e^{-M(t)} \int_{x=1}^t e^{M(x)} \frac{d n_K(x)}{dx} dx
$$

The case $K=0$ is shown above. Induction follows from

\begin{align*}
u &= e^{M(x)} n(x) \text{ with } U = e^{M(x)} \\
V &= n_{K+1}(x) \text{ with } v = \frac{d n_{K+1}(x)}{dx}
\end{align*}


%Seems this sequence  converges for $n_{k+1}(x)/n_k(x) \rightarrow 0$ for $x \rightarrow \infty$ [have not thought this through].
%
%
%Suppose $n(t) = \frac{1}{t \ln t}$, then
%
%$$
%n_1(t) = [ \frac{-1}{(t \ln t)^2}] * (1 + ln t ) *(t ln t) =  \frac{-(1+ln t)}{t \ln t} \approx -1/t.
%$$
%
%\textcolor{red}{
%It is evident that $n_1(t)/n_0(t)= -(1+ln(t))$ does not converge to $0$ and it contradicts Marten's thought, i.e., for $n_{k+1}(x)/n_k(x) \rightarrow 0$ for $x \rightarrow \infty$. Moreover, what exactly we can have from this derivation???}


\section{BBB}
\label{sec:BBB}

We consider a multivariate normal distribution of a $k$-dimensional random vector $\xi$, i.e., $\xi \sim \mathcal{N}(m,\Sigma)$, where $m=\mathrm{E}[\xi]$ and $\Sigma = \mathrm{E}[(\xi-m)(\xi-m)^{\mathrm{T}}]$. The density function of $\xi$ is
$$
g(\xi) = \frac{\exp( \frac{- (\xi-m)^\mathrm{T}\Sigma^{-1}(\xi-m)}{2} )}{\sqrt{(2\pi)^k|\Sigma|}}. 
$$

Let us consider the following simple example $$f(w;\xi)=\frac{\|w-\xi\|^2}{2},$$
and $$F(w) = \frac{\mathrm{E}_{\xi}[\|w-\xi\|^2]}{2}.$$


Since
$$\nabla_w [ \|w-\xi\|^2 ] = \nabla_w [ \langle w,w \rangle - 2\langle w,\xi \rangle + \langle \xi,\xi \rangle ] = 2w -2 \xi = 2(w-\xi), 
$$
we have $$ \nabla_w f(w;\xi)= w-\xi. $$

Moreover, $f(w;\xi)$ is $L$-smooth with $L=1$ due to the fact that $\|\nabla_w f(w;\xi)-\nabla_{w'} f(w';\xi) \|=\|w-\xi-(w'-\xi) \|=\|w-w'\|$.  

Notice that
\begin{enumerate}
\item $\|w-\xi\|^2 = \|(w-m)+(m-\xi)\|^2= \|w-m\|^2 + 2 \langle w-m,m-\xi \rangle + \|m-\xi \|^2$. 
\item Since $m=\mathrm{E}[ \xi ]$, we have $\mathrm{E}[ m-\xi ] =0$.
\item   $\mathrm{E}[ \|m-\xi\|^2 ]=\sum_{i=1}^k \mathrm{E}[ (m_i-\xi_i)^2 ] = \sum_{i=1}^k \Sigma_{i,i} = \mathrm{Tr}(\Sigma)$. 
\end{enumerate}

Therefore, $F(w) = \mathrm{E}_{\xi}[ \|w-\xi\|^2 ] = \frac{\|w-m\|^2}{2} + \frac{\mathrm{Tr}(\Sigma)}{2}$, and this shows $F$ is strongly convex, smooth, and has minimum $w^* = m$. Therefore, 
\begin{align*}
F(w) - F(w') &= \frac{\|w-m\|^2 - \|w'-m\|^2}{2} \\
&= \frac{<w,w> - 2<w, m> - <w',w'> + 2<w',m>}{2} \\
&= \frac{-2<m, w-w'> +2 <w', w-w'> - 2<w', w-w'> + <w,w> - <w',w'>}{2} \\
&= < w'-m , w-w' > + \frac{1}{2}[<w,w> - 2<w',w> + <w',w'>]\\
&= < \nabla F(w') , w-w' > + \frac{1}{2} \|w-w'\|^2.
\end{align*}
This means $F$ is $\mu$-strongly convex function with $\mu=1$. 




 Notice that in our notation $N=2 \mathrm{E}_\xi[\|\nabla f(w^*;\xi) \|^2]=2 \mathrm{E}_{\xi}[\|w^* -\xi \|^2]= 2 \mathrm{E}[ \nabla_\xi [ \|m-\xi\|^2 ] ]=2\mathrm{Tr}(\Sigma)$. 
 
We have:
$$
w_{t+1} = w_t - \eta_t \nabla f(w_t;\xi_t) = w_t - \eta_t (w_t - \xi_t) = (1-\eta_t) w_t + \eta_t \xi_t. 
$$

%What is the expectation over $\xi_t$? (We know that $\mathrm{E}[ \xi_t ] = m = w^*$.) 
%
%$$
%\mathrm{E}[ w_{t+1} | \mathcal{F}_t ] = (1-\eta_t) w_t +  \eta_t w^*.
%$$
%
%This in itself already indicates that we get fast convergence to $w^*$ in expectation. But we do need to be precise:

$$
\mathrm{E}[ \|w_{t+1}-w^*\|^2 | \mathcal{F}_t ]
=\mathrm{E}[ \|(1-\eta_t) (w_t -w^*) + \eta_t (\xi_t - w^*) \|^2 | \mathcal{F}_t ]
$$
which is equal to 
$$
(1-\eta_t)^2 \|w_t -w^*\|^2 + 2\eta_t (1-\eta_t ) <w_t-w^*, \mathrm{E}[\xi_t - w^*]> +  \eta_t^2 \mathrm{E}[ \|\xi_t -w*\|^2]. 
$$

Again notice that $\mathrm{E}[\xi_t -w^*] = 0$ and $\mathrm{E}[ \| \xi_t - w^* \|^2 ] = \mathrm{Tr}(\Sigma)$. So,

$$
\mathrm{E}\|w_{t+1}-w^*\|^2 | \mathcal{F}_t ]= (1-\eta_t)^2 \|w_t -w^*\|^2 +  \eta_t^2 \frac{N}{2}.
$$

%Notice that in our notation $N = 2 \mathrm{E} [ \| \nabla[ \|w*-xi\|^2 ] \|^2 ] = 2 \mathrm{E} [ 4 \|w^*-\xi\|^2 ] = 8k$. So, we get $4k = \frac{N}{2}$ in the above equation. Also 

Notice that $L=1$ in our example. Also, 
$$(1-\eta_t)^2 = (1- 2\eta_t + \eta_t^2).$$


for $\mu = 1$. We get:

$$
\mathrm{E}\|w_{t+1}-w^*\|^2 | \mathcal{F}_t ]=(1- \mu\eta_t(2-\eta_t)) \|w_t -w^*\|^2 + \frac{N}{2} \eta_t^2.
$$

This is very close to Equation~\ref{main_ineq_sgd_new02}, i.e., 
 
$$
\mathrm{E}\|w_{t+1}-w^*\|^2 | \mathcal{F}_t ]\leq (1- \mu\eta_t) \|w_t -w^*\|^2 +  N \eta_t^2.
$$

Let denote $Y_t=\mathrm{E}\|w_{t}-w^*\|^2]$. From the equation above, we have
$$
Y_{t+1}=(1-\eta_t)^2 Y_t + \frac{N}{2} \eta_t^2.
$$

From here, we can derive 

$$
Y_{t+1} = \sum_{i=1}^t[\prod_{j=i+1}^t (1-\eta_j)^2]\frac{N}{2}\eta_i^2+[\prod_{j=1}^t(1-\eta_j)^2]Y_1,
$$

where $Y_1=\mathrm{E}[\|w_0-w^*\|^2]$. 


Now, we consider the following functions:  $\exp(-bx)$ and $1-x$ where $b>0$. Let $0<h<1$, is the place where two functions crosses each other, then $\exp(-bh)=1-h$. From here, we have $b=-\frac{\ln(1-h)}{h}$.

Let $2\eta_1 -\eta_1^2 = h $. When $\eta_j<1$, we have $2\eta_j -\eta_j^2 $ decreasing beause $(2\eta_j -\eta_j^2)'= 2\eta'_j - 2\eta'_j\eta_j=2\eta'_j(1-\eta_j) \leq 0$. It implies $2\eta_j -\eta_j^2\leq h$. 

For any $0<x\leq h$, we have $\exp(-bx)\leq 1-x$. Now, we can compute the lower bound of $Y_{t+1}$ as follows.

\begin{align*}
Y_{t+1} &\geq \sum_{i=1}^t[\prod_{j=i+1}^t \exp(-b[2\eta_j-\eta_j^2])]\frac{N}{2}\eta_i^2+[\prod_{j=1}^t\exp(-b[2\eta_j-\eta_j^2])]Y_1 \\
&\geq \sum_{i=1}^t\exp(-b\sum_{j=i+1}^t[2n(j)-n^2(j)])n^2(i)\frac{N}{2} + \exp(-b\sum_{j=1}^t[2n(j)-n^2(j)])\\
&\geq \sum_{i=1}^t\exp(-2b\sum_{j=i+1}^t n(j))n^2(i)\frac{N}{2} + \exp(-2b\sum_{j=1}^tn(j))
\end{align*}

We have the following inequality
$$
  \sum_{j=i+1}^t n(j) \leq \int_{x=i}^t n(x)dx = M(t)-M(i).
$$

Hence, 
\begin{align*}
Y_{t+1} &\geq \sum_{i=1}^t\exp(-2b[ M(t)-M(i)])n^2(i)\frac{N}{2} + \exp(-2b[ M(t)-M(0)])Y_1\\
&\geq \exp(-2bM(t)) \int_{x=1}^t \exp(2bM(x))n^2(x)dx\frac{N}{2} + \exp(-2b[M(t)-M(0)])Y_1\\
&\geq C_b(t)\frac{N}{2} + \exp(-2bM(t))\exp(2bM(0))Y_1,
\end{align*}
where 
$$
C_b(t) = \exp(-2bM(t)) \int_{x=1}^t \exp(2bM(x))n^2(x)dx. 
$$

If we denote $\bar{n}(x)=2bn(x)$ and $\bar{M}(x)=2bM(x)$, then 

$$
C_b(t) = \frac{C(t)}{4b^2},
$$
with $\bar{n}(x)$. 

Note that, from Equation~\ref{eq:Yt_Ct_nt}, we have
$$
 C(t) = \exp(-M(t)) \int_{x=1}^{t} \exp(M(x))n^2(x)  dx.
$$

%We just miss a factor 2 in the last term (I may even made a calculation mistake) -- but this does not affect the behavior of the convergence rate for small or large t. Also the $-4\eta_t$ in the first term becomes very small. So, this function meets  our conditions pretty much with equality: we now need to just precisely calculate how this function behaves in a precise way. 
%
%$$
%Y_{t+1} = \mathrm{E} [\|w_{t+1} -w^* \|^2 ]. 
%$$
%
%Then,
%
%$$
%Y_{t+1} = (1-(\mu - 4 \eta_t) \eta_t)  Y_t + \eta_t^2 \frac{N}{2}. 
%$$
%
%Let's solve this precisely and compare with the analysis we did for the bound. They should pretty much match.  This would prove that our bounds are tight and solves the problem of Martin ! We can also use this example to find out what happens for larger stepsize etc. This we need to discuss as well for the current asymptotic analysis.
%The paper is improving !
%
%If you agree with the analysis, we can send it to Lam and Martin. I think we are on the right track, we actually can prove tight bounds here. We should also generalize for arbitrary positive definite symmetric co-variance matrix $\Sigma$. This will allow us to manipulate $N$. And as a consequence show how the step size should be chosen in relation to $N$ for small $t$. Cool, I think we are going to nail this problem this Friday. 
%
%If indeed correct, then we may actually see that for this worst-case example the choice $\frac{1}{t}$ is best for large but also small $t$ unless $\frac{Y_1}{N}$ is really large (so, the trace of Sigma is very small). 
%
%The question is "Does the value of $\frac{Y_1}{N}$ explain the experiments?" I expect the answer is no. In fact, I expect that the ratio $\frac{Y_1}{N}$ indicates the initial step size we should start with -- so, may be the explanation is a different one:
%
%
%1) If we choose $w_0$ at random given an a-priori distribution on $w^*$, then we can calculate $Y_1$. E.g., $w^*$ is itself again normal distributed with some mean and $\Sigma'$. Of course we choose $w_0$ to be this mean. But now we have an expected initial distance from $w^*$ and if the traces of $\Sigma'$ and $\Sigma$ are related in some way, then we can calculate $\frac{Y_1}{N}$ and precisely calculate the best diminishing stepsizes -- I expect again $\frac{1}{t}$ but with a different initial stepsize. We can definitely add this type of calculation.
%
%
%2) Or: For more specific other data sets, it may be better to start off with $\frac{1}{\sqrt{t}}$ -- this is what experiments and literature seem to confirm. So, there may be another parameter -- related to another assumption -- with which we can improve the bound showing that $\frac{1}{t^q}$ is preferable for some $q<1$.
%
%Tomorrow, we need to study the bounding technique of our part of the proof: $1-x\leq \exp(-x)$ is pretty tight, if we know that $x\leq h$, then for $b$ such that
%
%$\exp(-bh) = 1-h$, i.e., $b = - \frac{\ln(1-h)}{h}$. 
%
%We have $\exp(-bx) \leq 1-x$ and this can be used to lower bound the convergence rate for our worst-case example and show how Equation~\ref{eq:Yt_Ct_nt} is tight up to a multiplicative factor. Beyond Equation~\ref{eq:Yt_Ct_nt}  we need to discuss whether the bounding technique is tight enough:
%
%
%= We should add the recurrence for $C(t)$ into the draft and use it to get an expression of $C(t)$ as a function of $q$. Now we will have a nice expression for Equation~\ref{eq:Yt_Ct_nt}  and we can find the optimal $q$ as a function of $\frac{Y_1}{N}$.
%
%= We should also further analyse $\frac{Y_1}{N}$: We do not know what its value is equal to. However, with a a-priori distribution on $w^*$ we will be able to find its expected value ... Another more practical way is to use an exponentially decreasing stepsize to begin with as this allows us to obtain fast convergence on very large $\frac{Y_1}{N}$, i.e., this would cover highly unlikely training data sets.
%
%We can use our other strong convergence result: 
%
%We take a small set of samples (something like $\kappa$ as far as I remember) and apply full gradient.
%
%Now we use this computation to get an estimate of $w^*$ which will be our initial $w_0$ for SGD, and we can estimate $Y_1$ and $N$. Now we use the best $n(t)$ as predicted by Equation~\ref{eq:Yt_Ct_nt}.

\section{CCC}
\label{sec:CCC}

As a follow-up, let me try to figure out the value of $W$:


$Y_t = \mathrm{E}[ \|w_t-w^*\|^2 ]$


$Y_{t+1} \leq (1 - \mu \eta_t)Y_t + \eta_t^2 N$


We want to prove by induction:


$Y_t \leq Z_t$


Basis: $Z_1=Y_1$


Let us define 
\begin{equation}
\label{eq:zz}
Z_{t+1} = (1 - \mu \eta_t)Z_t + \eta_t^2 N.
\end{equation}

We have the following induction:

\begin{align*}
Y_{t+1} &\leq (1 - \mu \eta_t)Y_t + \eta_t^2 N \\
&\leq (1 - \mu \eta_t)Z_t + \eta_t^2 N \\
&= Z_{t+1}.
\end{align*}

We want to minimize $Z_t$ given the following requirement: $\eta_t \leq 1/(2L)$. 
Let's take the derivative of Equation~\ref{eq:zz} with respect to $\eta_t$:
$- \mu Z_t + 2 N \eta_t =0$ gives $\eta_t = \mu Z_t /(2N)$

So, we need to set
$$
\eta_t = \text{min} \{ 1/(2L) , \mu Z_t/(2N)\}.
$$

That is, $\eta_t = 1/(2L)$ if $Z_t \geq N/(\mu L)$, and $\eta_t = \mu Z_t/(2N)$ otherwise.

So, initially:
$$
Z_{t+1} = (1 - \mu /(2L))Z_t +  N  /(4L^2) \text{ with } Z_1=Y_1.
$$

So, 
$$
Z_t = (1-\mu/(2L))^{t-1} Y_1 + \sum_{i=0}^{t-2} (1-\mu/(2L))^i N/(4L^2).
$$

Hence,
\begin{align*}
Z_t &=  (1-\mu/(2L))^{t-1} Y_1 +  [N/(4L^2)] [1-(1-\mu/(2L)^{t-1}]/[\mu/(2L)]\\
&= N/(2 \mu L) + (1-\mu/(2L))^{t-1} (Y_1 - N/(2 \mu L) ). 
\end{align*}

So, $Z_t \geq N/(\mu L)$ if and only if

$$
(1-\mu/(2L))^{t-1} (Y_1 - N/(2 \mu L) ) \geq N/(2 \mu L)
$$

That is

$$
(t-1) \ln( 1- \mu/(2L)) \geq - \ln( 2 \mu L Y_1/N  - 1)
$$

or
$$
t \leq 1 +  [\ln( 2 \mu L Y_1/N  - 1)]/[\ln( (1- \mu/(2L))^{-1}  )] = T
$$

So for $W = \lceil T \rceil$ we have $Z_W \leq N/(\mu L)$. For $t\geq W$ the recurrence relation becomes

$$
Z_{t+1} = (1 - \mu \eta_t)Z_t + \eta_t^2 N  
$$
with $\eta_t = \mu Z_t/(2N)$ and $Z_W <= N/(\mu L)$. 


We have

$$
Z_{t+1} = Z_t - \mu^2 Z_t^2 /(2N) + \mu^2 Z_t^2 /(4N) = Z_t - \mu^2 Z_t^2 /(4N)
$$

We define $Q_t = \mu^2 Z_t /(4N)$. This gives $Q_{t+1} = Q_t - Q_t^2$  with $Q_W \leq mu/(4L)$. Now we use $U_t = 1/Q_t$ and we continue:
$$
U_{t+1} = U_t + 1/(U_t-1) +1
$$

giving

$$
U_{t+1} = (t+1-W) + U_W + \sum_{i=W}^t 1/(U_i-1).
$$

This shows $U_{t+1} \geq (t+1-W) + U_W$. Hence, $\sum_{i=W}^t 1/(U_i-1) \geq \sum_{i=0}^{t-W} 1/(i+U_W)$. Which is approximately equal to $\ln(t+1-W+U_W) - \ln(U_W)$.  This proves

$$
U_{t+1} \geq (t+1-W) + U_W + \ln(t+1-W+U_W) - \ln(U_W). 
$$

I.e.,
$$
U_t >= t-W+U_W +  \ln(t-W+U_W) - \ln(U_W).
$$

This gives, $U_W>= 4L/\mu$

$$
Q_t <= 1/[ t-W+4L/\mu + \ln(t-W+4L/\mu) - ln(4L/\mu) ]
$$

We have $\eta_t = \mu Z_t/(2N) = 2 Q_t/\mu$, so 
$$
\eta_t = (2/\mu) /[ t-W+4L/\mu + \ln(t-W+4L/\mu) - \ln(4L/\mu) ].
$$

is the right choice leading to 
$
Z_t \leq (2N/\mu) \eta_t. 
$

Actually, the convergence rate improvement is not too much less if we simply use
$\eta_t = (2/\mu) /[ t-W+4L/\mu ]$ for $t\geq W$. And this fits how we think of the best step size.

The analysis above shows that ideally we have the largest possible step size $1/(2L)$ for an initial period till $t=W$.

\section{DDD}
\label{sec:DDD}

An interesting generalization of the tightness example. Consider a multivariate polynomial $f(w;\xi)$ with the property that $f(w;\xi)$ is a sum of terms of the form
$q(w-m) \prod_i (m_i-\xi_i)^{r_i}$ where $q(y)$ is a multivariate polynomial with terms $C \times \prod y_i^{s_i}$ where all $s_i$ are even and coefficient $C>0$.
In the above formula $m$ is again the mean of the considered multivariate normal distribution with co-variance matrix $\Sigma$. We assume $\Sigma\geq 0$.
Now consider $F(w) = \mathrm{E}[ f(w,\xi) ]$. Consider a term:
$q(w-m) \prod_i (m_i-\xi_i)^{r_i}$. Notice that

$\mathrm{E}[ \prod_i (m_i-x_i)^{r_i} ]$ = { see wikipedia page on multivariate normal distribution}
\begin{itemize}
\item $0$ if $k=\sum_i r_i$ is odd.
\item Suppose $k$ is even: Then the central $k$-th order moments are equal to $\sum (c_{i,j} c_{k,l} . . . c_{x,z})$. The sum is taken over all different permutations of the $k$ indices, where it is noted that covariance $c_{i,j} = c_{j,i}$. That is, all permutations of the string $1^{r_1}2^{r_2}...d^{r_d}$ (which has length $k=\sum r_i$), where $d$ is the dimension/length of the vectors $x$ and $m$.
\end{itemize}

This shows us how to calculate $F(w)$, which can now become a rather arbitrary complex function.  The co-variance matrix is assumed to be larger than $0$, and $q(y)$ has only 'quadratic' terms with positive coefficients. This implies $q(w-m) \prod_i (m_i-\xi_i)^{r_i} \geq 0$ for all $w$. Hence, $F(w)$ has minimum $w^*=m$. Also $F(w)$ is strongly convex but with what parameter? The $f(w;xi)$ can be non-convex ... what is their smoothness? Can this lead to a large $W$? 

It would be nicer to start with functions $f(w;\xi)=p(w-\xi)$ and write $p(w-\xi)=p(w-m + m-\xi)$ and consider this as a polynomial $q(w-m, m-\xi)$ and assume some conditions around the coefficients of $p$ and its terms. This makes the $f$ independent of $m$ and we may get more practical possibilities. But now i cannot say much about when $w^*=m$ ... Anyway there may be some degrees of freedom we can play with. We can also think of for example: $f(w;\xi) =  s(\xi) \times \|w-\xi\|^2$ where $s(\xi)$ draws something uniform from interval $[a,b]$. Now we know $F(w) = \mathrm{E}_\xi [s(\xi) \times \|w-\xi\|^2 ] = \mathrm{E}_{u,\xi} [ u \times \|w-\xi\|^2]$ where $u \leftarrow [a,b]$ uniform. And we conclude $F(w) = (a+b) \times ( \|w-m\|^2 /2 + \mathrm{Tr}(\Sigma)/2 )$. So, $\mu = a+b$, while the individual $f(w;\xi)$ have strong convexity and smoothness equal to $s(\xi)$.


In stead of a uniform distribution, we can have an exponentially decreasing function with parameter $\mu$ (so drawing $u$ has probability density $\exp(-\mu u)/\mu$.
Now we have strong convexity $\mu$.  


Each component function can have a very large smoothness (unbounded in the infinite case). But in practice for a finite set of epochs etc., we would be able to show that with large probability the data set has a bounded $L$. Actually we can see that the maximum of exponential distributions $\leq L$ has probability like $(1-\exp(-mu L)^t$ where $t$ is the number of component functions considered during SGD up to moment $t$.

So bound $L$ should be something like $t \times \exp(-\mu L)$ is small of the order $L= \ln(t)/\mu$. 


Now this starts to look like a promising example with large $W$. Of course 'in practice' one would throw out all $s(\xi)$ that are to large (as these have large smoothness and deviate from finding $w^*$). And this would allow us to bound $L$ to something much smaller. 


This leads to a general question: What if SGD simply throws out all component functions with $L$ 'too large' (making $L\leq \text{constant} \times \mu$), when would this work?


In the above calculation: $N = \mu \times \mathrm{Tr}(\Sigma)$. $Y_1= \mathrm{E}[ \|\text{ minimum of } f(w;\xi) - w^*\|^2] = \mathrm{Tr}(\Sigma)$.

We get $Y_1/N = 1/\mu$.  $W = 1 + (2L/\mu) \ln( 2 \mu L Y_1/N  - 1) = 1 + 2 ( \ln(t) / \mu^2) \ln( 2 \ln(t) /\mu -1)$ this is going to be $> t$ for $\mu < 1/ \sqrt{t}$ 
which is true if $\mu = \mathcal{O}(1/n)$ and maximum $t$ is say 100 epochs times $n$ ...


So, we would have a 'constant' stepsize $1/2L = \mu/(2 \ln(t))$ ....  ($L$ is a function of $t$, probably something like $L = (20+\ln(t))/\mu$ is more appropriate. We could experiment ....). The above shows that there are artificial tight constructions with large $W$ ...


May be we can generalize to other exponential like distributions: May be a truncated (at $L$) exponential distribution.


Or $s(\xi)$ is taken from $[0,b]$ with mean $\mu$ in the following way:

$s(\xi)$ = uniform in $[0,b_0]$ with probability $1-p$ and uniform in $[0,b_1]$ with probability $p$. Its mean is $(1-p)\times b_0/2 + p\times b_1/2 = \mu$ and $b_0<b_1=L$. For example, $p=\mu/L$ and $b_0=\mu/(1-\mu/L)$. Now we can get any combination $(\mu,L)$ of our choice. We still have $Y_1/N=1/(2\mu)$ or something and
$$
W = 1 + (2L/\mu) \ln( 2 \mu L Y_1/N  - 1) = 1 + (2L/\mu) \ln(L-1).
$$

So for $L=1+\exp(c)$ with $0<c<1$ we have $W$ is at most $2 \exp(c)/\mu$ and we get a nice variation among the $W$. Ok, so in theory we can have our optimized solution with $W>1$. I guess I may have been wrong and the lower bound on the white board is not that coarse: We can have $N = \mu \mathrm{Tr}(\Sigma)$. Our lower bound introduces $\mu^2$ .. this is no good -- can we get a better bound? Or can we simply assume 
$N \geq \mu \mathrm{E}[ \|w^*_\xi-w^*\|^2 ]$ and show that this makes sense?
$N = 2 \mathrm{E} \|\nabla[ f(w^*;\xi) ] \|^2 ]$. Can we show:
$$
2 \|\nabla[ f(w^*;\xi) ]\|^2 \geq \mu \|w^*_\xi-w^*\|^2.  
$$

That is,  $\|\nabla[ f(w;\xi) ] \|^2 \geq (\mu/2) \|w^*_\xi-w\|^2$. May be we should introduce another parameter $\tau$: $\|\nabla[ f(w;\xi) ] \|^2 \geq (\tau/2) \|w^*_\xi-w\|^2$. It does make sense that $\|\nabla [ f(w;\xi) ] \|^2$ is $\tau$-strong convex on its own ? Then we can prove $Y_1/N \leq 1/(2 \tau)$ ...


Interesting !






==> sections/Fundamental.tex <==
\section{Fundamental}
\label{sec:fundamental}

To begin with this section, we are using the following result in \cite{SVRG}. 
\begin{lem}[Generalization of the result in \cite{SVRG}]\label{lem_bound_diff_grad}
Let Assumptions \ref{ass_stronglyconvex} and \ref{ass_convex} hold. Then, $\forall w \in \mathbb{R}^d$, 
\begin{align}\label{eq:001}
\mathbb{E}[ \| \nabla f(w; \xi) - \nabla f(w_{*};\xi) \|^2 ] \leq 2L [ F(w) - F(w_{*})],   
\end{align}
where $\xi$ is a random variable, and $w_{*} = \arg \min_w F(w)$.  
\end{lem}
 
 
We then provide the following bound of $\mathbb{E}\|\nabla f_i(w)\|^2$. 

\begin{lem}[\cite{NguyenNguyenvanDijkEtAl2018}]\label{lem_bounded_secondmoment_04}
Let Assumptions \ref{ass_stronglyconvex}, \ref{ass_convex} and \ref{ass_smooth} hold. Then, for $\forall w \in \mathbb{R}^d$,
\begin{gather*}
\mathbb{E}[\|\nabla f(w; \xi)\|^2] \leq  4 L [ F(w) - F(w_{*}) ] + N,
\end{gather*}
where $N = 2 \mathbb{E}[ \|\nabla f(w_{*}; \xi)\|^2 ]$; $\xi$ is a random variable, and $w_{*} = \arg \min_w F(w)$.
\end{lem}


\begin{proof}
Note that 
\begin{gather*}
\|a\|^2 = \|a - b + b\|^2 \leq 2\|a - b\|^2 + 2\|b\|^2, \tagthis{\label{eq_aaa001}} \\
\Rightarrow \frac{1}{2}\|a\|^2 - \|b\|^2 \leq \|a - b\|^2. \tagthis{\label{eq_aaa002}}
\end{gather*}


Hence, 
\begin{align*}
\frac{1}{2} \mathbb{E}[ \| \nabla f(w; \xi) \|^2 ] - \mathbb{E}[ \| \nabla f(w_{*}; \xi) \|^2 ] &= \mathbb{E} \left[ \frac{1}{2} \| \nabla f(w; \xi) \|^2 - \| \nabla f(w_{*}; \xi) \|^2 \right] \\ 
& \overset{\eqref{eq_aaa002}}{\leq} \mathbb{E}[\| \nabla f(w; \xi) - \nabla f(w_{*}; \xi) \|^2 ] \\
& \overset{\eqref{eq:001}}{\leq} 2 L [ F(w) - F(w_{*})] \tagthis{\label{eq_aaa005}}
\end{align*}

Therefore,
\begin{align*}
\mathbb{E}[\| \nabla f(w; \xi) \|^2] &\overset{\eqref{eq_aaa001}\eqref{eq_aaa005}}{\leq} 4 L [ F(w) - F(w_{*})] + 2 \mathbb{E}[ \| \nabla f(w_{*}; \xi) \|^2 ]. 
\end{align*}
\end{proof}




In case all $f_i, i \in [n]$ are not convex, a similar lemma to Lemma \ref{lem_bounded_secondmoment_04} can be developed as follows.

\begin{lem}[~\cite{NguyenNguyenvanDijkEtAl2018}]\label{lem_bounded_secondmoment_04_new}
Let Assumptions \ref{ass_stronglyconvex} and \ref{ass_smooth} hold. Then, for $\forall w \in \mathbb{R}^d$, 
\begin{gather*}
\mathbb{E}\|\nabla f(w; \xi)\|^2 \leq  4L \kappa [ F(w) - F(w_{*}) ] + N,
\end{gather*}
where $\kappa = \frac{L}{\mu}$ and $N = 2 \mathbb{E}[ \|\nabla f(w_{*}; \xi)\|^2 ]$; $\xi$ is a random variable, and $w_{*} = \arg \min_w F(w)$.
\end{lem}


\begin{proof}
Analogous to the proof of Lemma \ref{lem_bounded_secondmoment_04}, we have

Hence, 
\begin{align*}
\frac{1}{2} \mathbb{E}[ \| \nabla f(w; \xi) \|^2 ] - \mathbb{E}[ \| \nabla f(w_{*}; \xi) \|^2 ] &= \mathbb{E} \left[ \frac{1}{2} \| \nabla f(w; \xi) \|^2 - \| \nabla f(w_{*}; \xi) \|^2 \right] \\ 
& \overset{\eqref{eq_aaa002}}{\leq} \mathbb{E}[\| \nabla f(w; \xi) - \nabla f(w_{*}; \xi) \|^2 ] \\
& \overset{\eqref{eq:Lsmooth_basic}}{\leq} L^2 \| w - w_{*} \|^2 \\ 
& \overset{\eqref{eq:stronglyconvex_00}}{\leq} \frac{2L^2}{\mu}[F(w) - F(w_{*})] = 2 L \kappa [F(w) - F(w_{*})]. 
 \tagthis{\label{eq_aaa005_new}}
\end{align*}

Therefore,
\begin{align*}
\mathbb{E}[\| \nabla f(w; \xi) \|^2] \overset{\eqref{eq_aaa001}\eqref{eq_aaa005_new}}{\leq} 4 L \kappa [ F(w) - F(w_{*})] + 2 \mathbb{E}[ \| \nabla f(w_{*}; \xi) \|^2 ]. 
\end{align*}
\end{proof}







We follow the convention that an empty product is equal to 1 and an empty sum is equal to 0, i.e., 
\begin{gather*}
\prod_{i=h}^k g_i = 1 \text{ and } \sum_{i=h}^k g_i =0 \text{ if } k<h. \tagthis \label{eq:rec00} 
\end{gather*}

\begin{lem}[~\cite{NguyenNguyenvanDijkEtAl2018}]\label{lemma:hogwild_recursive_form}
Let $Y_t, \beta_t$ and $\gamma_t$ be sequences such that $Y_{t+1} \leq \beta_t Y_t + \gamma_t$, for all $t\geq 1$. Then: 
\begin{gather*}
Y_{t+1} \leq (\sum_{i=1}^t[\prod_{j=i+1}^t \beta_j]\gamma_i)+(\prod_{j=1}^t\beta_j)Y_1. 
\tagthis \label{hogwild:recursive_form}
\end{gather*}
\end{lem}

\begin{proof}
We prove the lemma by using induction. It is obvious that \eqref{hogwild:recursive_form} is true for $t=1$ because $Y_2\leq \beta_1Y_1+ \gamma_1$. Assume as induction hypothesis that \eqref{hogwild:recursive_form} is true for $t-1$. Since $Y_{t+1} \leq \beta_t Y_t + \gamma_t$,
\begin{align*}
Y_{t+1} &\leq \beta_t Y_t + \gamma_t \\
&\leq \beta_{t}[(\sum_{i=1}^{t-1}[\prod_{j=i+1}^{t-1} \beta_j]\gamma_i)+(\prod_{j=1}^{t-1}\beta_j)Y_1] + \gamma_{t} \\
&\overset{\eqref{eq:rec00}}{=} (\sum_{i=1}^{t-1} \beta_{t}[\prod_{j=i+1}^{t-1} \beta_j]\gamma_i)+\beta_{t}(\prod_{j=1}^{t-1}\beta_j)Y_1 + (\prod_{j=t+1}^{t}\beta_j)\gamma_{t}\\
&= [(\sum_{i=1}^{t-1} [\prod_{j=i+1}^{t} \beta_j]\gamma_i)+ (\prod_{j=t+1}^{t}\beta_j)\gamma_{t}] +(\prod_{j=1}^{t}\beta_j)Y_1 \\
&= (\sum_{i=1}^{t}[\prod_{j=i+1}^{t} \beta_j]\gamma_i)+(\prod_{j=1}^{t}\beta_j)Y_1
\end{align*}
\end{proof}

==> sections/General_SGD.tex <==
\section{General Problem}

\subsection{Notation}

For the sake of analysis, we follow the notations introduced in~\cite{NguyenNguyenvanDijkEtAl2018} and recall them here. For each $\xi$, we define $D_\xi \subseteq \{1,\ldots, d\}$ as the set of possible non-zero positions in a vector of the form $\nabla f(w;\xi)$ for some $w$. We consider a fixed mapping from $u\in U$ to subsets $S^{\xi}_u\subseteq D_\xi$ for each possible $\xi$. In our notation we also let $D_\xi$ represent the diagonal $d\times d$ matrix with ones exactly at the positions corresponding to $D_\xi$ and with zeroes elsewhere. Similarly, $S^{\xi}_u$ also denotes a diagonal matrix with ones at the positions corresponding to $D_\xi$.

We will use a probability distribution $p_\xi(u)$ to indicate how to randomly select a matrix $S^\xi_u$. We choose the matrices $S^\xi_u$ and distribution $p_\xi(u)$ so that there exist $d_\xi$ such that
\begin{equation} d_\xi \mathbb{E}[S^\xi_u | \xi] = D_\xi, \label{eq:Sexp} \end{equation}
where the expectation is over $p_\xi(u)$.

We will restrict ourselves to choosing {\em non-empty} sets  $S^\xi_u$ that partition $D_\xi$ in $D$ approximately equally sized sets together with uniform distributions $p_\xi(u)$ for some fixed $D$. So, if $D\leq |D_\xi|$, then sets have sizes $\lfloor |D_\xi|/D \rfloor$ and $\lceil |D_\xi|/D \rceil$. For the special case $D>|D_\xi|$ we have exactly $|D_\xi|$ singleton sets of size $1$ (in our definition we only use non-empty sets).

For example, for $D=\bar{\Delta}$, where 
$$ \bar{\Delta} = \max_\xi \{ |D_\xi|\}$$
represents the maximum number of non-zero positions in any gradient computation $f(w;\xi)$, we have that for all $\xi$, there are exactly $|D_\xi|$ singleton sets $S^\xi_u$ representing each of the elements in $D_\xi$. Since  $p_\xi(u)= 1/|D_\xi|$ is the uniform distribution, we have $\mathbb{E}[S^\xi_u | \xi] = D_\xi / |D_\xi|$, hence, $d_\xi = |D_\xi|$.
As another example at the other extreme, for $D=1$, we have exactly one set $S^\xi_1=D_\xi$ for each $\xi$. Now $p_\xi(1)=1$ and we have $d_\xi=1$.



\subsection{Analysis}

We first derive a couple lemmas which will help us deriving our main bounds. In what follows let Assumptions \ref{ass_stronglyconvex}, \ref{ass_smooth} and \ref{ass_convex} hold for all lemmas.


\begin{lem}
\label{lemma:general_form111}
Let us define $f(w;(\xi_1,\dotsc,\xi_{k}))=\frac{1}{k}\sum_{i=1}^k f(w;\xi_i)$, then we have the following properties:
%\begin{align*}
$$\mathbb{E}[f(w;(\xi_1,\dotsc,\xi_{k}))]= F(w),$$
$$\mathbb{E}[\| \nabla f(w_*;(\xi_1,\dotsc,\xi_{k}))\|^2] = \frac{\mathbb{E}[\| \nabla f(w_*;\xi)\|^2]}{k},$$
and
$$
\mathbb{E}[\| \nabla f(w;(\xi_1,\dotsc,\xi_{k}))\|^2] \leq 4L [F(w)-F(w_*)] + \frac{N}{k}
$$
%\end{align*}
%where $N= \mathbb{E}[\| \nabla f(w_*;\xi)\|^2]$.
\end{lem}

\begin{proof}

The expectation of $f(w;(\xi_1,\dotsc,\xi_{k}))$ is equal to 

\begin{align*}
\mathbb{E}[f(w;(\xi_1,\dotsc,\xi_{k}))]&= \frac{1}{k}\sum_{i=1}^k \mathbb{E}[f(w;\xi_i)]= F(w). \tagthis \label{eq:111xx}
\end{align*}

Now we write $\mathbb{E}[\| \nabla f(w_*;(\xi_1,\dotsc,\xi_{k}))\|^2]$ as $\mathbb{E}[\sum_{j=1}^d(\frac{1}{k} \sum_{i=1}^k[\nabla f(w_*;\xi_i)]_j)^2]$. It is equal to 
\begin{align*}
 &\mathbb{E}[\sum_{j=1}^d\{ \frac{1}{k^2} \sum_{i=1}^k[\nabla f(w_*;\xi_i)]^2_j + \frac{1}{k} \sum_{i_0 \neq i_1}[\nabla f(w_*;\xi_{i_0})]_j [\nabla f(w_*;\xi_{i_1})]_j \}]\\
 =&\mathbb{E}[\sum_{j=1}^d \frac{1}{k^2} \sum_{i=1}^k[\nabla f(w_*;\xi_i)]^2_j \}] + \mathbb{E}[\sum_{j=1}^d \frac{1}{k} \sum_{i_0 \neq i_1}[\nabla f(w_*;\xi_{i_0})]_j [\nabla f(w_*;\xi_{i_1})]_j].
\end{align*}



The first term $\mathbb{E}[\sum_{j=1}^d \frac{1}{k^2} \sum_{i=1}^k[\nabla f(w_*;\xi_i)]^2_j \}]$ is equal to 
\begin{align*}
&= \sum_{j=1}^d \frac{1}{k^2} \sum_{i=1}^k \mathbb{E}[[\nabla f(w_*;\xi_i)]^2_j]=
\frac{1}{k^2} \sum_{i=1}^k \mathbb{E}[\sum_{j=1}^d[\nabla f(w_*;\xi_i)]^2_j]=
\frac{1}{k^2} \sum_{i=1}^k \mathbb{E}[\|\nabla f(w_*;\xi_i) \|^2] \\
&= \frac{1}{k}E[\| \nabla f(w_*;\xi)\|^2].
\end{align*}

The second term $\mathbb{E}[\sum_{j=1}^d \frac{1}{k} \sum_{i_0 \neq i_1}[\nabla f(w_*;\xi_{i_0})]_j [\nabla f(w_*;\xi_{i_1})]_j]$ is equal to 
\begin{align*}
&\sum_{j=1}^d \frac{1}{k} \sum_{i_0 \neq i_1} \mathbb{E}[[\nabla f(w_*;\xi_{i_0})]_j] \cdot \mathbb{E}[[\nabla f(w_*;\xi_{i_1})]_j]= \sum_{j=1}^d \frac{1}{k} \sum_{i_0 \neq i_1}[ \mathbb{E}[\nabla f(w_*;\xi_{i_0})]]_j \cdot [ \mathbb{E}[\nabla f(w_*;\xi_{i_1})]]_j. 
\end{align*}

Note that $\mathbb{E}[\nabla f(w_*;\xi_{i_0})]= \nabla \mathbb{E}[f(w_*;\xi_i)]=\nabla F(w_*)=0$. It means that the second term is equal to $0$ and then we obtain
\begin{equation}
\label{eq:ffff11}
\mathbb{E}[\| \nabla f(w_*;(\xi_1,\dotsc,\xi_{k}))\|^2] = \frac{\mathbb{E}[\| \nabla f(w_*;\xi)\|^2]}{k}.
\end{equation}

We have the following fact:

\begin{align*}
  \| \nabla f(w;(\xi_1,\dotsc,\xi_{k})) - \nabla f(w_*;(\xi_1,\dotsc,\xi_{k}))\|^2 & 
  = \frac{1}{k^2} [\|\sum_{i=1}^k (\nabla f(w;\xi_i) - \nabla f(w_*;\xi_i))\|^2] \\  
  &\leq \frac{1}{k}  \sum_{i=1}^k \| \nabla f(w;\xi_i) - \nabla f(w_*;\xi_i)\|^2\\
&= \| \nabla f(w;\xi_i) - \nabla f(w_*;\xi_i)\|^2.
\end{align*} 

Since $\mathbb{E}[\|\nabla f(w;\xi) -\nabla f(w_*;\xi) \|^2] \leq 2L[F(w)-F(w_*)]$ (see \eqref{eq:001}), we obtain

$$
\mathbb{E}[\| \nabla f(w;(\xi_1,\dotsc,\xi_{k})) - \nabla f(w_*;(\xi_1,\dotsc,\xi_{k}))\|^2] \leq 2L[F(w)-F(w_*)]. 
$$ 

With similar argument in Lemma~\ref{lem_bounded_secondmoment_04}, we can derive 

\begin{align*}
\mathbb{E}[\| \nabla f(w;(\xi_1,\dotsc,\xi_{k}))\|^2] &\leq 4L [F(w)-F(w_*)] + 2\mathbb{E}[\| \nabla f(w_*;(\xi_1,\dotsc,\xi_{k}))\|^2] \\
&\overset{\eqref{eq:ffff11}}{\leq } 4L [F(w)-F(w_*)] + 2\frac{\mathbb{E}[\| \nabla f(w_*;\xi)\|^2]}{k}\\
&=  4L [F(w)-F(w_*)] + \frac{N}{k}, \tagthis \label{eq:ffffkkkk}
\end{align*}
where $N=2\mathbb{E}[\| \nabla f(w_*;\xi)\|^2]$.

\end{proof}


We define 
$$\mathcal{F}_t=\sigma(w_0,\xi'_1,u_1,\dotsc, \xi'_{t-1},u_{t-1}), $$
where
$$\xi'_i = (\xi_{i1}, \ldots, \xi_{ik_i}).$$

We consider the following general algorithm with the following gradient updating rule:

\begin{equation}
\label{eq:general_updating}
w_{t+1} = w_t -\eta_t d_{\xi'_{t}} S^{\xi'_t}_{u_t} \nabla f(w_t;\xi'_t), 
\end{equation} 

where $f(w_t;\xi'_t) = \frac{1}{k_t} \sum_{i=1}^{k_t} f(w_t;\xi_{ti})$.
 
 \begin{lem} \label{lem:expect}  %Let $d_t$ denote the cardinality of $\mathcal{D}_t$ and assume $d_t\leq D$. 
 We have
 $$\mathbb{E}[\| d_{\xi'_t}S^{\xi'_t}_{u_t} \nabla  f(w_t;\xi'_t)  \|^2| \mathcal{F}_t, \xi'_t]\leq  D \|\nabla f(w_t;\xi'_t) \|^2$$
% $$\mathbb{E}[\|\eta_t d_t \langle \nabla f(\hat{w}_t;\xi_t)-\nabla f(w_*;\xi_t) ,e[s_t] \rangle e[s_t] \|^2| \mathcal{F}_t, \xi_t, \sigma_t]\leq \eta^2_t D \|\nabla f(\hat{w}_t;\xi_t)-\nabla f(w_*;\xi_t) \|^2, $$
 and
 $$\mathbb{E}[d_{\xi'_t}S^{\xi'_t}_{u_t} \nabla  f(w_t;\xi'_t) | \mathcal{F}_t ] 
= \nabla F(w_t).$$
 \end{lem}
 
 \begin{proof}
 For the first bound, if we take the expectation of $\| d_{\xi'_t}S^{\xi'_t}_{u_t} \nabla  f(w_t;\xi'_t)  \|^2$ with respect to $u_t$, then we have (for vectors $x$ we denote the value if its $i$-th position by $[x]_i$)
 \begin{align*}
& \mathbb{E}[\|d_{\xi'_t}S^{\xi'_t}_{u_t} \nabla  f(w_t;\xi'_t)  \|^2| \mathcal{F}_t, \xi'_t] = 
 d_{\xi'_t}^2 \sum_u p_{\xi'_t}(u)  \|S^{\xi'_t}_{u} \nabla  f(w_t;\xi'_t)  \|^2 = 
 d_{\xi'_t}^2 \sum_u p_{\xi'_t}(u)  \sum_{i\in S^{\xi'_t}_{u}} [\nabla f(w_t;\xi'_t)]_i^2 \\
&= 
 d_{\xi'_t} \sum_{i\in D_{\xi'_t}} [\nabla f(w_t;\xi'_t)]_i^2 =
 d_{\xi'_t} \| f(w_t;\xi'_t) \|^2 \leq  D \|\nabla f(w_t;\xi'_t) \|^2,
\end{align*}
where the transition to the second line follows from (\ref{eq:Sexp}).
%Since $\nabla f(.;\xi_j)$ has support $D_j$, we can use the same argument to derive the second bound.


For the second bound, if we take the expectation of $ d_{\xi'_t}S^{\xi'_t}_{u_t} \nabla  f(w_t;\xi'_t)$ wrt $u_t$, then we have:
\begin{align*}
\mathbb{E}[ d_{\xi'_t}S^{\xi'_t}_{u_t} \nabla  f(w_t;\xi'_t) | \mathcal{F}_t, \xi'_t] &=
 d_{\xi'_t} \sum_u p_{\xi'_t}(u) S^{\xi'_t}_{u}  \nabla f(w_t;\xi'_t) = \nabla f(w_t;\xi'_t),
\end{align*}
and this can be used to derive
\begin{align*}
\mathbb{E}[ d_{\xi'_t}S^{\xi'_t}_{u_t}  f(w_t;\xi'_t) | \mathcal{F}_t]
=
\mathbb{E}[\mathbb{E}[d_{\xi'_t}S^{\xi'_t}_{u_t}  f(w_t;\xi'_t) | \mathcal{F}_t, \xi'_t] | \mathcal{F}_t]
= \mathbb{E}[\nabla f(w_t;\xi'_t)]  &=  \nabla F(w_t).  %\tagthis \label{eq:Ewhat1}
\end{align*}
The last equality comes from \eqref{eq:111xx}.
\end{proof}




\begin{lem}
Let Assumptions \ref{ass_stronglyconvex}, \ref{ass_smooth} and \ref{ass_convex} hold, $0< \eta_t \leq \frac{1}{2LD}$ for all $t\geq 1$. Then, 
$$
\mathbb{E}[\|w_{t+1}-w_* \|^2] \leq (1-\mu \eta_t) \|w_t-w_*\|^2 + \eta^2_t \frac{ND}{k_t}. 
$$
\end{lem}
\begin{proof}
Since $w_{t+1} = w_t - \eta_t  d_{\xi'_t} S^{\xi'_t}_{u_t} \nabla f(w_t;\xi'_t)$, we have 
\begin{align*}
 \|w_{t+1}-w_{*}\|^2 &= \|w_t-w_{*}\|^2 - 2\eta_t \langle  d_{\xi'_t} S^{\xi'_t}_{u_t} \nabla f(w_t;\xi'_t), (w_t-w_{*})\rangle +   \eta_t^2 \|d_{\xi'_t} S^{\xi'_t}_{u_t} \nabla f(w_t;\xi'_t)\|^2.
\end{align*}

We now take expectations over $u_t$ and $\xi_t$ and use Lemmas~\ref{lem:expect} and ~\ref{lemma:general_form111}:
\begin{align}
&\mathbb{E}[\|w_{t+1} -w_* \|^2 | \mathcal{F}_t] \\
&\leq \|w_t-w_* \|^2 - 2\eta_t \langle \nabla F(w), w_t - w_*\rangle + \eta^2_t D \mathbb{E}[\| \nabla f(w_t;\xi'_t)\|^2|\mathcal{F}_t]
\end{align}

By \eqref{ass_stronglyconvex}, we have  
\begin{equation}
\label{eq:ppppppp}
 -  \langle \nabla F(w), w_t - w_*\rangle \leq - [F(w)-F(w_*)] - \mu/2 \| w_t - w_*\|^2
\end{equation}

Thus, $\mathbb{E}[\|w_{t+1} -w_* \|^2 | \mathcal{F}_t]$ is at most
\begin{align*}
&\overset{\eqref{eq:ppppppp}}{\leq} \|w_t-w_* \|^2 - \mu \eta_t \| w_t - w_*\|^2 - 2\eta_t[F(w)-F(w_*)] + \eta^2_t D \mathbb{E}[\| \nabla f(w_t;\xi'_t)\|^2|\mathcal{F}_t]. 
\end{align*}

Since $\mathbb{E}[\| \nabla f(w_t;\xi'_t)\|^2|\mathcal{F}_t] \leq 4L [F(w)-F(w_*)] + \frac{N}{k_t}$  (see \eqref{eq:ffffkkkk}), $\mathbb{E}[\|w_{t+1} -w_* \|^2 | \mathcal{F}_t]$ is at most 

\begin{align*}
&\overset{\eqref{eq:ffffkkkk}}{\leq} (1- \mu \eta_t) \| w_t - w_*\|^2 - 2\eta_t(1-2\eta_t LD)[F(w)-F(w_*)] + \eta^2_t \frac{ND}{k_t}. 
\end{align*}

Using the condition $\eta_t \leq \frac{1}{2LD}$ yields the lemma. 


\end{proof}


As shown above, 
$$\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]  \leq (1-\mu \eta_t) \mathbb{E}[ \| w_{t} - w_{*} \|^2 ] +  \frac{\eta_t^2 ND}{k_t},$$

when $\eta_t \leq \frac{1}{2LD}$.

Let $Y_{t+1}=\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]$, $Y_{t}=\mathbb{E}[\| w_{t} - w_{*} \|^2 ]$, $\beta_t= 1 - \mu \eta_t$ and $\gamma_t=\frac{\eta^2_tND}{k_t}$. As proved in Lemma~\ref{lemma:hogwild_recursive_form}, if $Y_{t+1} \leq \beta_t Y_t + \gamma_t$, then 
\begin{align*}
Y_{t+1} &\leq \sum_{i=1}^t [\prod_{j=i+1}^t \beta_j] \gamma_i + (\prod_{i=1}^t\beta_i)Y_1\\
&=  \sum_{i=1}^t [\prod_{j=i+1}^t (1 - \mu \eta_j)] \gamma_i + [\prod_{i=1}^t(1 - \mu \eta_i)]\mathbb{E}[\| w_{1} - w_{*} \|^2 ]\\
\end{align*}

Let us define $n(j)=\mu n_j$ and $M(y) = \int_{x=1}^y n(x) dx$ as in Section~\ref{sec:convergence_SGD}. We also obtain 

$$
C(t) = \exp(-M(t)) \int_{x=1}^t \exp(M(x)) \frac{n^2(x)}{k(x)}dx. 
$$

\begin{thm}
Let Assumptions \ref{ass_stronglyconvex}, \ref{ass_smooth} and \ref{ass_convex} hold, $0< \eta_t \leq \frac{1}{2LD}$ for all $t\geq 1$ and $\eta_t$ is diminishing with the condition $\sum_{t=1}^{\infty} \eta_t \rightarrow \infty$. Then, the sequence $w_1,\dotsc,w_t,\dotsc$ converges where
$$w_{t+1} = w_t -\eta_t d_{\xi'_{t}} S^{\xi'_t}_{u_t} \nabla f(w_t;\xi'_t).$$ 
\end{thm}

\begin{proof}
To prove the convergence of $w_t$, we only need to prove the convergence of $$C(t) = \exp(-M(t)) \int_{x=1}^t \exp(M(x)) \frac{n^2(x)}{k(x)}dx.$$

Let denote $T$ the total number of gradient computations and define $K(t)= \int_{x=1}^t k(x)dx=T$. From, here we have $t=K^{-1}(T)$ and $\frac{dK(x)}{dx}=k(x)$. Now, we define $y=K(x)$ or $x=K^{-1}(y)$ and $dy=k(x)dx$. We write 
\begin{align*}
C(t) &= \exp(-M(t)) \int_{x=1}^t \exp(M(x)) \frac{n^2(x)}{k(x)}dx \\
&= \exp(-M(K^{-1}(T))) \int_{K(1)}^{K^{-1}(T)}  \exp(M(K^{-1}(y))) \frac{n^2(x)}{k^2(x)} k(x)dx \\
&\leq  \exp(-M(K^{-1}(T))) \int_{1}^{K^{-1}(T)}  \exp(M(K^{-1}(y))) \frac{n^2(x)}{k^2(x)} k(x)dx.
\end{align*}
The last inequality is based on the fact that $K(1) \geq 1$. 

Let us define $n'(x)=\frac{n(x)}{k(x)}$ and using the fact that $dy=k(x)dx$, we obtain

\begin{align*}
C(t) &= C(K^{-1}(T)) \\&\leq \exp(-M(K^{-1}(T))) \int_{1}^{K^{-1}(T)}  \exp(M(K^{-1}(y))) [n'(K^{-1}(y))]^2 dy. 
\end{align*} 

Since $K^{-1}(K(x))=x$ or $\frac{dK^{-1}(K(x))}{dx}=1/\frac{dK(x)}{dx}=1/k(x)$, we have the $\frac{dM(K^{-1}(y))}{dy}= \frac{n(K^{-1}(y))}{k(K^{-1}(y))}=n'(K^{-1}(y))$. Hence, by denoting 

\begin{align*}
C'(t) &=C(K^{-1}(t)),\\
n'(x) &= \frac{n(x)}{k(x)},\\
M'(x) &= M(K^{-1}(x)),
\end{align*}

we can convert the general problem into the problem in Section~\ref{sec:convergence_SGD}. 
This implies that the analysis of $C(t)$ in Section~\ref{sec:convergence_SGD} can directly apply to analyze $C(K^{-1}(T))$ [\textcolor{red}{Ha: ask Marten to verify the correctness of this claim}]. Since we already proved the convergence of $C(t)$ in Section~\ref{sec:convergence_SGD}, we obtain the theorem.   
\end{proof}






==> sections/SGD_assumptions.tex <==
\section{SGD Algorithm and Basic Assumptions}
\label{sec:SGD_assumptions}

We introduce SGD algorithm in Algorithm \ref{sgd_algorithm}. 
\begin{algorithm}[h]
   \caption{Stochastic Gradient Descent (SGD) Method}
   \label{sgd_algorithm}
\begin{algorithmic}
   \STATE {\bfseries Initialize:} $w_1$
   \STATE {\bfseries Iterate:}
   \FOR{$t=1,2,\dots$}
  \STATE Choose a step size (i.e., learning rate) $\eta_t>0$. 
  \STATE Generate a random variable $\xi_t$.
  \STATE Compute a stochastic gradient $\nabla f(w_{t};\xi_{t}).$
   \STATE Update the new iterate $w_{t+1} = w_{t} - \eta_t \nabla f(w_{t};\xi_{t})$.
   \ENDFOR
\end{algorithmic}
\end{algorithm}


Before moving to the next discussions, let us introduce the following common assumptions, which are $L$-smoothness and $\mu$-strong convexity.

%Let us introduce our key assumption that each realization $\nabla f(w;\xi)$ is an $L$-smooth function. 

\begin{ass}[$\mu$-strongly convex]
\label{ass_stronglyconvex}
The objective function $F: \mathbb{R}^d \to \mathbb{R}$ is a $\mu$-strongly convex, i.e., there exists a constant $\mu > 0$ such that $\forall w,w' \in \mathbb{R}^d$, 
\begin{gather*}
F(w) - F(w') \geq \langle \nabla F(w'), (w - w') \rangle + \frac{\mu}{2}\|w - w'\|^2. \tagthis\label{eq:stronglyconvex_00}
\end{gather*}
\end{ass}
It is well-known in literature \cite{nesterov2004,bottou2016optimization} that Assumption \ref{ass_stronglyconvex} implies
\begin{align*}
2\mu [ F(w) - F(w_{*}) ] \leq \| \nabla F(w) \|^2 \ , \ \forall w \in \mathbb{R}^d. \tagthis\label{eq:stronglyconvex}
\end{align*}


\begin{ass}[$L$-smooth]
\label{ass_smooth}
$f(w;\xi)$ is $L$-smooth for every realization of $\xi$, i.e., there exists a constant $L > 0$ such that, $\forall w,w' \in \mathbb{R}^d$, 
\begin{align*}
\| \nabla f(w;\xi) - \nabla f(w';\xi) \| \leq L \| w - w' \|. \tagthis\label{eq:Lsmooth_basic}
\end{align*} 
\end{ass}

Assumption \ref{ass_smooth} implies that $F$ is also $L$-smooth. Then, by the property of $L$-smooth function (in \cite{nesterov2004}), we have, $\forall w, w' \in \mathbb{R}^d$, 
\begin{align*}
F(w) &\leq F(w') + \langle \nabla F(w'),(w-w') \rangle + \frac{L}{2}\|w-w'\|^2. \tagthis\label{eq:Lsmooth}
\end{align*}

The following additional convexity assumption can be made, as it holds for many problems arising in machine learning.

\begin{ass}\label{ass_convex}
$f(w;\xi)$ is convex for every realization of $\xi$, i.e., $\forall w,w' \in \mathbb{R}^d$, 
\begin{gather*}
f(w;\xi)  - f(w';\xi) \geq \langle \nabla f(w';\xi),(w - w') \rangle.
\end{gather*}
\end{ass}

We first derive our analysis under Assumptions  \ref{ass_smooth}, and \ref{ass_convex} and then we derive weaker results under only Assumption  \ref{ass_smooth}. 




==> sections/append_01.tex <==
\section{Discussion on $Z_t$}
\label{sec:append_01}

\subsection{Proof of optimal stepsize $\eta_t$}
\label{subsec:append_01_optimal_etat}

$\mathbf{Theorem~\ref{theorem:optimal_etat}}$
\textit{Let Assumptions~\ref{ass_stronglyconvex} ,\ref{ass_smooth} and \ref{ass_convex} hold. Let us consider Algorithm ~\ref{sgd_algorithm} with $N = 2 \mathbb{E}[ \|\nabla f(w_{*}; \xi)\|^2 ]$ and $Z_t$ as described in (~\ref{recZ}), i.e.,} $$Z_0=Y_0 \mbox{ and } Z_{t+1} = (1 - \mu \eta_t)Z_t + \eta_t^2 N.$$
\textit{Let $Y_0 = \mathbb{E}[\|w_0 - w_*\|^2]$ and define } 
\begin{equation*}
W = 
  \begin{cases}{} 
 \lceil \frac{\ln( \frac{2 \mu L Y_0}{N}  - 1)}{\ln( (1- \frac{\mu}{2L})^{-1}  )}\rceil, & \mbox{if } \frac{N}{Y_0} < \mu L, \\
 0, & \mbox{if } \frac{N}{Y_0} \geq \mu L.
 \end{cases} 
\end{equation*}
\textit{We consider the following sequence of $\eta_t$: }
\begin{itemize}
\item \textit{If $Y_0 \leq \frac{N}{\mu L}$, then $\eta_t = \frac{\mu Z_t}{2N}$ for $t\geq 0$.}
\item \textit{Otherwise},  \begin{equation*} \eta_t = \left\{ \begin{array}{ll}
\frac{1}{2L}, & \mbox{if } t< W, \\
\frac{\mu Z_t}{2N}, & \mbox{if } t\geq W .
\end{array} \right.
\end{equation*}
with
$$ \frac{N}{2\mu L} \leq Z_W \leq \frac{N}{\mu L}.$$
\end{itemize}
\textit{This stepsize minimizes $Z_t$.} 
\begin{proof}
In order to minimize $Z_{t+1}$ as a function of $\eta_t$ we take the derivative of the right hand side in (\ref{recZ}) with respect to $\eta_t$. This gives
$-\mu Z_t + 2\eta_t N$, which is increasing in $\eta_t$ and equals $0$ for $\eta_t= \frac{\mu Z_t}{2N}$. This implies that $(1 - \mu \eta_t)Z_t + \eta_t^2 N$ achieves its minimum for $\eta_t= \frac{\mu Z_t}{2N}$. Due to constraint $\eta_t\leq \frac{1}{2L}$, we should choose
$$ \eta_t = \min \{ \frac{1}{2L} , \frac{\mu Z_t}{2N} \}. $$
In other words,
$$ \eta_t = \left\{ \begin{array}{ll}
\frac{1}{2L}, & \mbox{if } Z_t \geq \frac{N}{\mu L}, \\
\frac{\mu Z_t}{2N}, & \mbox{otherwise.} 
\end{array} \right.
$$

Assume for now that $Z_0=Y_0 > \frac{N}{\mu L}$. Then, for the first initial recursion steps (\ref{recZ}) translates to
$$ Z_0=Y_0 \mbox{ and } Z_{t+1} = (1 - \frac{\mu}{2L})Z_t + \frac{N}{(2L)^2}$$
till $Z_t\leq \frac{N}{\mu L}$. Solving this recursion gives
\begin{eqnarray}
 Z_t &=&  (1-\frac{\mu}{2L})^{t} Y_0 + \sum_{i=0}^{t-1} (1-\frac{\mu}{2L})^i \frac{N}{4L^2} \nonumber \\
 &=&  (1-\frac{\mu}{2L})^{t} Y_0 +  \frac{N}{4L^2}[1-(1- \frac{\mu}{2L})^t]/[1-(1-\frac{\mu}{2L})] \nonumber \\
 &=& \frac{N}{2 \mu L} + (1-\frac{\mu}{2L})^{t} (Y_0 - \frac{N}{2 \mu L}). \label{eqZsmall}
 \end{eqnarray}
 This implies that $Z_t\geq \frac{N}{2\mu L}$ and $Z_t$ remains $> \frac{N}{\mu L}$ as long as 
 $$(1-\frac{\mu}{2L})^{t} (Y_0 - \frac{N}{2 \mu L} ) > \frac{N}{2 \mu L}.$$
 This is equivalent to
 $$ t< T \mbox{ where } T=  \frac{\ln( \frac{2 \mu L Y_0}{N}  - 1)}{\ln( (1- \frac{\mu}{2L})^{-1}  )}$$
 (note that $T> 0$ is properly defined since we assume $Y_0>N/(\mu L)$).
 By defining
 $$
  W = \lceil T\rceil = \lceil \frac{\ln( 2 \frac{\mu L Y_0}{N}  - 1)}{\ln( (1- \frac{\mu}{2L})^{-1}  )}  \rceil
  $$
 (note that $W\geq 1$ since $T>0$)
 we conclude
 \begin{equation*} \eta_t = \left\{ \begin{array}{ll}
\frac{1}{2L}, & \mbox{if } t< W, \\
\frac{\mu Z_t}{2N}, & \mbox{if } t\geq W .
\end{array} \right.
%\label{eqEta}
\end{equation*}
with
$$ \frac{N}{2\mu L} \leq Z_W \leq \frac{N}{\mu L}.$$

If $Y_0 \leq \frac{N}{\mu L}$, then
$$\eta_t = \frac{\mu Z_t}{2N} \mbox{ for } t\geq 0.$$
We may extend the definition of $W$ as follows:

\begin{equation*}
W = 
  \begin{cases}{} 
 \lceil \frac{\ln( \frac{2 \mu L Y_0}{N}  - 1)}{\ln( (1- \frac{\mu}{2L})^{-1}  )}\rceil, & \mbox{if } \frac{N}{Y_0} < \mu L, \\
 0, & \mbox{if } \frac{N}{Y_0} \geq \mu L.
 %\label{eqW}
 \end{cases} 
\end{equation*}

Then, combining both cases shows that (\ref{eqEta}) holds in general for  the extended definition of $W$.

We conclude that (\ref{eqEta}) with (\ref{eqW})  in combination with recurrence (\ref{recZ}) gives a {\em precise} recursive characterization of  (a) the sequence of step sizes $\eta_t$ that minimizes the upper bound $Z_t$ on the convergence rate $Y_t$, and (b) the minimized upper bound values $Z_t$ themselves.
\end{proof}





\subsection{Proof of the bounds of $Z_t$}
\label{subsec:append_01_bound_Zt}

$\mathbf{Theorem}~\ref{theorem:bound_Zt}$
\textit{We consider the sequence $Z_t$ as described in~(\ref{recZ}), i.e., $$Z_0=Y_0 \mbox{ and } Z_{t+1} = (1 - \mu \eta_t)Z_t + \eta_t^2 N$$ where $\eta_t$ is defined as in Theorem~\ref{theorem:optimal_etat}. We have:}
\begin{itemize}
\item \textit{For $t<W$ where $W$ is defined as in (\ref{eqW}),}  $$Z_t=\frac{N}{2 \mu L} + (1-\frac{\mu}{2L})^{t} (Y_0 - \frac{N}{2 \mu L} ).$$
\item \textit{For $t\geq W$, we have the following tight upper and lower bounds of $Z_t$}
\begin{equation*}
 \frac{4N}{\mu^2} \frac{1}{ (t-W) + \frac{4N}{\mu^2 Z_W}}  \geq  Z_{t} \geq 
 \frac{4N}{\mu^2} \frac{1}{ (t-W) + \frac{4N}{\mu^2 Z_W} + \ln(t-W+ \frac{4N}{\mu^2 Z_W}) - \ln( \frac{4N}{\mu^2 Z_W})}. 
\end{equation*}

\textit{Let define $\omega = \max\{\frac{N}{\mu L Y_0},1\}$. We have general weaker upper bound and lower bound of $Z_t$ as follows.}

\textbf{Weaker Upper Bound}
\begin{equation*} 
Z_t \leq  \frac{4N}{\mu} \frac{1}{ \mu t- 2L \ln( \frac{2 \omega \mu L Y_0}{N}  - 1) + 4L\omega }.
\end{equation*}

\textbf{Weaker Lower Bound}
\begin{equation*}
Z_t \geq \frac{4N}{\mu} \frac{1}{ \mu (t +\ln( \frac{t\mu}{4L\omega}+1))   +  8L\omega   }. 
\end{equation*} 
\end{itemize}


\begin{proof}
For $t<W$ the precise solution is given by $\eta_t=\frac{1}{2L}$ and $Z_t=\frac{N}{2 \mu L} + (1-\frac{\mu}{2L})^{t} (Y_0 - \frac{N}{2 \mu L} )$ in (\ref{eqEta})  and (\ref{eqZsmall}); these are easy to interpret closed form expressions. For $t\geq W$, we do not have an easy to interpret close form solution (a closed form can be constructed but depends in a rather complex way on $N$ and $Y_0$). For this reason we will derive easy to interpret lower and upper bounds on $Z_t$.


For $t\geq W$ (assumed throughout the remainder of this section), we substitute  (\ref{eqEta}) for $\eta_t$  in recurrence (\ref{recZ}): 
$$
Z_{t+1} = Z_t - \frac{\mu^2 Z_t^2}{2N} + \frac{\mu^2 Z_t^2}{4N} = Z_t - \frac{\mu^2 Z_t^2}{4N}.
$$
Let $\gamma = \frac{\mu^2}{4N}$. We obtain
\begin{equation}
\gamma Z_{t+1} =  \gamma Z_t (1 -\gamma Z_t), \label{eqZZ}
\end{equation}
where (see (\ref{eqZW}))
$$ \gamma Z_W \leq \gamma \frac{N}{\mu L} = \frac{\mu}{4L}.$$
We may rewrite (\ref{eqZZ}) as
$$ (\gamma Z_{t+1})^{-1} = 1+  (\gamma Z_{t})^{-1}  + \frac{1}{ (\gamma Z_{t})^{-1} -1}.$$
This immediately shows that  for $t+1\geq W$,
\begin{equation}
(\gamma Z_{t+1})^{-1} = (t+1-W) + (\gamma Z_{W})^{-1} + \sum_{i=W}^t \frac{1}{ (\gamma Z_{i})^{-1} -1}.\label{eqZZ1}
\end{equation}



This implies the lower bound
\begin{equation}
(\gamma Z_{t+1})^{-1} \geq (t+1-W) + (\gamma Z_{W})^{-1}, \label{eqZZL}
\end{equation}
which can be used in the sum to obtain the  upper bound
\begin{eqnarray}
\sum_{i=W}^t \frac{1}{ (\gamma Z_{i})^{-1} -1} &\leq&  \sum_{i=0}^{t-W} \frac{1}{i+(\gamma Z_{W})^{-1}} \\
&\approx& \ln(t+1-W+(\gamma Z_{W})^{-1}) - \ln((\gamma Z_{W})^{-1}).
\end{eqnarray}
  Substituting this into (\ref{eqZZ1}) yields the upper bound
\begin{equation}
(\gamma Z_{t+1})^{-1} \leq (t+1-W) + (\gamma Z_{W})^{-1} + \ln(t+1-W+ (\gamma Z_{W})^{-1}) - \ln( (\gamma Z_{W})^{-1}). 
\label{eqZZU}
\end{equation}



Bounds (\ref{eqZZL}) and (\ref{eqZZU}) hold for $t+1\geq W$. Combining these two bounds with $\gamma = \frac{\mu^2}{4N}$ (and substituting $t+1$ by $t$) proves for $t\geq W$,

\begin{equation*}
%\label{approxZ} 
 \frac{4N}{\mu^2} \frac{1}{ (t-W) + \frac{4N}{\mu^2 Z_W}}  \geq  Z_{t} \geq 
 \frac{4N}{\mu^2} \frac{1}{ (t-W) + \frac{4N}{\mu^2 Z_W} + \ln(t-W+ \frac{4N}{\mu^2 Z_W}) - \ln( \frac{4N}{\mu^2 Z_W})}. 
\end{equation*}

The upper bound and lower bounds in (\ref{approxZ}) are close. In order to gain better understanding we weaken both bounds by using  the bounds on $Z_W$ in (\ref{eqZW}). When we show our tightness example we will compare its convergence rate against the upper bound of the optimal $Z_t$ and this will teach us within what factor our example is tight. When we show how to approximate the minimizing step size function $\eta_t$ by making it independent of the unknown parameters $N$ and $Y_0$, we compare the convergence rate for the approximated $\eta_t$ against the lower bound of the optimal $Z_t$ and this will teach us within what factor the convergence rate corresponding to the approximated $\eta_t$ is close to the optimal $Z_t$.

The weakened upper and lower bounds will use parameter
$$ \omega = \max\{\frac{N}{\mu L Y_0},1\}.$$

\vspace{2mm}
{\bf For the case $W=0$:}
(\ref{eqW}) and (\ref{eqZW}) tell us that $Z_W=Y_0$ and $Y_0\leq \frac{N}{\mu L}$, hence, $\omega=\frac{N}{\mu L Y_0}$. Substituting this in (\ref{approxZ}) shows
$$\frac{4N}{\mu} \frac{1}{\mu t + 4L\omega }\geq  Z_{t} \geq \frac{4N}{\mu} \frac{1}{ \mu t +4L\omega + \mu[\ln(t+ \frac{4L\omega}{\mu}) - \ln( \frac{4L\omega}{\mu} )]}.$$


\vspace{2mm}

{\bf For the case $W\geq 1$:}      

$Y_0> \frac{N}{\mu L}$, hence, $\omega=1$.  From (\ref{eqW}) and (\ref{eqZW}) we infer that  $\frac{N}{2\mu L}\leq Z_W\leq \frac{N}{\mu L}$. Substituting these upper and lower bounds on $Z_W$ at the appropriate spots in (\ref{approxZ}) shows
$$ \frac{4N}{\mu} \frac{1}{ \mu (t-W) + 4L}\geq  Z_{t} \geq \frac{4N}{\mu} \frac{1}{ \mu (t-W) + 8L + \mu[ \ln(t-W+ \frac{4L}{\mu}) - \ln(\frac{4L}{\mu})]}.$$

By multiplying each $L$ with $\omega=1$ we notice that the upper and lower bounds for both cases start to resemble one another.

Let us analyze $W$.  If $\omega=1$, then, by assuming $\frac{\mu}{2L}$ is very small (which is true in practical settings),
\begin{equation}
\label{appW1}
 W\approx  \frac{\ln( \frac{2 \mu L Y_0}{N}  - 1)}{\ln( (1- \frac{\mu}{2L})^{-1}  )}
\approx \frac{2L}{\mu} \ln( \frac{2 \mu L Y_0}{N}  - 1) = \frac{2L}{\mu} \ln( \frac{2 \omega \mu L Y_0}{N}  - 1).
\end{equation}

If $\omega=\frac{N}{\mu L Y_0}$, then
$$\frac{2L}{\mu} \ln( 2 \omega \frac{\mu L Y_0}{N}  - 1) =\frac{2L}{\mu} \ln( 2 - 1)=0$$
and $W=0$ implying (\ref{appW1}) also holds for $\omega = \frac{N}{\mu L Y_0}$.
Hence, we obtain a general weaker upper bound for both cases:
\begin{equation*} Z_t \leq  \frac{4N}{\mu} \frac{1}{ \mu t- 2L \ln( \frac{2 \omega \mu L Y_0}{N}  - 1) + 4L\omega }.
%\label{eqUP}
\end{equation*}

A general weaker lower bound can be derived by multiplying $4L\omega$  with $2$ in the case $W=0$ at the approriate spots:
\begin{eqnarray*}
Z_t &\geq &  \frac{4N}{\mu} \frac{1}{ \mu t - 2L \ln( 2 \frac{\omega \mu L Y_0}{N}  - 1)   + 8L\omega + \mu[ \ln(t- \frac{2L}{\mu} \ln( 2 \frac{\omega \mu L Y_0}{N}  - 1)+ \frac{4L\omega}{\mu}) - \ln(\frac{4L\omega}{\mu})]} \nonumber \\
&\geq&  \frac{4N}{\mu} \frac{1}{ \mu t   + 8L\omega + \mu[ \ln(t+ \frac{4L\omega}{\mu}) - \ln(\frac{4L\omega}{\mu})]}  \nonumber \\
&=&  \frac{4N}{\mu} \frac{1}{ \mu (t +\ln( \frac{t\mu}{4L\omega}+1))   +  8L\omega   }. %\label{eqLOW}
\end{eqnarray*}

We conclude upper bound (\ref{eqUP}) and lower bound (\ref{eqLOW}) on $Z_t$  for $\frac{\mu}{2L}$ small and $t\geq W$.
\end{proof}


==> sections/append_02.tex <==
\section{Discussion on Approximation of the Optimal Step Size}
\label{append:approximation_stepsize}

$\mathbf{Theorem}~\ref{theorem:ration_zt_ztp}$
\textit{Assume  $\frac{\mu}{2L} \ll 1$ and $q$ is a constant which is larger or equal to 2. For given weaker lower bound of $Z_t$ as described in (\ref{eqLOW}) and upper bound $Z'_t$ as shown in (\ref{eqAPPRSOL}), we have:}
 \begin{equation*}
  (\ref{eqAPPRSOL})/ (\ref{eqLOW})  \leq
 4 \frac{q + 2\max\{0, \frac{N}{\mu L Y_0} -1\}  }{q-1} .
 \end{equation*}

\begin{proof}
For $t\geq T'= 4L^2 \omega Y_0/N - 4L/\mu$, 
\begin{align*}
(\ref{eqAPPRSOL})/ (\ref{eqLOW})  &= \frac{16N}{\mu} \frac{1}{\mu (t -T') +4L} 
/  \frac{4N}{\mu} \frac{1}{ \mu (t +\ln(\frac{t\mu}{4L\omega} +1))   +  8L\omega   } \\
&=4 \frac{ t +\ln(\frac{t\mu}{4L\omega} +1) + \omega 8L/\mu }{(t-T') + 4L/\mu}.
\end{align*}


Let
$$ t = q (T' +\frac{4L}{\mu})  - \frac{8L}{\mu} = q\frac{4L}{\mu} \max\{ \frac{L\mu Y_0}{N}, 1\}- \frac{8L}{\mu}$$



for some $q\geq 2$ (note that $t\geq T'$).
After substituting this formula for $t$, we obtain
\footnotesize{
\begin{eqnarray*}
 t +\ln(\frac{t\mu}{4L\omega} +1) + \frac{\omega 8L}{\mu}
&=&
 q (T' +\frac{4L}{\mu})  - \frac{8L}{\mu} +\ln( \frac{\mu(q (T' +\frac{4L}{\mu})  - \frac{8L}{\mu})}{4L\omega} +1) + \frac{\omega 8L}{\mu} \\
 &=&
 q (T' +\frac{4L}{\mu}) +\ln( \frac{\mu(q (T' +\frac{4L}{\mu})  - \frac{8L}{\mu})}{4L\omega} +1) + (\omega -1) \frac{8L}{\mu}\\
 &=& 
  q(T' +\frac{4L}{\mu}) +\ln( \frac{q \mu (T'+\frac{4L}{\mu})}{4L\omega}  - \frac{2}{\omega} +1) + (\omega -1) \frac{8L}{\mu}\\
 &=&   q(T' +\frac{4L}{\mu}) +\ln(q \mu (T'+\frac{4L}{\mu}) -8L + 4L\omega) + (\omega -1) \frac{8L}{\mu} - \ln(4L\omega).
\end{eqnarray*}
}


 
In the case $\omega = \frac{N}{\mu L Y_0}\geq 1$, $T'=0$ and we have $T'+\frac{4L}{\mu}=\frac{4L}{\mu}$. We derive
 $$ \frac{ (\omega -1) \frac{8L}{\mu} - \ln(4L\omega)}{T' +\frac{4L}{\mu}}
 =
  2(\frac{N}{\mu L Y_0} -1)  - \frac{\mu}{4L} \ln(\frac{4N}{\mu  Y_0})
  =
  2(\frac{N}{\mu L Y_0} -1)  + \frac{\mu}{4L} \ln(\frac{4N}{\mu  Y_0}) .$$

Inequality $\omega = \frac{N}{\mu L Y_0}\geq 1$ implies $\frac{\mu  Y_0}{4N} \leq \frac{1}{4L}$. Therefore,
$$ \frac{ (\omega -1) \frac{8L}{\mu} - \ln(4L\omega)}{T'+\frac{4L}{\mu}}
 = 2(\frac{N}{\mu L Y_0} -1)  + \frac{\mu}{4L} \ln(\frac{\mu  Y_0}{4N})
 \leq 2(\frac{N}{\mu L Y_0} -1)  + \frac{\mu}{4L}  \max\{0, -\ln(4L)\}.$$
  
 In the case $\omega =1\geq \frac{N}{\mu L Y_0}$,  $T'+ 4L/\mu = \frac{4L^2  Y_0}{N}$ and we derive
 $$ \frac{ (\omega -1) \frac{8L}{\mu} - \ln(4L\omega)}{T'+4L/\mu}
 =\frac{ - \ln(4L) }{ 4L^2  Y_0/N}= -\frac{N}{4L^2 Y_0} \ln(4L) .$$
 If $4L\geq 1$, then $-\ln(4L)\leq 0$. If $4L<1$, then $-\ln(4L)>0$ and by using $\frac{N}{\mu L Y_0}\leq 1$ we obtain
 $-\frac{N}{4L^2 Y_0} \ln(4L)\leq - \frac{\mu}{4L} \ln(4L)$. Hence,
 $$\frac{ (\omega -1) \frac{8L}{\mu} - \ln(4L\omega)}{T' +\frac{4L}{\mu}}
  = -\frac{N}{4L^2 Y_0} \ln(4L)\leq  \frac{\mu}{4L}  \max\{0,  -\ln(4L)\}.$$
  
  Combining both cases gives
\begin{equation}
\label{xxxx111}  
 \frac{ (\omega -1) \frac{8L}{\mu} - \ln(4L\omega)}{T'+\frac{4L}{\mu}} \leq 2\max\{0, \frac{N}{\mu L Y_0} -1\} + \frac{\mu}{4L}  \max\{0,  -\ln(4L)\} 
\end{equation}  
  Now we can derive (we use $(t-T')+\frac{4L}{\mu} = (q-1)(T'+\frac{4L}{\mu})$)
\begin{align*}
  (\ref{eqAPPRSOL})/ (\ref{eqLOW})  &= 
 4 \frac{ t +\ln(\frac{t\mu}{4L\omega} +2) + \frac{\omega 8L}{\mu} }{(t-T') + \frac{4L}{\mu}}\\
 & \leq
 4 \frac{ q(T'+\frac{4L}{\mu}) +\ln(q\mu (T'+\frac{4L}{\mu}) -8L+ 4L\omega ) - \ln(4L\omega) + (\omega -1) \frac{8L}{\mu}}{ (q-1)(T' +\frac{4L}{\mu})} \\
 & =
 4 ( \frac{q}{q-1} + \frac{\ln(q\mu(T' +\frac{4L}{\mu})-8L+4L\omega)}{(q-1)(T' +\frac{4L}{\mu})} + \frac{1}{q-1}\frac{ (\omega -1) \frac{8L}{\mu} - \ln(4L\omega)}{T' +4L/\mu} )\\
 & \overset{(\ref{xxxx111})}{\leq} 
 4( \frac{q + 2\max\{0, \frac{N}{\mu L Y_0} -1\} + \frac{\mu}{4L}  \max\{0,  -\ln(4L)\} }{q-1}
  + \frac{\ln(q\mu(T'+\frac{4L}{\mu})-8L+4L\omega)}{(q-1)(T'+\frac{4L}{\mu})})\\
  & =
 4( \frac{q + 2\max\{0, \frac{N}{\mu L Y_0} -1\} + \frac{\mu}{4L}  \max\{0,  -\ln(4L)\} }{q-1} + \frac{\ln( q \mu \frac{4L}{\mu} \omega -8L+4L\omega) }{(q-1) \frac{4L}{\mu} \omega})\\
   & =
 4( \frac{q + 2\max\{0, \frac{N}{\mu L Y_0} -1\} + \frac{\mu}{4L}  \max\{0,  -\ln(4L)\} }{q-1} + \frac{\ln( 4qL  \omega -8L+4L\omega) }{(q-1) \frac{4L}{\mu}\omega})\\
    & =
 4( \frac{q + 2\max\{0, \frac{N}{\mu L Y_0} -1\} + \frac{\mu}{4L}  \max\{0,  -\ln(4L)\} }{q-1} + \frac{\ln( 4L(q+1)\omega -8L) }{(q-1) \frac{4L}{\mu} \omega})\\
 &\leq  4( \frac{q + 2\max\{0, \frac{N}{\mu L Y_0} -1\} + \frac{\mu}{4L}  \max\{0,  -\ln(4L)\} }{q-1} + \frac{\ln( 4L(q+1)\omega) }{(q-1) \frac{4L}{\mu} \omega}).
\end{align*} 
  
Since $\frac{L}{\mu}\gg 1$ in practice, the last term with the natural logarithm is close to $0$ and also $\frac{\mu}{4L}  \max\{0,  -\ln(4L)\} \approx 0$. We may conclude for $\frac{\mu}{2L} \ll 1$,
 \begin{equation*}
  (\ref{eqAPPRSOL})/ (\ref{eqLOW})  \leq
 4 \frac{q + 2\max\{0, \frac{N}{\mu L Y_0} -1\}  }{q-1}.
 \end{equation*}
\end{proof}




==> sections/append_03.tex <==
\section{Discussion on Tightness of the Convergence Rate $Z_t$}
\label{sec:example_tightness}

$\mathbf{Theorem}~\ref{theorem:example_tightness}$
\textit{We consider a multivariate normal distribution of a $k$-dimensional random vector $\xi$, i.e., $\xi \sim \mathcal{N}(m,\Sigma)$, where $m=\mathrm{E}[\xi]$ and $\Sigma = \mathrm{E}[(\xi-m)(\xi-m)^{\mathrm{T}}]$ is the (symmetric positive semi-definite) correlation matrix. The density function of $\xi$ is}
$$
g(\xi) = \frac{\exp( \frac{- (\xi-m)^\mathrm{T}\Sigma^{-1}(\xi-m)}{2} )}{\sqrt{(2\pi)^k|\Sigma|}}. 
$$

\textit{We select  component functions }
 $$f(w;\xi)=s(\xi)\frac{\|w-\xi\|^2}{2},$$
 \textit{where function $s(\xi)$ is constructed {\em a-priori} according to the following random process: 
 \begin{itemize} 
 \item With probability $1-\mu/L$, we draw $s(\xi)$ from the uniform distribution over interval $[0, \mu/(1-\mu/L)]$, and
 \item with probability $\mu/L$, we draw $s(\xi)$ from the uniform distribution over interval $[0, L]$.
 \end{itemize}}
We run Algorithm~\ref{sgd_algorithm} with stepsize $\eta_t$ as described in~(\ref{eqCand})
(i.e., $\eta_t = \frac{2}{\mu t + 4L} \mbox{ for } t\geq 0$). Then
\begin{equation*}
 Y_t \geq \frac{N}{2\mu} \frac{1}{\mu (t + \ln(t+ L/12 ))} ,
\end{equation*}
For $t\geq W \approx \frac{4.796\cdot L}{\mu}$,
\begin{equation*}
Z_t \leq \frac{4N}{\mu} \frac{1}{ \mu t- 0.796\cdot L }. 
\end{equation*}
\textit{Now we can compare (\ref{tightLOW}) and (\ref{tightZUP}): For $t\geq  \frac{4.796\cdot L}{\mu}$,}
\begin{equation*}
\frac{(\ref{tightZUP})}{(\ref{tightLOW})} 
= \frac{ \frac{4N}{\mu} \frac{1}{ \mu t- 0.796\cdot L }}{ \frac{N}{2\mu} \frac{1}{\mu (t + \ln(t+ L/12 ) )}}
= 8 \frac{t + \ln(t+ L/12 )}{ t - 0.796\cdot L/\mu }.
\end{equation*}

\begin{proof}
Clearly, $f(w;\xi)$ is $s(\xi)$-smooth where the maximum value of $s(\xi)$ is equal to $L$. That is, all functions $f(w;\xi)$ are $L$-smooth (and we cannot claim a smaller smoothness parameter). We notice that

 $$ \mathrm{E}_{\xi}[s(\xi)]  = (1-\mu/L) \frac{\mu/(1-\mu/L)}{2} + (\mu/L) \frac{L}{2} = \mu$$
 and
 $$  \mathrm{E}_{\xi}[s(\xi)^2]  =  (1-\mu/L) \frac{(\mu/(1-\mu/L))^2}{12}+ (\mu/L) \frac{L^2}{12}= \frac{\mu (L + \frac{\mu}{1-\mu/L})}{12}.$$
 
With respect to $f(w;\xi)$ and distribution $g(\xi)$ we define
  $$F(w) = \mathrm{E}_{\xi}[f(w;\xi)] = \mathrm{E}_{\xi}[s(\xi) \frac{\|w-\xi\|^2}{2}].$$
  Since $s(\xi)$ only assigns a random variable to $\xi$ which is drawn from a distribution whose description is not a function of $\xi$, random variables $s(\xi)$ and $\xi$ are statistically independent. Therefore,
   $$F(w) = \mathrm{E}_{\xi}[s(\xi) \frac{\|w-\xi\|^2}{2}] = \mathrm{E}_{\xi}[s(\xi)]  \mathrm{E}_{\xi}[\frac{\|w-\xi\|^2}{2}]
   = \mu  \mathrm{E}_{\xi}[\frac{\|w-\xi\|^2}{2}].
   $$
 Notice:
\begin{enumerate}
\item $\|w-\xi\|^2 = \|(w-m)+(m-\xi)\|^2= \|w-m\|^2 + 2 \langle w-m,m-\xi \rangle + \|m-\xi \|^2$. 
\item Since $m=\mathrm{E}[ \xi ]$, we have $\mathrm{E}[ m-\xi ] =0$.
\item   $\mathrm{E}[ \|m-\xi\|^2 ]=\sum_{i=1}^k \mathrm{E}[ (m_i-\xi_i)^2 ] = \sum_{i=1}^k \Sigma_{i,i} = \mathrm{Tr}(\Sigma)$. 
\end{enumerate}
 Therefore, 
 $$F(w) = \mu  \mathrm{E}_{\xi}[\frac{\|w-\xi\|^2}{2}] = \mu \frac{\|w-m\|^2}{2} + \mu \frac{\mathrm{Tr}(\Sigma)}{2},$$ and this shows $F$ is $\mu$-strongly convex and has minimum 
 $$w^* = m.$$
 
 Since
$$\nabla_w [ \|w-\xi\|^2 ] = \nabla_w [ \langle w,w \rangle - 2\langle w,\xi \rangle + \langle \xi,\xi \rangle ] = 2w -2 \xi = 2(w-\xi), 
$$
we have $$ \nabla_w f(w;\xi)= s(\xi)(w-\xi). $$
In our notation 
$$N=2 \mathrm{E}_\xi[\|\nabla f(w^*;\xi) \|^2]=2 \mathrm{E}_{\xi}[s(\xi)^2 \|w^* -\xi \|^2].$$
By using similar arguments we can split the expectation and obtain
$$ N = 2 \mathrm{E}_{\xi}[s(\xi)^2 \|w^* -\xi \|^2] = 2  \mathrm{E}_{\xi}[s(\xi)^2] \mathrm{E}_{\xi}[ \|w^* -\xi \|^2].$$
We already calculated 
$$\mathrm{E}_{\xi}[ \|w^* -\xi \|^2] = \|w^*-m\|^2 + \mathrm{Tr}(\Sigma)= \mathrm{Tr}(\Sigma)$$
and we know $ \mathrm{E}_{\xi}[s(\xi)^2] = \frac{\mu (L + \frac{\mu}{1-\mu/L})}{12}$. This yields
$$ N =  2  \mathrm{E}_{\xi}[s(\xi)^2] \mathrm{E}_{\xi}[ \|w^* -\xi \|^2]
= \frac{\mu (L + \frac{\mu}{1-\mu/L})}{6} \mathrm{Tr}(\Sigma).$$

In the SGD algorithm we compute
$$
w_{t+1} = w_t - \eta_t \nabla f(w_t;\xi_t) = w_t - \eta_t s(\xi) (w_t - \xi_t) = (1-\eta_t s(\xi)) w_t + \eta_t s(\xi) \xi_t. 
$$
We choose $w_0$ according to the following computation: We draw $\xi$ from its distribution and apply full gradient descent in order to find $w^*_\xi$ which minimizes $f(w;\xi)$. Since  $f(w;\xi)=s(\xi)\frac{\|w-\xi\|^2}{2}$, $w^*_i=\xi$ and
$$ Y_0 = \mathrm{E}[ \|w_0-w^*\|^2] = \mathrm{E}[ \|\xi-w^*\|^2]] = \mathrm{Tr}(\Sigma).$$

Again let $\omega = \max\{\frac{N}{\mu L Y_0},1\}$. By using our expressions for $N$ and $Y_0$ we derive, for small $\frac{\mu}{2L}$,
$$ \omega = \max\{\frac{N}{\mu L Y_0},1\} = \max\{ \frac{ 1+ \frac{\mu}{L(1-\mu/L)}}{6}, 1\} =1.$$
Furthermore, see (\ref{appW1}),
\begin{equation} W \approx \frac{2L}{\mu} \ln( \frac{2 \omega \mu L Y_0}{N}  - 1)
= 
\frac{2L}{\mu} \ln ( \frac{12}{1 + \frac{\mu}{L(1-\mu/L)}} -1) \approx \frac{2 \ln(11) L}{\mu} \approx \frac{4.796\cdot L}{\mu}.\label{eqWtight}
\end{equation}



Let $\mathcal{F}_t=\sigma(w_0,\xi_0,\dotsc,\xi_{t-1})$ be the $\sigma$-algebra generated by $w_0,\xi_0,\dotsc,\xi_{t-1}$. We derive
$$
\mathrm{E}[ \|w_{t+1}-w^*\|^2 | \mathcal{F}_t ]
=\mathrm{E}[ \|(1-\eta_t s(\xi)) (w_t -w^*) + \eta_t s(\xi) (\xi_t - w^*) \|^2 | \mathcal{F}_t ]
$$
which is equal to 
$$
\mathrm{E}[ (1-\eta_t s(\xi))^2 \|w_t -w^*\|^2 + 2\eta_t s(\xi)(1-\eta_t s(\xi) ) <w_t-w^*, \xi_t - w^*> +  \eta_t^2 s(\xi)^2 \|\xi_t -w*\|^2 | \mathcal{F}_t]. 
$$
Given $\mathcal{F}_t$, $w_t$ is not a random variable. Furthermore, we can use linearity of taking expectations and as above split expectations:
$$
\mathrm{E}[(1-\eta_t s(\xi))^2] \|w_t -w^*\|^2 + \mathrm{E}[2\eta_t s(\xi)(1-\eta_t s(\xi) )] <w_t-w^*, \mathrm{E}[\xi_t - w^*]> + \mathrm{E}[ \eta_t^2 s(\xi)^2] \mathrm{E}[ \|\xi_t -w*\|^2]. $$
Again notice that $\mathrm{E}[\xi_t -w^*] = 0$ and $\mathrm{E}[ \| \xi_t - w^* \|^2 ] = \mathrm{Tr}(\Sigma)$. So,
\begin{eqnarray*}
\mathrm{E}[\|w_{t+1}-w^*\|^2 | \mathcal{F}_t ] &=&
\mathrm{E}[(1-\eta_t s(\xi))^2] \|w_t -w^*\|^2  +\eta_t^2 \frac{N}{2}  \\
&=& (1- 2\eta_t \mu + \eta_t^2 \frac{\mu (L + \frac{\mu}{1-\mu/L})}{12}) \|w_t -w^*\|^2  +\eta_t^2 \frac{N}{2} \\
&=& (1-\mu \eta_t (2 - \eta_t (L + \frac{\mu}{1-\mu/L})/12)  \|w_t -w^*\|^2  +\eta_t^2 \frac{N}{2} .
\end{eqnarray*}
In terms of $Y_t=[\mathrm{E}\|w_{t}-w^*\|^2]$, by taking the full expectation (also over $\mathcal{F}_t$) we get
$$ Y_{t+1} = (1-\mu \eta_t (2 - \eta_t (L + \mu(1-\mu/L))/12)  Y_t  +\eta_t^2 \frac{N}{2}.$$
This is very close to recurrence Equation~\ref{main_ineq_sgd_new02}.
 
 The optimal step size in this case is again solved by taking the derivative with respect to $\eta_t$. The derivative is now equal to
 $$-2\mu Y_t + 2\eta_t \mu  (L + \frac{\mu}{1-\mu/L}) Y_t/12 + N\eta_t$$
 which shows the minimum is achieved for
 $$ \eta_t = \frac{ 2\mu Y_t }{N + \mu  (L + \frac{\mu}{1-\mu/L}) Y_t/6}$$
 giving
  $$  Y_{t+1} =Y_t - \frac{ 2\mu^2 Y_t^2 }{N + \mu  (L + \mu(1-\mu/L)) Y_t/6}
  = Y_t - \frac{ 2\mu^2 Y_t^2 }{N (1+ Y_t/ \mathrm{Tr}(\Sigma))}.$$
  
  We proceed by proving a lower bound on $Y_t$.
  Clearly,
  $$  Y_{t+1} \geq Y_t - \frac{ 2\mu^2 Y_t^2 }{N}.$$
  We may use the exact same derivation from (\ref{eqZZ}) onwards with $\gamma = 2\mu^2/N$ (and $W=0$ since the recursion on $Y_t$ already holds from $0$ onwards).
  This gives a bound similar to (\ref{eqZZU}): 
$$(\gamma Y_{t+1})^{-1} \leq (t+1) + (\gamma Y_0)^{-1} + \ln(t+1+ (\gamma Y_0)^{-1}) - \ln( (\gamma Y_0)^{-1}) $$
Reordering, substituting $\gamma = 2\mu^2/N$, and replacing  $t+1$ by $t$ yields, for $t\geq 0$, the lower bound
\begin{eqnarray*}
 Y_t &\geq&  \frac{N}{2\mu} \frac{1}{\mu t + N/(2 Y_0) + \mu[ \ln(t+ \frac{N}{2\mu Y_0} ) - \ln( \frac{N}{2\mu Y_0} )]} \nonumber \\
&=& \frac{N}{2\mu} \frac{1}{\mu t + \frac{\mu (L + \mu/(1-\mu/L))}{12} + \mu[ \ln(t+ L \frac{ 1 + \mu/(L(1-\mu/L))}{12} ) - \ln(  L \frac{ 1 + \mu/(L(1-\mu/L))}{12} )]} \nonumber  \\
&\approx &  \frac{N}{2\mu} \frac{1}{\mu (t + \ln(t+ L/12 ))} , 
\end{eqnarray*}
where the approximation follows from $\mu/(2L)\ll 1$. 
%
%
We notice that $Y_t\leq Z_t$ and $Z_t$ satisfies the upper bound (\ref{eqUP}) for 
$t\geq W \approx \frac{4.796\cdot L}{\mu}$  (see the derivation above for $W$ in (\ref{eqWtight})):
\begin{eqnarray*}
Z_t &\leq&  \frac{4N}{\mu} \frac{1}{ \mu t- 2L \ln( 2 \omega \mu L Y_0/N  - 1) + 4L\omega } \nonumber \\
&=&  \frac{4N}{\mu} \frac{1}{ \mu t- 2L \ln( 2  \mu L Y_0/N  - 1) + 4L } \nonumber \\
&\approx&  \frac{4N}{\mu} \frac{1}{ \mu t- 2L \ln(11) + 4L } = \frac{4N}{\mu} \frac{1}{ \mu t- 0.796\cdot L }  . 
\end{eqnarray*}
Now we can compare (\ref{tightLOW}) and (\ref{tightZUP}): For $t\geq  \frac{4.796\cdot L}{\mu}$,
\begin{equation*}
\frac{(\ref{tightZUP})}{(\ref{tightLOW})} 
= \frac{ \frac{4N}{\mu} \frac{1}{ \mu t- 0.796\cdot L }}{ \frac{N}{2\mu} \frac{1}{\mu (t + \ln(t+ L/12 ) )}}
= 8 \frac{t + \ln(t+ L/12 )}{ t - 0.796\cdot L/\mu }.
\end{equation*}
\end{proof}



==> sections/append_04.tex <==
\section{Numerical Experiments on Tightness}
\label{sec:experiments_tightness}

We continue Section~\ref{subsec_numerical_tightness} for the experiments with different values of $n$ (1000, 10000, and 100000) and $d$ (10, 100, and 1000) in Figures~\ref{figure_n_1000}, \ref{figure_n_10000}, and \ref{figure_n_100000}. 

\begin{figure}[h]
 \centering
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_1000_s3_10}
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_1000_s4_10} 
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_1000_s3_100}
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_1000_s4_100}
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_1000_s3_1000}
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_1000_s4_1000} 
   \caption{$Y_t$ with its lower bound and $Z_t$ with its upper bound ($n = 1,000$)}
  \label{figure_n_1000}
 \end{figure}
 
\begin{figure}[h]
 \centering
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_10000_s3_10}
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_10000_s4_10} 
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_10000_s3_100}
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_10000_s4_100}
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_10000_s3_1000}
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_10000_s4_1000} 
   \caption{$Y_t$ with its lower bound and $Z_t$ with its upper bound ($n = 10,000$)}
  \label{figure_n_10000}
 \end{figure} 
 
\begin{figure}[h]
 \centering
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_100000_s3_10}
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_100000_s4_10} 
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_100000_s3_100}
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_100000_s4_100}
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_100000_s3_1000}
 \includegraphics[width=0.49\textwidth]{Exp_Sec5/data_100000_s4_1000} 
   \caption{$Y_t$ with its lower bound and $Z_t$ with its upper bound ($n = 100,000$)}
  \label{figure_n_100000}
 \end{figure}  

==> sections/convexity.tex <==
\section{Convexity}
\label{sec:convexity}

Assume all $f(w;\xi_i)$ are convex and $L$-smooth, and $F(w)$ is $\mu$-strongly convex. For given $w,w',\xi$, we have
\begin{align*}
f(w;\xi) - f(w';\xi) &= \langle \nabla f(w';\xi),w-w'\rangle + \alpha(w,w';\xi)\|w-w' \|^2. \tagthis \label{eq:xxffff}
\end{align*}

Since $f$ is convex and $L$-smooth, $0 \leq \alpha(w,w';\xi) \leq \frac{L}{2}$. We take the expectation of \eqref{eq:xxffff}:

\begin{align*}
F(w) - F(w') &= \langle \nabla F(w'),w-w'\rangle + \mathbb{E}_{\xi}[\alpha(w,w';\xi)]\|w-w' \|^2. \tagthis \label{eq:xxfffff}
\end{align*}

Since $F$ is $\mu$-strongly convex, we obtain:

$$
  \frac{\mu}{2} \leq  \mathbb{E}_{\xi}[\alpha(w,w';\xi)]  \leq \mathrm{Pr}(\alpha(w,w';\xi) \geq \epsilon)\frac{L}{2} + [1- \mathrm{Pr}(\alpha(w,w';\xi) \geq \epsilon)]\epsilon.
$$

Let define $\beta = \mathrm{Pr}(\alpha(w,w';\xi)\geq \epsilon )$. From the inequality above, we obtain
\begin{align*}
\beta &= \mathrm{Pr}(\alpha(w,w';\xi)\geq \epsilon ) \geq \frac{\mu-2\epsilon}{L-2\epsilon}.
\end{align*}

We define $\xi(k)=(\xi_1,\dotsc,\xi_k)$ and 
$$
   f(w;\xi(k))=\frac{1}{k} \sum_{i=1}^k f(w;\xi_i) 
$$

and $w^*_{\xi(k)}$ is the minimum of $f(w;\xi(k))$. Moreover, let $\alpha(w,w';\xi(k))=\frac{1}{k}\sum_{i=1}^k \alpha(w,w';\xi_i)$. We consider the following update
$$
w_{t+1} = w_t -\eta_t \nabla f(w_t;\xi_t(k)).
$$

Let $\mathcal{F}_t$ be the $\sigma$-algebra which contains $w_0,\xi(0),w_1,\dotsc,w_{t-1},\xi(t-1)$.

From the update above, we can derive
\begin{align*}
\mathbb{E}[\|w_{t+1} - w^*_{\xi_t(k)} \|^2|\mathcal{F}_t] &\leq (1-2\eta_t \mathbb{E}[\alpha(w,w';\xi_t(k))] + \eta^2_t L) \|w_t -w^*_{\xi_t(k)} \|^2.
\end{align*}

We have $\mathbb{E}[\alpha(w,w';\xi_t(k))] \geq \epsilon \frac{\mu-2\epsilon}{L-2\epsilon} \frac{1}{c}$ with probability larger than $$1-(1-\frac{\mu-2\epsilon}{L-2\epsilon})^{c\frac{L-2\epsilon}{\mu-2\epsilon}} $$

\textcolor{red}{Ha: Marten, i cannot understand how we can have the probability above. Could you check the computation? I think $\mathbb{E}[\alpha(w,w';\xi_t(k))]=\mathbb{E}[\alpha(w,w';\xi)]\geq \epsilon$ with the probability $\beta= \frac{\mu-2\epsilon}{L-2\epsilon}$. Thus, we have 
\begin{align*}
\mathbb{E}[\|w_{t+1} - w^*_{\xi_t(k)} \|^2|\mathcal{F}_t] &\leq (1-2\eta_t\epsilon + \eta^2_t L) \|w_t -w^*_{\xi_t(k)} \|^2.
\end{align*}
Let define $\gamma_t=2\eta_t\epsilon - \eta^2_t L$. We can write the inequality above as:
\begin{align*}
\mathbb{E}[\|w_{t+1} - w^*_{\xi_t(k)} \|^2|\mathcal{F}_t] &\leq (1-\gamma_t) \|w_t -w^*_{\xi_t(k)} \|^2,
\end{align*}
with the probability $\beta= \frac{\mu-2\epsilon}{L-2\epsilon}$.
}

If $\eta_t < \frac{1}{\epsilon} \frac{1}{L^2}\frac{\mu-2\epsilon}{L-2\epsilon} \frac{1}{c}$, 
we obtain 

\begin{align*}
\|w_{t+1} - w^*_{\xi_t(k)} \|^2 &\leq (1-\gamma) \|w_t -w^*_{\xi_t(k)} \|^2, 
\end{align*}
where 
$\gamma =\frac{2[\epsilon(\mu-2\epsilon)]^2}{[L(L-2\epsilon)c]^2}$.

If we set $\epsilon=\mu/4$, then $\gamma \leq 2 \frac{\mu^4}{[4L(2L-\mu)c]^2}$.

\textcolor{red}{Ha: what is our message here? It is trivial from the update form that $w_t$ will go ahead toward $w^*_{\xi_t(k)}$. Maybe, the only \textbf{novel} contribution is that it would be ahead toward $w^*_{\xi_t(k)}$ with some probability computed as above and the computation of $\gamma$. Moreover, in one email, you claimed that when $k=\frac{c(2L-\mu)}{\mu}$, then $f(w;xi(k))$ would be $\mu/2$-strongly convex with probability $1-\exp(-c)$. How can we compute this probability?}



Let consider $F'(w)=\frac{1}{k} \sum_{i=1}^k f(w;\xi_i)$ and its minimum is $w+$, then we have 
\begin{align*}
F(w*) &\leq F(w+) \\
F'(w+) &\leq F'(w*). 
\end{align*}

We are interested in $|F(w*) - F'(w+)|< \epsilon$, where $\epsilon = m\sigma$ and $\sigma^2=\mathbb{E}[F'(w)^2]-(\mathbb{E}[F'(w)])^2$. 

Note that
\begin{align*}
\sigma^2 &= \frac{1}{k}[\mathbb{E}[f^2(w;\xi)]-[\mathbb{E}[f(w;\xi)]]^2]\\
&=\frac{1}{k}[\mathbb{E}[f^2(w;\xi)]-F^2(w)].\\
\end{align*}

We assume that for all $w$, $\sigma^2 \leq \sigma'$. \textcolor{red}{Ha: how do we compute $\sigma'$?} 

\textcolor{red}{Somehow we need $k\geq \frac{\sigma'}{\epsilon^2 \delta}$ and $k \geq \frac{L-\mu/4}{\mu}$, where $\delta = \exp(-c)$}. From here, we conclude $k=\max\{n, \max\{\frac{\sigma'}{\epsilon^2 \delta}, \frac{L-\mu/4}{\mu} \} \}$ to replace $F$ by $F'$ which is $\epsilon$-strongly convex and satisfies $|F(w*) - F'(w+)|< \epsilon$ with a probability at least $1-\delta$.



==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}


\textcolor{red}{Attention: we borrow many texts from the paper of SGD-Hogwild!. Somehow we need to rephrase the texts. The structure of the draft may be drastically changed, i.e., the proofs of some lemmas may be moved to the appendix section.}

We are interested in solving the following stochastic optimization problem
\begin{align*}
\min_{w \in \mathbb{R}^d} \left\{ F(w) = \mathbb{E} [ f(w;\xi) ] \right\}, \tagthis \label{main_prob_expected_risk}  
\end{align*}
where $\xi$ is a random variable  obeying some distribution. 

In the case of empirical risk minimization with a training set $\{(x_i,y_i)\}_{i=1}^n$, $\xi_i$ is a random variable that is defined 
 by a single random sample  $(x,y)$  pulled uniformly from the training set. Then,  by defining  $f_i(w) := f(w;\xi_{i})$, empirical risk minimization reduces to  
\begin{gather}\label{main_prob}
\min_{w \in \mathbb{R}^d} \left\{ F(w) = \frac{1}{n} \sum_{i=1}^n f_i(w) \right\}.  
\end{gather}


We focus on the case of \eqref{main_prob} when $F$ is strongly convex. Throughout the paper, we assume that there exists an optimal solution $w^{*}$ of \eqref{main_prob}. 

Problem of this type arise frequently in supervised learning applications \cite{ESL}. The classic first-order methods to solve the problem (\ref{main_prob}) are gradient descent (GD) \cite{Nocedal2006NO}  and stochastic gradient descent (SGD)~\footnote{We mark here that even though stochastic gradient is referred to as SG in literature, the term stochastic gradient descent (SGD) has been widely used in many important works of large-scale learning} \cite{RM1951} algorithms. GD is a standard deterministic gradient method, which updates iterates along the negative full gradient with the learning $\eta_t$ as follows
\begin{gather*}
w^{t+1} = w^{t} - \eta_t \nabla F(w^{t}) = w^{t} - \frac{\eta_t}{n} \sum_{i=1}^n \nabla f_i(w^{t}) \ , \ t \geq 1.  
\end{gather*}

We can choose $\eta_t = \eta = \Ocal(1/L)$ and achieve a linear convergence rate for the strongly convex case \cite{nesterov2004}. However, GD requires evaluation of $n$ derivatives at each step, which is very expensive and avoided to use in large-scale optimization. Instead of evaluating full gradient at each step, SGD generate an unbiased random variable $\xi_t$ such as $$\mathbb{E}_{\xi_t}[\nabla f(w_t;\xi_t)]=\nabla F(w),$$
and then evaluates gradient $\nabla f(w_t;\xi_t)$. After that, $w_t$ is updated as follows
\begin{gather*}
w^{t+1} = w^{t} - \eta_t \nabla f(w^{t};\xi_t). \tagthis \label{sgd_step}
\end{gather*}

Obviously, the computational cost of SGD is $n$ times cheaper than that of GD. However, we need to choose $\eta_t = \Ocal(1/t)$ and the convergence rate of SGD is slowed down to $\Ocal(1/t)$ \cite{bottou2016optimization}, which is a sublinear convergence rate. 

In the current literature of SGD, there are two following requirements of diminishing stepsizes $\{\eta_t\}$ to make SGD converge: (1) $\sum_{t=1}^{\infty} \eta_t \rightarrow \infty$ and (2) $\sum_{t=1}^{\infty} \eta^2_t < \infty$. In this paper, we show the latter condition is not necessary. Moreover, it is believed that the larger stepsizes $\eta_t$s are, the faster SGD converges. For example, if we consider the class of stepsize $\eta_t=\frac{1}{(K+t)^q}$ for $0<q\leq 1$ and $K$ is a certain positive constant. Then the smaller $q$ (or the larger stepsize $\eta_t$) is, the faster SGD converges. But it is not true. We will show that the fastest convergence rate SGD can achieve is $\mathcal{O}(1/t)$ with the stepsize $\eta_t = 1/(K+t)$ (i.e., the smallest stepsize). We believe that all contributions made in this paper will enrich the knowledge on SGD algorithm, the most popular and powerful algorithm in Machine Learning. 

The paper is organized as follows. The description of SGD algorithm and basic assumptions for our analysis are provided in Section~\ref{sec:SGD_assumptions}. Section~\ref{sec:fundamental} discusses some fundamentals which are used in this paper. We discuss the convergence of SGD in Section~\ref{sec:convergence_SGD}. Section~\ref{sec:conclusion} concludes the paper. 

==> sections/introductionNIPS.tex <==
Title: Optimal Diminishing Stepsizes in SGD for Strong Convex Objective Functions

Abstract:

TO DO Reference paper that shows Adam is no better than SGD -- SGD is the best we can do ... Makes this paper relevant.

We show that by only assuming $\mu$-strongly convex, $L$-smooth, ..

We provide a close to optimal step size function which only depends on $\mu$ and $L$ in that the corresponding convergence rates are at most a factor $32$ away from 

$$  \sup_{ \{f(w;\xi), g(\xi)\} } \frac{ \mathbb{E}[ \| w_{t} - w_{*} \|^2 ] \mbox{ for } \eta'_t }{ \inf_{ \{ \eta_t \} }  \mathbb{E}[ \| w_{t} - w_{*} \|^2 ]} \leq 32.$$


\section{Introduction}

We are interested in solving the following stochastic optimization problem
\begin{align*}
\min_{w \in \mathbb{R}^d} \left\{ F(w) = \mathbb{E} [ f(w;\xi) ] \right\}, \tagthis \label{main_prob_expected_risk}  
\end{align*}
where $\xi$ is a random variable  obeying some distribution. 
In the case of empirical risk minimization with a training set $\{(x_i,y_i)\}_{i=1}^n$, $\xi_i$ is a random variable that is defined 
 by a single random sample  $(x,y)$  pulled uniformly from the training set. Then,  by defining  $f_i(w) := f(w;\xi_{i})$, empirical risk minimization reduces to  
\begin{gather}\label{main_prob}
\min_{w \in \mathbb{R}^d} \left\{ F(w) = \frac{1}{n} \sum_{i=1}^n f_i(w) \right\}.  
\end{gather}

Problems of this type arise frequently in supervised learning applications \cite{ESL}. The classic first-order methods to solve  problem (\ref{main_prob}) are gradient descent (GD) \cite{Nocedal2006NO}  and stochastic gradient descent (SGD)~\footnote{We notice that even though stochastic gradient is referred to as SG in literature, the term stochastic gradient descent (SGD) has been widely used in many important works of large-scale learning.} \cite{RM1951} algorithms. GD is a standard deterministic gradient method, which updates iterates along the negative full gradient with  learning $\eta_t$ as follows
\begin{gather*}
w^{t+1} = w^{t} - \eta_t \nabla F(w^{t}) = w^{t} - \frac{\eta_t}{n} \sum_{i=1}^n \nabla f_i(w^{t}) \ , \ t \geq 1.  
\end{gather*}

We can choose $\eta_t = \eta = \Ocal(1/L)$ and achieve a linear convergence rate for the strongly convex case \cite{nesterov2004}. However, GD requires evaluation of $n$ derivatives at each step, which is very expensive and avoided to use in large-scale optimization. Instead of evaluating full gradient at each step, SGD generates an unbiased random variable $\xi_t$ such as 
$$\mathbb{E}_{\xi_t}[\nabla f(w_t;\xi_t)]=\nabla F(w),$$
and then evaluates gradient $\nabla f(w_t;\xi_t)$. After that, $w_t$ is updated as follows
\begin{gather*}
w^{t+1} = w^{t} - \eta_t \nabla f(w^{t};\xi_t). \tagthis \label{sgd_step}
\end{gather*}
Algorithm \ref{sgd_algorithm} provides a detailed description.
Obviously, the computational cost of SGD is $n$ times cheaper than that of GD. However, as has been shown in literature we need to choose $\eta_t = \Ocal(1/t)$ and the convergence rate of SGD is slowed down to $\Ocal(1/t)$ \cite{bottou2016optimization}, which is a sublinear convergence rate. 

\begin{algorithm}[h]
   \caption{Stochastic Gradient Descent (SGD) Method}
   \label{sgd_algorithm}
\begin{algorithmic}
   \STATE {\bfseries Initialize:} $w_1$
   \STATE {\bfseries Iterate:}
   \FOR{$t=1,2,\dots$}
  \STATE Choose a step size (i.e., learning rate) $\eta_t>0$. 
  \STATE Generate a random variable $\xi_t$.
  \STATE Compute a stochastic gradient $\nabla f(w_{t};\xi_{t}).$
   \STATE Update the new iterate $w_{t+1} = w_{t} - \eta_t \nabla f(w_{t};\xi_{t})$.
   \ENDFOR
\end{algorithmic}
\end{algorithm}

In this paper we focus on the general problem \eqref{main_prob_expected_risk} where $F$ is strongly convex. Since $F$ is strobly convex, a unique optimal solution of \eqref{main_prob_expected_risk} exists and throughout the paper we denote this optimal solution by $w^{*}$. 
The starting point for analysis is the recurrence 
\begin{align*}
\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]  \leq (1-\mu \eta_t) \mathbb{E}[ \| w_{t} - w_{*} \|^2 ] + \eta_t^2 N, \tagthis \label{main_ineq_sgd_new02}
\end{align*}
where  
$$N = 2 \mathbb{E}[ \|\nabla f(w_{*}; \xi)\|^2 ]$$
and $eta_t$ is uper bounded by $\frac{1}{2L}; the recurrence has been shown to hold if we assume (1) $N$ is finite, (2) $F(.)$ is $\mu$-strongly convex, (3) $f(w;\xi)$ is $L$-smooth and (4) convex  \cite{our, leblond}; we detail these assumptions below:

\begin{ass}[$\mu$-strongly convex]
\label{ass_stronglyconvex}
The objective function $F: \mathbb{R}^d \to \mathbb{R}$ is  $\mu$-strongly convex, i.e., there exists a constant $\mu > 0$ such that $\forall w,w' \in \mathbb{R}^d$, 
\begin{gather*}
F(w) - F(w') \geq \langle \nabla F(w'), (w - w') \rangle + \frac{\mu}{2}\|w - w'\|^2. \tagthis\label{eq:stronglyconvex_00}
\end{gather*}
\end{ass}
%It is well-known in literature \cite{nesterov2004,bottou2016optimization} that Assumption \ref{ass_stronglyconvex} implies
%\begin{align*}
%2\mu [ F(w) - F(w_{*}) ] \leq \| \nabla F(w) \|^2 \ , \ \forall w \in \mathbb{R}^d. \tagthis\label{eq:stronglyconvex}
%\end{align*}


\begin{ass}[$L$-smooth]
\label{ass_smooth}
$f(w;\xi)$ is $L$-smooth for every realization of $\xi$, i.e., there exists a constant $L > 0$ such that, $\forall w,w' \in \mathbb{R}^d$, 
\begin{align*}
\| \nabla f(w;\xi) - \nabla f(w';\xi) \| \leq L \| w - w' \|. \tagthis\label{eq:Lsmooth_basic}
\end{align*} 
\end{ass}

Assumption \ref{ass_smooth} implies that $F$ is also $L$-smooth. 
%Then, by the property of $L$-smooth function (in \cite{nesterov2004}), we have, $\forall w, w' \in \mathbb{R}^d$, 
%\begin{align*}
%F(w) &\leq F(w') + \langle \nabla F(w'),(w-w') \rangle + \frac{L}{2}\|w-w'\|^2. \tagthis\label{eq:Lsmooth}
%\end{align*}

%The following additional convexity assumption can be made, as it holds for many problems arising in machine learning.

\begin{ass}\label{ass_convex}
$f(w;\xi)$ is convex for every realization of $\xi$, i.e., $\forall w,w' \in \mathbb{R}^d$, 
\begin{gather*}
f(w;\xi)  - f(w';\xi) \geq \langle \nabla f(w';\xi),(w - w') \rangle.
\end{gather*}
\end{ass}
   
We notice that the earlier established recurrence in \cite{francescopaper} under the same set of assumptions 
\begin{align*}
\mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]  \leq (1-2\mu \eta_t + 2L^2\eta_t^2) \mathbb{E}[ \| w_{t} - w_{*} \|^2 ] + \eta_t^2 N
\end{align*}
is similar, but worse than (\ref{main_ineq_sgd_new02}) as it only holds for $eta_t < \mu /L^2$ where  (\ref{main_ineq_sgd_new02}) holds for $\eta_t\leq 1/(2L)$.  Only for step sizes $eta_t < \mu/(2L^2)$  the above recurrence provides a better bound than (\ref{main_ineq_sgd_new02}). 
In practical settings such as logistic regression  $\mu=\Ocal(1/n)$, $L=\Ocal(1)$, and $t=\Ocal(n)$ (i.e. $t$ is at most a relatively small constant number of epochs, where a single epoch represents $n$ iterations resembling the complexity of a single GD computation). 
As we will show, for this parameter setting the optimally chosen step sizes are $\gg \mu/L^2$. This is the reason we focus in this paper  on analysing recurrence  (\ref{main_ineq_sgd_new02}).
% n practice $\ll 1/(2L)$, since typically  $\mu=\Ocal(1/n)$ is small. For small step sizes 

%for $\mu/L^2\leq eta_t$ (which, as we will show, is true in practice for optimally chosen step sizes, where $\mu=O(1/n)$ and $t=O(n)$ at most a relatively small constant number of epochs).

% 1-2 mu eta + 2L^2 eta^2 < 1 iff eta<mu/L^2
% 1-mu eta < 1-2 mu eta + 2L^2 eta^2  iff mu eta < 2L^2 eta^2 iff mu/(2L^2) < eta

%TO DO: remark on removing convexity -- much later

Recurrence (\ref{main_ineq_sgd_new02}) can be reformulated as:
$$\mbox{For } \eta_t \leq 1/(2L), \hspace{3mm}
 Y_{t+1} \leq (1 - \mu \eta_t)Y_t + \eta_t^2 N, \mbox{ where } Y_t= \mathrm{E}[ \|w_t-w^*\|^2 ]. $$
% \mbox{ where } Y_t = \mathrm{E}[ \|w_t-w^*\|^2 ].$$
%We want to prove an upper bound $Y_t\leq Z_t$. 
If we define recurrence
\begin{equation} Z_0=Y_0 \mbox{ and } Z_{t+1} = (1 - \mu \eta_t)Z_t + \eta_t^2 N, \label{recZ} \end{equation}
then by induction on $t$ we can prove the upper bound  $Y_t\leq Z_t$ if all  $\eta_t \leq 1/(2L)$.

\vspace{2mm}

\noindent
{\bf Contributions:}
\begin{itemize}
\item We characterize the step sizes $\eta_t$ that minimize the convergence rates $Z_t$. We give tight lower and upper bounds on the minimized $Z_t$.
\item We approximate the step sizes $\eta_t$ by step sizes $\eta'_t$ (as given by Th. 2 in \cite{ours}) which only depend on the known parameters $\mu$ and $L$ and do not depend on the unknown parameters $N$ and $Y_0$. We show that our step sizes $\eta'_t$ produce convergence rates $Z'_t$ such that
$$ \frac{Z'_t}{Z_t} \leq 4 ... $$
for $t \geq ...$.
This shows that without knowledge of $N$ and $Y_0$ we can still provide step sizes that lead to convergence rates that meet the optimal solution within a factor 4.
\item For $\mu \neq L$, we provide an example for a distribution $g(\xi)$ and convex and $L$-smooth functions $f(w;\xi)$ leading to a $\mu$-strongly convex function $F(w)$ such that its expected convergence rate $Y'_t$ for the SGD algorithm is such that
$$ \frac{Z_t}{Y'_t} \leq 8 .... $$
for $t \geq ...$.
This shows that $Z_t$ cannot be proven to be smaller by more than a factor 8 under assumptions ..... So, to achieve a better convergence rate we need additional application specific assumptions in order to (hopefully) derive better bounds.
\end{itemize}

TO DO: refer to exact formulas later in the paper; provide the general conclusion as promised in the abstract


%MORE ??????????

%3) we show from a theoretical perspective that the recurrence is strong in that only a decreasing sequence $eta_t\rightarrow 0$ suffices for the convergence rate to tend to zero. This means that the rule of thumb ... can be replaced by .... For the specific examples $1/t^q$ .... this was already shown by .. in their Theorem 1.

%4) to prove the above result we develop a new framework which we show naturally applies to minibatch SGD -- for which we can also show that step size ... is optimal, and the convergence rate remains O(1/g) where g is the number of individual gradient computations done so far in a minibatch SGD. This is consistent with the recent higwild result showing ... delay.

%In the current literature of SGD, there are two following requirements of diminishing stepsizes $\{\eta_t\}$ to make SGD converge: (1) $\sum_{t=1}^{\infty} \eta_t \rightarrow \infty$ and (2) $\sum_{t=1}^{\infty} \eta^2_t < \infty$. In this paper, we show the latter condition is not necessary. Moreover, it is believed that the larger stepsizes $\eta_t$s are, the faster SGD converges. For example, if we consider the class of stepsize $\eta_t=\frac{1}{(K+t)^q}$ for $0<q\leq 1$ and $K$ is a certain positive constant. Then the smaller $q$ (or the larger stepsize $\eta_t$) is, the faster SGD converges. But it is not true. We will show that the fastest convergence rate SGD can achieve is $\mathcal{O}(1/t)$ with the stepsize $\eta_t = 1/(K+t)$ (i.e., the smallest stepsize). We believe that all contributions made in this paper will enrich the knowledge on SGD algorithm, the most popular and powerful algorithm in Machine Learning. 

\vspace{2mm}

\noindent
{\bf Outline:}
The paper is organized as follows. TO DO %The description of SGD algorithm and basic assumptions for our analysis are provided in Section~\ref{sec:SGD_assumptions}. Section~\ref{sec:fundamental} discusses some fundamentals which are used in this paper. We discuss the convergence of SGD in Section~\ref{sec:convergence_SGD}. Section~\ref{sec:conclusion} concludes the paper. 


\section{Solving the Recurrence}

%We recall the upper bound (\ref{main_ineq_sgd_new02}) on the convergence rate $Y_t= \mathrm{E}[ \|w_t-w^*\|^2 ]$: For $\eta_t \leq 1/(2L)$,
%$$ Y_{t+1} \leq (1 - \mu \eta_t)Y_t + \eta_t^2 N. $$
%If we define recurrence
%\begin{equation} Z_0=Y_0 \mbox{ and } Z_{t+1} = (1 - \mu \eta_t)Z_t + \eta_t^2 N, \label{recZ} \end{equation}
%then by induction on $t$ we can prove the upper bound  $Y_t\leq Z_t$ if all  $\eta_t \leq 1/(2L)$.

The recurrence (\ref{recZ}) on $Z_t$ depends on the parameters $L$, $\mu$, $Y_0$, and $N$, where we want to chose the sequence of step sizes $\eta_t$ such that the $Z_t$ are minimized (in order to give the best possible upper bound on $Y_t$) under the constraints $\eta_t \leq 1/(2L)$ (for which $Y_t\leq Z_t$ holds). In practice we know good estimates of $L$ and $\mu$. In our analysis below, we will show that the dependency of `optimal' $\eta_t$ on $Y_0$ and $N$ is in the form of a dependency on $N/Y_0$. We characterize the optimal $\eta_t$ that minimize $Z_t$ and we give precise lower and upper bounds on $Z_t$. 

In Section \ref{sec:app} we use the lower bound on $Z_t$ to show that we can approximate $\eta_t$ by a step size function $\eta'_t$ which does not depend on $N/Y_0$ and we show that the resulting convergence rates meet the minimized $Z_t$ within a small factor for $t$ large enough. In Section \ref{sec:tight} we use the upper bound on $Z_t$ to show that $Z_t$ is a tight bound for $Y_t$ by providing a class of examples for our main problem with convergence rates that meet $Z_t$ within a small factor for $t$ large enough.


\subsection{Minimizing Upper Bound $Z_t$ on the Convergence Rate}

In order to minimize $Z_{t+1}$ as a function of $\eta_t$ we take the derivative of the right hand side in (\ref{recZ}) with respect to $\eta_t$. This gives
$-\mu Z_t + 2\eta_t N$, which is increasing in $\eta_t$ and equals $0$ for $\eta_t= \mu Z_t /(2N)$. This implies that $(1 - \mu \eta_t)Z_t + \eta_t^2 N$ achieves its minimum for $\eta_t= \mu Z_t /(2N)$. Due to constraint $eta_t\leq 1/(2L)$, we should choose
$$ \eta_t = \min \{ 1/(2L) , \mu Z_t/(2N)\}. $$
In other words,
$$ \eta_t = \left\{ \begin{array}{ll}
1/(2L), & \mbox{if } Z_t \geq N/(\mu L), \\
\mu Z_t/(2N), & \mbox{otherwise.} 
\end{array} \right.
$$

Assume for now that $Z_0=Y_0 > N/(\mu L)$. Then, for the first initial recursion steps (\ref{recZ}) translates to
$$ Z_0=Y_0 \mbox{ and } Z_{t+1} = (1 - \frac{\mu}{2L})Z_t + \frac{N}{(2L)^2}$$
till $Z_t\leq N/(\mu L)$. Solving this recursion gives
\begin{eqnarray}
 Z_t &=&  (1-\mu/(2L))^{t} Y_0 + \sum_{i=0}^{t-1} (1-\mu/(2L))^i N/(4L^2) \nonumber \\
 &=&  (1-\mu/(2L))^{t} Y_0 +  [N/(4L^2)] [1-(1-\mu/(2L)^{t}]/[\mu/(2L)] \nonumber \\
 &=& N/(2 \mu L) + (1-\mu/(2L))^{t} (Y_0 - N/(2 \mu L) ). \label{eqZsmall}
 \end{eqnarray}
 This implies that $Z_t\geq N/(2\mu L)$ and $Z_t$ remains $> N/(\mu L)$ as long as 
 $$(1-\mu/(2L))^{t} (Y_0 - N/(2 \mu L) ) > N/(2 \mu L).$$
 This is equivalent to
 $$ t< T \mbox{ where } T=  \frac{\ln( 2 \mu L Y_0/N  - 1)}{\ln( (1- \mu/(2L))^{-1}  )}$$
 (note that $T> 0$ is properly defined since we assume $Y_0>N/(\mu L)$).
 By defining
 $$
  W = \lceil T\rceil = \lceil \frac{\ln( 2 \mu L Y_0/N  - 1)}{\ln( (1- \mu/(2L))^{-1}  )} 
  $$
 (note that $W\geq 1$ since $T>0$)
 we conclude
 \begin{equation} \eta_t = \left\{ \begin{array}{ll}
1/(2L), & \mbox{if } t< W, \\
\mu Z_t/(2N), & \mbox{if } t\geq W .
\end{array} \right.
\label{eqEta}
\end{equation}
 %$$ \eta_t = \left\{ \begin{array}{ll}
%1/(2L), & \mbox{if } t< W, \\
%\mu Z_t/(2N), & \mbox{if } t\geq W
%\end{array} \right.
%$$
with
$$ N/(2\mu L) \leq Z_W \leq N/(\mu L).$$

If $Y_0 \leq N/(\mu L)$, then
$$\eta_t =\mu Z_t/(2N) \mbox{ for } t\geq 0.$$
We may extend the definition of $W$ as follows:
\begin{equation}
W = 
 \left\{ \begin{array}{ll} 
 \lceil \frac{\ln( 2 \mu L Y_0/N  - 1)}{\ln( (1- \mu/(2L))^{-1}  )}\rceil, & \mbox{if } N/Y_0 < \mu L, \\
 0, & \mbox{if } N/Y_0 \geq \mu L.
 \rceil \label{eqW}
  \end{equation}
 %$$ \eta_t = \left\{ \begin{array}{ll}
%1/(2L), & \mbox{if } [t< W \mbox{ and } N/Y_0 < \mu L], \\
%\mu Z_t/(2N), & \mbox{if } [t\geq W \mbox{ and } N/Y_0 < \mu L] \mbox{ or } [t\geq 0 \mbox{ and } N/Y_0\geq \mu L].
%\end{array} \right.
%$$
Then, combining both cases shows that (\ref{eqEta}) holds in general for  the extended definition of $W$.

We conclude that (\ref{eqEta}) with (\ref{eqW})  in combination with recurrence (\ref{recZ}) gives a {\em precise} recursive characterization of  (a) the sequence of step sizes $\eta_t$ that minimizes the upper bound $Z_t$ on the convergence rate $Y_t$, and (b) the minimized upper bound values $Z_t$ themselves.
 
We also note that the above analysis shows
\begin{equation}
Z_W = 
 \left\{ \begin{array}{ll} 
N/(2\mu L) \leq Z_W \leq N/(\mu L), & \mbox{if } N/Y_0 < \mu L, \\
 Y_0\leq  N/(\mu L), & \mbox{if } N/Y_0 \geq \mu L.
\end{array} \right. \label{eqZW}
\end{equation}
We will use this property in the next subsection where we provide lower and upper bounds on the minimizing $Z_t$.


\subsection{Approximating the Minimal Bound $Z_t$ on the Convergence Rate}

For $t<W$ the precise solution is given by $\eta_t=1/(2L)$ and $Z_t=N/(2 \mu L) + (1-\mu/(2L))^{t} (Y_0 - N/(2 \mu L) )$ in (\ref{eqEta})  and (\ref{eqZsmall}); these are easy to interpret closed form expressions. For $t\geq W$, we do not have an easy to interpret close form solution (a closed form can be constructed but depends in a rather complex way on $N$ and $Y_0$). For this reason we will derive easy to interpret lower and upper bounds on $Z_t$.
%For $t\geq W$, the precise solution for $\eta_t$ is a complex function of all parameters including the unknown $Y_0$ and $N$. In this subsection we approximate the minimizing $\eta_t$ in order to gain understanding aboput how $\eta_t$ and $Z_t$ behave as functions of $t$ and each of the parameters $\mu$, $L$, $N$, and $Y_0$.


For $t\geq W$ (assumed throughout the remainder of this section), we substitute  (\ref{eqEta}) for $\eta_t$  in recurrence (\ref{recZ}): 
$$
Z_{t+1} = Z_t - \mu^2 Z_t^2 /(2N) + \mu^2 Z_t^2 /(4N) = Z_t - \mu^2 Z_t^2 /(4N).
$$
Let $\gamma = \mu^2/ (4N)$. We obtain
\begin{equation}
\gamma Z_{t+1} =  \gamma Z_t (1 -\gamma Z_t), \label{eqZZ}
\end{equation}
where (see (\ref{eqZW}))
$$ \gamma Z_W \leq \gamma N/(\mu L) = \mu/(4L).$$
We may rewrite (\ref{eqZZ}) as
$$ (\gamma Z_{t+1})^{-1} = 1+  (\gamma Z_{t})^{-1}  + \frac{1}{ (\gamma Z_{t})^{-1} -1}.$$
This immediately shows that  for $t+1\geq W$,
\begin{equation}
(\gamma Z_{t+1})^{-1} = (t+1-W) + (\gamma Z_{W})^{-1} + \sum_{i=W}^t \frac{1}{ (\gamma Z_{i})^{-1} -1}.\label{eqZZ1}
\end{equation}
This implies the lower bound
\begin{equation}
(\gamma Z_{t+1})^{-1} \geq (t+1-W) + (\gamma Z_{W})^{-1}, \label{eqZZL}
\end{equation}
which can be used in the sum to obtain the  upper bound
\begin{eqnarray*}
\sum_{i=W}^t \frac{1}{ (\gamma Z_{i})^{-1} -1} &\leq&  \sum_{i=0}^{t-W} \frac{1}{i+(\gamma Z_{W})^{-1}} \\
&\approx& \ln(t+1-W+(\gamma Z_{W})^{-1}) - \ln((\gamma Z_{W})^{-1}).
\end{eqnarray*}
  Substituting this into (\ref{eqZZ1}) yields the upper bound
\begin{equation}
(\gamma Z_{t+1})^{-1} \leq (t+1-W) + (\gamma Z_{W})^{-1} + \ln(t+1-W+ (\gamma Z_{W})^{-1}) - \ln( (\gamma Z_{W})^{-1}) \label{eqZZU}
\end{equation}.
Bounds (\ref{eqZZL}) and (\ref{eqZZU}) hold for $t+1\geq W$. Combining these two bounds with $\gamma = \mu^2/ (4N)$ (and substituting $t+1$ by $t$) proves for $t\geq W$,
\begin{eqnarray}
&& \frac{4N}{\mu^2} \frac{1}{ (t-W) + (\mu^2 Z_{W}/(4N))^{-1}} \nonumber\\
&& \hspace{2cm} \geq  Z_{t} \geq  \label{approxZ} \\
&& \frac{4N}{\mu^2} \frac{1}{ (t-W) + (\mu^2 Z_{W}/(4N))^{-1} + \ln(t-W+ (\mu^2 Z_{W}/(4N))^{-1}) - \ln( (\mu^2 Z_{W}/(4N))^{-1})}. \nonumber
\end{eqnarray}

The upper bound and lower bounds in (\ref{approxZ}) are close. In order to gain better understanding we weaken both bounds by using  the bounds on $Z_W$ in (\ref{eqZW}). When we show our tightness example we will compare its convergence rate against the upper bound of the optimal $Z_t$ and this will teach us within what factor our example is tight. When we show how to approximate the minimizing step size function $\eta_t$ by making it independent of the unknown parameters $N$ and $Y_0$, we compare the convergence rate for the approximated $\eta_t$ against the lower bound of the optimal $Z_t$ and this will teach us within what factor the convergence rate corresponding to the approximated $\eta_t$ is close to the optimal $Z_t$.

%Let $t\geq W$ (
The weakened upper and lower bounds will use parameter
$$ \omega = \max\{N/(\mu L Y_0),1\}.$$
For the case $W=0$,  (\ref{eqW}) and (\ref{eqZW}) tell us that $Z_W=Y_0$ and $Y_0\leq N/(\mu L)$, hence, $\omega=N/(\mu L Y_0)$: Substituting this in (\ref{approxZ}) shows
$$\frac{4N}{\mu} \frac{1}{\mu t + 4L\omega }\geq  Z_{t} \geq \frac{4N}{\mu} \frac{1}{ \mu t +4L\omega + \mu[\ln(t+ 4L\omega) - \ln( 4L\omega )]}.$$
%$$\frac{4N}{\mu} \frac{1}{\mu t + 4N/(\mu Y_0) }\geq  Z_{t} \geq \frac{4N}{\mu} \frac{1}{ \mu t +4N/(\mu Y_0) + \mu[\ln(t+ 4N/(\mu Y_0)) - \ln( 4N/(\mu Y_0)])}.$$
     
For the case $W\geq 1$, $Y_0> N/(\mu L)$, hence, $\omega=1$.  From (\ref{eqW}) and (\ref{eqZW}) we infer that  $N/(2\mu L)\leq Z_W\leq N/(\mu L)$. Substituting these upper and lower bounds on $Z_W$ at the appropriate spots in (\ref{approxZ}) shows
$$ \frac{4N}{\mu} \frac{1}{ \mu (t-W) + 4L}\geq  Z_{t} \geq \frac{4N}{\mu} \frac{1}{ \mu (t-W) + 8L + \mu[ \ln(t-W+ 8L) - \ln(4L)]}.$$
By multiplying each $L$ with $\omega=1$ we notice that the upper and lower bounds for both cases start to resemble one another.

Let us analyse $W$.  If $\omega=1$, then, by assuming $\mu/(2L)$ is very small (which is true in practical settings),
\begin{equation} W\approx  \frac{\ln( 2 \mu L Y_0/N  - 1)}{\ln( (1- \mu/(2L))^{-1}  )}
\approx \frac{2L}{\mu} \ln( 2 \mu L Y_0/N  - 1) = \frac{2L}{\mu} \ln( 2 \omega \mu L Y_0/N  - 1).\label{appW}
\end{equation}
If $\omega=N/(\mu L Y_0)$, then
$$\frac{2L}{\mu} \ln( 2 \omega \mu L Y_0/N  - 1) =0$$
and $W=0$ implying (\ref{appW}) also holds for $\omega = N/(\mu L Y_0)$.
Hence, we obtain a general weaker upper bound for both cases:
\begin{equation} Z_t \leq  \frac{4N}{\mu} \frac{1}{ \mu t- 2L \ln( 2 \omega \mu L Y_0/N  - 1) + 4L\omega }.\label{eqUP}
\end{equation}

A general weaker lower bound can be decuced by multiplying $4L\omega$  with $2$ in the case $W=0$ at the approriate spots:
\begin{eqnarray}
Z_t &\geq &  \frac{4N}{\mu} \frac{1}{ \mu t - 2L \ln( 2 \omega \mu L Y_0/N  - 1)   + 8L\omega + \mu[ \ln(t- \frac{2L}{\mu} \ln( 2 \omega \mu L Y_0/N  - 1)+ 8L\omega) - \ln(4L\omega)]} \nonumber \\
&\geq&  \frac{4N}{\mu} \frac{1}{ \mu t   + 8L\omega + \mu[ \ln(t+ 8L\omega) - \ln(4L\omega)]}  \nonumber \\
&=&  \frac{4N}{\mu} \frac{1}{ \mu (t +\ln(t/(4L\omega) +2))   +  8L\omega   }. \label{eqLOW}
\end{eqnarray}

We conclude upper bound (\ref{eqUP}) and lower bound (\ref{eqLOW}) on $Z_t$  for $\mu/(2L)$ small and $t\geq W$.

\section{Approximating the Optimal Step Sizes}

We propose to use upper bound (\ref{eqUP}) on $Z_t$ in (\ref{eqEta}) to create a new, but hopefully close to optimal, candidate step size function $\eta'_t$. According to (\ref{eqEta}) this gives candidate $eta'_t=1/(2L)$  if $t<W\approx \frac{2L}{\mu} \ln( 2 \omega \mu L Y_0/N  - 1)$, and for $t\geq W$,
$$\eta'_t = \frac{2}{ \mu t- 2L \ln( 2 \omega \mu L Y_0/N  - 1) + 4L\omega }.$$
Still $\eta'_t$ depends on the unknown parameter $Y_0/N$ in a rather complex way. A much coarser approximation would be to simply substitute $0$ for $W$ (it seems $W$ may often be equal to $0$ and if not, it may be rather small in relation to the larger $t$ which we see used in practice). And in addition we want to replace constant  $2L \ln( 2 \omega \mu L Y_0/N  - 1) + 4L\omega$ by $4L$ making it independent of $Y_0/N$. This leads to the candidate step size function 
\begin{equation}
 \eta'_t = \frac{2}{\mu t + 4L} \mbox{ for } t\geq 0. \label{eqCand}
 \end{equation}
Note that this candidate step size function has no dependency on the unknown parameters $N$ and $Y_0$ at all.

It turns out that step size function $\eta'_t$ in (\ref{eqCand}) has been analysed in Th. 2 of \cite{ours} where the following convergence bound has been proved: Let $Y_t$ denote the convergence rate for step sizes $\eta'_t$ in the SGD algorithm. 
%Let $Z_t$ be the minimizing solution for the convergence rates for the optimal step sizes $\eta_t$ as analysed in the previous section. 
Then,
\begin{equation} Y'_t \leq  Z'_t = \frac{16N}{\mu} \frac{1}{\mu (t -T') +4L}, \label{eqAPPRSOL} \end{equation}
for ($Y'_0=Y_0$)
$$ t\geq T' =  \frac{4L}{\mu} \max\{ L\mu Y_0/N, 1\} -\frac{4L}{\mu}
= (4L/mu) \omega \mu L Y_0/N - 4L/mu =4L^2 \omega Y_0/N - 4L/\mu.$$

We notice that $\omega \mu L Y_0/N \geq 1$ and $\ln x \leq x-1$ for $x\geq 1$. Applying this to $W$ gives (see (\ref{appW})
$$W \approx \frac{2L}{\mu} \ln( 2 \omega \mu L Y_0/N  - 1) \leq \frac{2L}{\mu} (2\omega \mu L Y_0/N-2) = T'.$$
So, if $t\geq T'$ then also $t\geq W$ and we have the lower bound (\ref{eqLOW}) on $Z_t$. 

Convergence rates $Y_t$ correspond to the optimal step sizes $\eta_t$ and we have shown $Y_t\leq Z_t$. In the next section we show a class of examples that show that this upper bound is tight within a factor $\approx 8$ for $t$ large enough. This means that within a factor $\approx 8$ for $t$ large enough the lower bound (\ref{eqLOW}) on $Z_t$ can be met (or possibly be surpassed) by the $Y_t$ for this class of examples. Therefore,
comparing the 
lower bound (\ref{eqLOW}) on $Z_t$ 
 and the upper bound $Z'_t$ on $Y'_t$ in  (\ref{eqAPPRSOL})  tells us how close the convergence rate corresponding to $\eta'_t$ and the convergence rate corresponding to the optimal $\eta_t$ (as defined in the previous section) are:

For $t\geq T'= 4L^2 \omega Y_0/N - 4L/\mu$, 
$$ (\ref{eqAPPRSOL})/ (\ref{eqLOW})  = \frac{16N}{\mu} \frac{1}{\mu (t -T') +4L} 
/  \frac{4N}{\mu} \frac{1}{ \mu (t +\ln(t/(4L\omega) +2))   +  8L\omega   } 
= 4 \frac{ t +\ln(t/(4L\omega) +2) + \omega 8L/\mu }{(t-T') + 4L/\mu}.$$
Let
$$ t = q (T' +4L/\mu)  - 8L/\mu = q\frac{4L}{\mu} \max\{ L\mu Y_0/N, 1\}- 8L/\mu$$
for some $q\geq 2$ (note that $t\geq T'$).
After substituting this formula for $t$, we obtain
\begin{eqnarray*}
 t +\ln(t/(4L\omega) +2) + \omega 8L/\mu
&=&
 q (T' +4L/\mu)  - 8L/\mu +\ln((q (T' +4L/\mu)  - 8L/\mu)/(4L\omega) +2) + \omega 8L/\mu \\
 &\leq&
 q(T' +4L/\mu) +\ln((q (T' +4L/\mu)  - 8L/\mu)/(4L\omega) +2) + (\omega -1) 8L/\mu\\
 &=& 
  q(T' +4L/\mu) +\ln((q (T'+4L/\mu)/(4L\omega)  - 2/(\mu \omega) +2) + (\omega -1) 8L/\mu.
 \end{eqnarray*}
 In practice $ \mu \leq 1$, hence, $-2/(\mu \omega) \leq -2$ (we remind the reader that $\omega \leq 1$). This gives
 $$  t +\ln(t/(4L\omega) +2) + \omega 8L/\mu \leq q(T' +4L/\mu) +\ln(q (T' +4L/\mu)  ) - \ln(4L\omega) + (\omega -1) 8L/\mu.$$
 
 In the case $\omega = N/(\mu L Y_0)\geq 1$, $T'=0$ and we have $T'+4L/\mu=4L/\mu$. We derive
 $$ \frac{ (\omega -1) 8L/\mu - \ln(4L\omega)}{T' +4L/\mu}
 =
  2(N/(\mu L Y_0) -1)  - \frac{\mu}{4L} \ln(4N/(\mu  Y_0))
  =
  2(N/(\mu L Y_0) -1)  + \frac{\mu}{4L} \ln((\mu  Y_0)/(4N)) .$$
  Inequality $N/(\mu L Y_0)\geq 1$ implies $(\mu  Y_0)/(4N) \leq 1/(4L)$. Therefore,
  $$ \frac{ (\omega -1) 8L/\mu - \ln(4L\omega)}{T'+4L/\mu}
 = 2(N/(\mu L Y_0) -1)  + \frac{\mu}{4L} \ln((\mu  Y_0)/(4N))
 \leq 2(N/(\mu L Y_0) -1)  + \frac{\mu}{4L}  \max\{0, -\ln(4L)\}.$$
  
 In the case $\omega =1\geq N/(\mu L Y_0)$,  $T'+ 4L/\mu = 4L^2  Y_0/N$ and we derive
 $$ \frac{ (\omega -1) 8L/\mu - \ln(4L\omega)}{T'+\beta+4L/\mu}
 =\frac{ - \ln(4L) }{ 4L^2  Y_0/N}= -\frac{N}{4L^2 Y_0} \ln(4L) .$$
 If $4L\geq 1$, then $-\ln(4L)\leq 0$. If $4L<1$, then $-\ln(4L)>0$ and by using $ N/(\mu L Y_0)\leq 1$ we obtain
 $-\frac{N}{4L^2 Y_0} \ln(4L)\leq - (\mu/(4L)) \ln(4L)$. Hence,
 $$\frac{ (\omega -1) 8L/\mu - \ln(4L\omega)}{T' +4L/\mu}
  = -\frac{N}{4L^2 Y_0} \ln(4L)\leq  (\mu/(4L))  \max\{0,  -\ln(4L)\}.$$
  
  Combining both cases gives
  $$ \frac{ (\omega -1) 8L/\mu - \ln(4L\omega)}{T'+4L/\mu} \leq 2\max\{0, N/(\mu L Y_0) -1\} + (\mu/(4L))  \max\{0,  -\ln(4L)\} 
  $$
  Now we can derive (we use $(t-T')+4L/mu = (q-1)(T'+4L/\mu)$)
  $$
 (\ref{eqAPPRSOL})/ (\ref{eqLOW})  = 
 4 \frac{ t +\ln(t/(4L\omega) +2) + \omega 8L/\mu }{(t-T') + 4L/\mu}
 \leq
 4 \frac{ q(T'+4L/\mu) +\ln(q (T'+4L/\mu)  ) - \ln(4L\omega) + (\omega -1) 8L/\mu}{ (q-1)(T' +4L/\mu)}
 =
 4 ( \frac{q}{q-1} + \frac{\ln(q(T' +4L/\mu))}{(q-1)(T' +4L/\mu)} + \frac{ (\omega -1) 8L/\mu - \ln(4L\omega)}{T' +4L/\mu} )
 \leq 
 4( \frac{q + 2\max\{0, N/(\mu L Y_0) -1\} + (\mu/(4L))  \max\{0,  -\ln(4L)\} }{q-1}
  + \frac{\ln(q(T'+4L/\mu))}{(q-1)(T'+4L/\mu)})
 =
 4( \frac{q + 2\max\{0, N/(\mu L Y_0) -1\} + (\mu/(4L))  \max\{0,  -\ln(4L)\} }{q-1} + \frac{\ln( q \frac{4L}{\mu} \max\{ L\mu Y_0/N , 1\}) }{(q-1) \frac{4L}{\mu} \max\{ L\mu Y_0/N , 1\}}).
 $$
 Since $L/\mu\gg 1$ in practice, the last term with the natural logarithm is close to $0$ and also $(\mu/(4L))  \max\{0,  -\ln(4L)\} \approx 0$. We may conclude for $\mu/(2L)\ll 1$,
 \begin{equation}
  (\ref{eqAPPRSOL})/ (\ref{eqLOW})  \leq
 4 \frac{q + 2\max\{0, N/(\mu L Y_0) -1\}  }{q-1} .\label{factorA}
 \end{equation}
 
 So, for $N/(\mu L Y_0)\leq 1$  we can get within a factor  $4\frac{q}{q-1}$ for $t=
   q \frac{4L}{\mu} \max\{ L\mu Y_0/N, 1\} - 8L/\mu =  q \frac{4L}{\mu} L\mu Y_0/N- 8L/\mu\leq (q-2) \frac{4L^2 Y_0}{N}$ with $q\geq 2$. If  $N/(\mu L Y_0)> 1$, i.e., $Y_0/N \leq 1/( \mu L)$, then for  $t= q \frac{4L}{\mu} \max\{ L\mu Y_0/N, 1\} - 8L/\mu =  (q-2)\frac{4L}{\mu}$ with $q\geq 2$ we can get within a factor 
   $4\frac{q+ 2(N/(\mu L Y_0) -1)}{q-1}$. Combining both arguments shows that (\ref{factorA}) holds for
   $$ t\geq (q-2)\frac{4L}{\mu} \max \{ \mu L Y_0/N, 1\} \mbox{ with } q\geq 2.$$
   
    The above shows that the convergence rate of the approximate solution $\eta'_t$ which is independent from $N$ and $Y_0$ approaches bound $Z_t$ on the convergence rate $Y_t$ of the optimal solution $\eta_t$ within a factor close to $4$ for $t$ large enough.
 
\section{Experimental Validation}
 
 TO DO Experimental results show that for common data sets $N/(\mu L Y_0)\leq 1$. .... Compare optimal versus approximate stepsizes. Also depict the bounds:
 \begin{itemize}
 \item Simulated $Y_t$ for optimal stepsizes $\eta_t$
 \item Simulated $Y'_t$ for $\eta'_t$
 \item Actual $Z_t$, and lower and upper bounds on Z_t
 \item The bound $Z'_t$ (on $Y'_t$)
 \end{itemize}
 This shows ``tightness'' within smaller $<32$ factor for practical data sets.
 
 We show in the next section that theoretical examples can be constructed showing that ``this factor'' cannot be larger than 32 -- refer to general conclusion abstract etc.
 
\section{Tightness of the Convergence Rate $Z_t$}
 
 
 We consider a multivariate normal distribution of a $k$-dimensional random vector $\xi$, i.e., $\xi \sim \mathcal{N}(m,\Sigma)$, where $m=\mathrm{E}[\xi]$ and $\Sigma = \mathrm{E}[(\xi-m)(\xi-m)^{\mathrm{T}}]$ is the (symmetric positive semi-definite) correlation matrix. The density function of $\xi$ is
$$
g(\xi) = \frac{\exp( \frac{- (\xi-m)^\mathrm{T}\Sigma^{-1}(\xi-m)}{2} )}{\sqrt{(2\pi)^k|\Sigma|}}. 
$$

We select  component functions 
 $$f(w;\xi)=s(\xi)\frac{\|w-\xi\|^2}{2},$$
 where function $s(\xi) is constructed {\em a-priori} according to the following random process: 
 \begin{itemize} 
 \item With probability $1-\mu/L$, we draw $s(\xi)$ from the uniform distribution over interval $[0, \mu/(1-\mu/L)]$, and
 \item with probability $\mu/L$, we draw $s(\xi)$ from the uniform distribution over interval $[0, L]$.
 \end{itemize}
 Clearly, $f(w;\xi)$ is $s(\xi)$-smooth where the maximum value of $s(\xi)$ is equal to $L$. That is, all functions $f(w;\xi)$ are $L$-smooth (and we cannot claim a smaller smoothness parameter). We notice that
 %%%% Mistake:  x^2 p(x|y=0) p(y=0) +  OKAY mu/L=1-e, then  e (mu/e)/2 etc. distribution with limit e-->0 is funny.
 $$ \mathrm{E}_{\xi}[s(\xi)]  = (1-\mu/L) \frac{\mu/(1-\mu/L)}{2} + (\mu/L) \frac{L}{2} = \mu$$
 and
 $$  \mathrm{E}_{\xi}[s(\xi)^2]  =  (1-\mu/L) \frac{(\mu/(1-\mu/L))^2}{12}+ (\mu/L) \frac{L^2}{12}= \frac{\mu (L + \mu(1-\mu/L))}{12}.$$
 
 
With respect to $f(w;\xi)$ and distribution $g(\xi)$ we define
  $$F(w) = \mathrm{E}_{\xi}[f(w;\xi)] = \mathrm{E}_{\xi}[s(\xi) \frac{\|w-\xi\|^2}{2}].$$
  Since $s(\xi)$ only assigns a random variable to $\xi$ which is drawn from a distribution whose description is not a function of $\xi$, random variables $s(\xi)$ and $\xi$ are staistically independent. Therefore,
   $$F(w) = \mathrm{E}_{\xi}[s(\xi) \frac{\|w-\xi\|^2}{2}] = \mathrm{E}_{\xi}[s(\xi)]  \mathrm{E}_{\xi}[\frac{\|w-\xi\|^2}{2}]
   = \mu  \mathrm{E}_{\xi}[\frac{\|w-\xi\|^2}{2}].
   $$
 Notice:
\begin{enumerate}
\item $\|w-\xi\|^2 = \|(w-m)+(m-\xi)\|^2= \|w-m\|^2 + 2 \langle w-m,m-\xi \rangle + \|m-\xi \|^2$. 
\item Since $m=\mathrm{E}[ \xi ]$, we have $\mathrm{E}[ m-\xi ] =0$.
\item   $\mathrm{E}[ \|m-\xi\|^2 ]=\sum_{i=1}^k \mathrm{E}[ (m_i-\xi_i)^2 ] = \sum_{i=1}^k \Sigma_{i,i} = \mathrm{Tr}(\Sigma)$. 
\end{enumerate}
 Therefore, 
 $$F(w) = \mu  \mathrm{E}_{\xi}[\frac{\|w-\xi\|^2}{2}] = \mu \frac{\|w-m\|^2}{2} + \mu \frac{\mathrm{Tr}(\Sigma)}{2}$, and this shows $F$ is $\mu$-strongly convex and has minimum 
 $$w^* = m.$$
 
 Since
$$\nabla_w [ \|w-\xi\|^2 ] = \nabla_w [ \langle w,w \rangle - 2\langle w,\xi \rangle + \langle \xi,\xi \rangle ] = 2w -2 \xi = 2(w-\xi), 
$$
we have $$ \nabla_w f(w;\xi)= s(\xi)(w-\xi). $$
In our notation 
$$N=2 \mathrm{E}_\xi[\|\nabla f(w^*;\xi) \|^2]=2 \mathrm{E}_{\xi}[s(\xi)^2 \|w^* -\xi \|^2].$$
By using similar arguments we can split the expectation and obtain
$$ N = 2 \mathrm{E}_{\xi}[s(\xi)^2 \|w^* -\xi \|^2] = 2  \mathrm{E}_{\xi}[s(\xi)^2] \mathrm{E}_{\xi}[ \|w^* -\xi \|^2].$$
We already calculated 
$$\mathrm{E}_{\xi}[ \|w^* -\xi \|^2] = \|w^*-m\|^2 + \mathrm{Tr}(\Sigma)= \mathrm{Tr}(\Sigma)$$
and we know $ \mathrm{E}_{\xi}[s(\xi)^2] = \frac{\mu (L + \mu(1-\mu/L))}{12}$. This yields
$$ N =  2  \mathrm{E}_{\xi}[s(\xi)^2] \mathrm{E}_{\xi}[ \|w^* -\xi \|^2]
= \frac{\mu (L + \mu(1-\mu/L))}{6} \mathrm{Tr}(\Sigma).$$

In the SGD algorithm we compute
$$
w_{t+1} = w_t - \eta_t \nabla f(w_t;\xi_t) = w_t - \eta_t s(\xi) (w_t - \xi_t) = (1-\eta_t s(\xi)) w_t + \eta_t s(\xi) \xi_t. 
$$
We choose $w_0$ according to the following computation: We draw $\xi$ from its distribution and apply full grdaient descent in order to find $w^*_\xi$ which minimizes $f(w;\xi)$. Since  $f(w;\xi)=s(\xi)\frac{\|w-\xi\|^2}{2}$, $w^*_i=\xi$ and
$$ Y_0 = \mathrm{E}[ \|w_0-w^*\|^2] = \mathrm{E}[ \|\xi-w^*\|^2]] = \mathrm{Tr}(\Sigma).$$

Again let $\omega = \max\{N/(\mu L Y_0),1\}$. By using our expressions for $N$ and $Y_0$ we derive, for small $\mu/(2L)$,
$$ \omega = \max\{N/(\mu L Y_0),1\} = \max\{ \frac{ 1+ (\mu/L) (1-\mu/L))}{6}, 1\} =1.$$
Furthermore, see (\ref{appW}),
\begin{equation} W \approx \frac{2L}{\mu} \ln( 2 \omega \mu L Y_0/N  - 1)
= 
\frac{2L}{\mu} \ln ( \frac{12}{1 + (\mu/L)(1-\mu/L)} -1) \approx \frac{2 \ln(11) L}{\mu} \approx \frac{4.796\cdot L}{\mu}.\label{eqWtight}
\end{equation}

By defining $\mathcal{F}_t $ TO DO, we derive
$$
\mathrm{E}[ \|w_{t+1}-w^*\|^2 | \mathcal{F}_t ]
=\mathrm{E}[ \|(1-\eta_t s(\xi)) (w_t -w^*) + \eta_t s(\xi) (\xi_t - w^*) \|^2 | \mathcal{F}_t ]
$$
which is equal to 
$$
\mathrm{E}[ (1-\eta_t s(\xi))^2 \|w_t -w^*\|^2 + 2\eta_t s(\xi)(1-\eta_t s(\xi) ) <w_t-w^*, \xi_t - w^*> +  \eta_t^2 s(\xi)^2 \|\xi_t -w*\|^2 | \mathcal{F}_t]. 
$$
Given $\mathcal{F}_t$, $w_t$ is not a random variable. Furthermore, we can use linearity of taking expectations and as above split expectations:
$$
\mathrm{E}[(1-\eta_t s(\xi))^2] \|w_t -w^*\|^2 + \mathrm{E}[2\eta_t s(\xi)(1-\eta_t s(\xi) )] <w_t-w^*, \mathrm{E}[\xi_t - w^*]> + \mathrm{E}[ \eta_t^2 s(\xi)^2] \mathrm{E}[ \|\xi_t -w*\|^2]. $$
Again notice that $\mathrm{E}[\xi_t -w^*] = 0$ and $\mathrm{E}[ \| \xi_t - w^* \|^2 ] = \mathrm{Tr}(\Sigma)$. So,
\begin{eqnarray*}
\mathrm{E}\|w_{t+1}-w^*\|^2 | \mathcal{F}_t ] &=&
\mathrm{E}[(1-\eta_t s(\xi))^2] \|w_t -w^*\|^2  +\eta_t^2 \frac{N}{2}  \\
&=& (1- 2\eta_t \mu + \eta_t^2 \frac{\mu (L + \mu(1-\mu/L))}{12}) \|w_t -w^*\|^2  +\eta_t^2 \frac{N}{2} \\
&=& (1-\mu \eta_t (2 - \eta_t (L + \mu(1-\mu/L))/12)  \|w_t -w^*\|^2  +\eta_t^2 \frac{N}{2} .
\end{eqnarray*}
In terms of $Y_t=\mathrm{E}\|w_{t}-w^*\|^2]$, by taking the full expectation (also over $\mathcal{F}_t$) we get
$$ Y_{t+1} = (1-\mu \eta_t (2 - \eta_t (L + \mu(1-\mu/L))/12)  Y_t  +\eta_t^2 \frac{N}{2}.$$
This is very close to recurrence Equation~\ref{main_ineq_sgd_new02}.

%YEP much better \mathbb{E}[\| w_{t+1} - w_{*} \|^2 ]  \leq (1-2\mu \eta_t + 2L^2\eta_t^2) \mathbb{E}[ \| w_{t} - w_{*} \|^2 ] + \eta_t^2 N
 
 The optimal step size in this case is again solved by taking the derivative with respect to $\eta_t$. The derivative is now equal to
 $$-2\mu Y_t + 2\eta_t \mu  (L + \mu(1-\mu/L)) Y_t/12 + N\eta_t$$
 which shows the minimum is achieved for
 $$ \eta_t = \frac{ 2\mu Y_t }{N + \mu  (L + \mu(1-\mu/L)) Y_t/6}$$
 giving
% $$  Y_{t+1} = (1- 2  \frac{ 2\mu Y_t }{N + \mu  (L + \mu(1-\mu/L)) Y_t/6}\mu ) Y_t + (\frac{ 2\mu Y_t }{N + \mu  (L + \mu(1-\mu/L)) Y_t/6})^2 (N/2 + 
 % \frac{\mu (L + \mu(1-\mu/L))}{12} Y_t)
 %  = (1- 2  \frac{ 2\mu Y_t }{N + \mu  (L + \mu(1-\mu/L)) Y_t/6}\mu ) Y_t + \frac{ 2(\mu Y_t)^2 }{N + \mu  (L + \mu(1-\mu/L)) Y_t/6}
 % = Y_t - \frac{ 4\mu^2 Y_t^2 }{N + \mu  (L + \mu(1-\mu/L)) Y_t/6}+ \frac{ 2(\mu Y_t)^2 }{N + \mu  (L + \mu(1-\mu/L)) Y_t/6}
 % = Y_t - \frac{ 2\mu^2 Y_t^2 }{N + \mu  (L + \mu(1-\mu/L)) Y_t/6}.$$
  $$  Y_{t+1} =Y_t - \frac{ 2\mu^2 Y_t^2 }{N + \mu  (L + \mu(1-\mu/L)) Y_t/6}
  = Y_t - \frac{ 2\mu^2 Y_t^2 }{N (1+ Y_t/ \mathrm{Tr}(\Sigma))}.$$
  
  We proceed by proving a lower bound on $Y_t$.
  Clearly,
  $$  Y_{t+1} \geq Y_t - \frac{ 2\mu^2 Y_t^2 }{N}.$$
  We may use the exact same derivation from (\ref{eqZZ}) onwards with $\gamma = 2\mu^2/N$ (and $W=0$ since the recursion on $Y_t$ already holds from $0$ onwards).
  This gives a bound similar to (\ref{eqZZU}): 
$$(\gamma Y_{t+1})^{-1} \leq (t+1) + (\gamma Y_0)^{-1} + \ln(t+1+ (\gamma Y_0)^{-1}) - \ln( (\gamma Y_0)^{-1}) $$
Reordering, substituting $\gamma = 2\mu^2/N$, and replacing  $t+1$ by $t$ yields, for $t\geq 0$, the lower bound
\begin{eqnarray}
 Y_t &\geq&  \frac{N}{2\mu} \frac{1}{\mu t + N/(2 Y_0) + \mu[ \ln(t+ \frac{N}{2\mu Y_0} ) - \ln( \frac{N}{2\mu Y_0} )]} \nonumber \\
&=& \frac{N}{2\mu} \frac{1}{\mu t + \frac{\mu (L + \mu(1-\mu/L))}{12} + \mu[ \ln(t+ L \frac{ 1 + (\mu/L)(1-\mu/L)}{12} ) - \ln(  L \frac{ 1 + (\mu/L)(1-\mu/L)}{12} )]} \nonumber  \\
&\approx $  \frac{N}{2\mu} \frac{1}{\mu (t + \ln(t+ L/12 ) )} , \label{tightLOW}
\end{eqnarray}
where the approximation follows from $\mu/(2L)\ll 1$. 


We notice that $Y_t\leq Z_t$ and $Z_t$ satisfies the upper bound (\ref{eqUP}) for $t\geq W \approx \frac{4.796\cdot L}{\mu}$  (see the derivation above for $W$ in (\ref{{eqWtight})):
\begin{eqnarray}
Z_t &\leq&  \frac{4N}{\mu} \frac{1}{ \mu t- 2L \ln( 2 \omega \mu L Y_0/N  - 1) + 4L\omega } \nonumber \\
&=&  \frac{4N}{\mu} \frac{1}{ \mu t- 2L \ln( 2  \mu L Y_0/N  - 1) + 4L } \nonumber \\
&\approx&  \frac{4N}{\mu} \frac{1}{ \mu t- 2L \ln(11) + 4L } = \frac{4N}{\mu} \frac{1}{ \mu t- 0.796\cdot L }  . \label{tightZUP}
\end{eqnarray}
Now we can compare (\ref{tightLOW}) and (\ref{tightZUP}): For $t\geq  \frac{4.796\cdot L}{\mu}$,
\begin{equation}
\frac{(\ref{tightUP})}(\ref{tightLOW}) 
= \frac{ \frac{4N}{\mu} \frac{1}{ \mu t- 0.796\cdot L }}{ \frac{N}{2\mu} \frac{1}{\mu (t + \ln(t+ L/12 ) )}}
= 8 \frac{t + \ln(t+ L/12 )}{ t - 0.796\cdot L/\mu }.
\label{factorT}
\end{equation}
This proves that for large enough $t$, our example meets the minimizing $Z_t$ within a factor $\approx 8$. In other words, the bound $Y_t\leq Z_t$ cannot be improved by a factor larger than $8$ unless additional assumptions are stated with which a smaller bound can be proven.

As a final note we remark that the above analysis also holds if we define each component function $f(w;\xi)$ with its own symmetric  positive semi-definite correlation matrix $\Sigma(\xi)$ drawn from a general distribution with $\mathrm{E}[\Sigma(\xi)]=\Sigma$. This shows that the class of examples leading to a tight bound is even somewhat more general and larger.


\section{Concluding Remarks}

\noindent
{\bf Summary.} We should that the convergence rate $Y_t$ in SGD can be upper bounded by $Y_t\leq Z_t$ where (after minimization over all possible step size functions) $Z_t$ is characterized by  (\ref{eqEta}) with (\ref{eqW})  in combination with recurrence (\ref{recZ}). The resulting $Z_t$ is a complex function in the unknown parameters $N$ and $Y_0$. In we show  lower and upper bounds,  (\ref{eqLOW}) and  (\ref{eqUP}),  on $Z_t$ that are simple functions in $N$ and $Y_0$ and hold for $\mu/(2L)$ small and $t\geq W$ with $W$ satisfying (\label{appW}).

The lower and upper bounds allow us to conclude our two main results assuming $\mu/L$ small:
\negin{enumerate}
\item For step sizes $\eta'_t  = \frac{2}{\mu t + 4L}$,  for $ t\geq 0$, see (\ref{eqCand}) and Th. 2 in \cite{ours}, we show that the resulting convergence rates $Y_t$ are upper bounded by  (\ref{eqAPPRSOL}) and we use this to prove that $Y_t$ is at most a factor $\tau_1$ larger than the lower bound (\ref{eqLOW}) on $Z_t$, where (see (\ref{factorA}))
$$ \tau_1 \leq  4 \frac{q + 2\max\{0, N/(\mu L Y_0) -1\}  }{q-1}$$
and
$$  t\geq (q-2)\frac{4L}{\mu} \max \{ \mu L Y_0/N, 1\} \mbox{ with } q\geq 2.$$
This shows that $Y_t$ is at most  approximately a factor $4$ worse than $Z_t$ for $t=O(L/\mu)$ large enough.
\item We provide a class with problems $\tt{P}'$ of $\mu$-strongly convex objective functions $F(w)$ with convex $L$-smooth component functions $f(w;\xi)$ and distribution $g(\xi)$ for which the SGD algorithm achieves  convergence rates $Y_t$ with the property that the upper bound  (\ref{eqUP}) on $Z_t$ is at most a factor $\tau_2$ larger than $Y_t$, where (see (\ref{factorT})
$$ \tau_2 \leq 8 \frac{t + \ln(t+ L/12 )}{ t - 0.796\cdot L/\mu }.
\label{factorT}$$
and
$$ t\geq  \frac{4.796\cdot L}{\mu}.$$
This shows that, for this class of examples,  $Z_t$  is at most approximately a factor $8$ worse than $Y_t$ for $t=O(L/\mu)$ large enough.
\end{itemize}

The above results show that if we define the convergence rate  $Y_t(\tt{P}, \eta)$ in SGD as a function of the problem statement $\tt{P}$ and the step size function $\eta$, and  if we define the minimizing upper bound $Z_t(\tt{P})$ as a function of the problem statement $\tt{P}$ (minimized over all possible step size functions),
then, for $t=O(\mu/L)$, we have 
$\inf_{\eta} Y_t(\tt{P},\eta) \leq Z_t(\tt{P})$,
$$ Y_t(\tt{P},\eta') \leq \tau_1 Z_t(\tt{P}),$$
and
$$ Z_t(\tt{P}') \leq \tau_2 \inf_{\eta} Y_t(\tt{P}',\eta).$$
This implies that $Z_t(\tt{P}')$ is close to $\inf_{\eta} Y_t(\tt{P}',\eta)$ within a factor $\tau_2\approx 8$, and $Y_t(\tt{P},\eta')$ meets $ Z_t(\tt{P}$ within a factor $\tau_1\approx 4$. As result 
$$ \sup_{\tt{P}}  Y_t(\tt{P},\eta') \leq \tau_1 \tau_2  \sup_{\tt{P}}  \inf_{\eta} Y_t(\tt{P},\eta),$$
where $\tau_1\tau_2 \approx 32$ for $t=O(L/\mu)$ large enough.
This shows that choosing stepsizes $\eta'_t$ is a factor 32 close to optimal.

\vspace{2mm}

\noindent
{\bf Convexity.} If we do not require the component functions $f(w;\xi)$ to be convex as in Th. 3 in \cite{ours}, then the general recurrence will only hold for much smaller step sizes\footnote{As for the recurrence in \cite{francescopaper}, see introduction. The proof in  \cite{francescopaper} does require the component functions to be convex.} $\eta_t\leq \mu/(2L^2)$. This means that our anlysis will lead to much larger $W$ and as a result  the above conclusion will only hold for $t=O( (L/\mu)^2)$.

TO DO Verify -- should be easy.

\vspace{2mm}

\noindent
{\bf Minibatch SGD.} TO DO (if we want this): Write out recurrence with $k_t$. One can do a similar analysis as above -- quickly verify what it gives -- my bet: the exact same factors. And no improvement over SGD at all, except $W$ may be smaller, so only $t=O(L/(k \mu))$ will be sufficient for our conclusions  ($k_t \approx k$).

\vspace{2mm}

\noindent
{\bf Transition Linear to Sublinear Convergence.} Our anlysis of $Z_t$ shows that for $t< W$ we can achieve linear convergence and for $t\geq W$ we achieve sublinear convergence. Our approximate solution $\eta'_t$ only starts to lead to convergence rates that come within a factor $4$ of $Z_t$ for $t$ at least a multiple of $W$, about $t\approx 2W$. This shows that the approximate solution completely misses the linear convergence phase. Yet, it catches up with some delay of $\approx 2W=O(\mu/L)$ after which the approximate solution achieves a convergence rate at iteration $t$ which lags about $4/\mu$ iterations behind (in that it achieves the convergence rate of the optimal solution at iteration $t-4/\mu$). TO DO HMMM - NOT SURE ABOUT THIS LAST CONCLUSION: VERIFY and remove or adapt, what do the experiments tell?

TO DO explain the above better


